Support vector machines and linear regression coincide with very high-dimensional features

The support vector machine (SVM) and minimum Euclidean norm least squares regression are two fundamentally different approaches to fitting linear models, but they have recently been connected in models for very high-dimensional data through a phenomenon of support vector proliferation, where every training example used to fit an SVM becomes a support vector. In this paper, we explore the generality of this phenomenon and make the following contributions. First, we prove a super-linear lower bound on the dimension (in terms of sample size) required for support vector proliferation in independent feature models, matching the upper bounds from previous works. We further identify a sharp phase transition in Gaussian feature models, bound the width of this transition, and give experimental support for its universality. Finally, we hypothesize that this phase transition occurs only in much higher-dimensional settings in the $\ell_1$ variant of the SVM, and we present a new geometric characterization of the problem that may elucidate this phenomenon for the general $\ell_p$ case.

==> SVM NeurIPS (3)/abstract.tex <==
The support vector machine (SVM) and minimum Euclidean norm least squares regression are two fundamentally different approaches to fitting linear models, but they have recently been connected in models for very high-dimensional data through a phenomenon of support vector proliferation, where every training example used to fit an SVM becomes a support vector.
In this paper, we explore the generality of this phenomenon and make the following contributions.
First, we prove a super-linear lower bound on the dimension (in terms of sample size) required for support vector proliferation in independent feature models, matching the upper bounds from previous works.
We further identify a sharp phase transition in Gaussian feature models, bound the width of this transition, and give experimental support for its universality.
Finally, we hypothesize that this phase transition occurs only in much higher-dimensional settings in the $\ell_1$ variant of the SVM, and we present a new geometric characterization of the problem that may elucidate this phenomenon for the general $\ell_p$ case. 

==> SVM NeurIPS (3)/asymptotic_new.tex <==
\section{Exact asymptotic threshold for Gaussian samples}\label{sec:asymptotic}
% \todo{Consistency of $\tau$ notation.}

% In Section~\ref{sec:nonasymp}, we observe that for training data with independent anisotropic subgaussian components, support vector proliferation occurs with high probability if $d = \Omega(n \log n)$ and does not occur with high probability if $d = O(n \log n)$ by analyzing \navid{Leave one out terms} \eqref{eq:1}. 
Section~\ref{sec:nonasymp} shows the existence of a change in model behavior when $d = \Theta(n \log n)$ without identifying a precise threshold where this phase transition appears.
% However it is natural to ask whether there is a sharp transition at this rate. 
Here, we refine that analysis for the isotropic Gaussian case to find such an exact threshold. 
That is, if $d = 2\tau n \log n$, as $n$ becomes large, SVP will occur when $\tau > 1$ and will not occur when $\tau < 1$. Roughly speaking, this phenomenon stems from the fact that terms in \eqref{eq:1} are weakly correlated, which causes \eqref{eq:1} to behave similarly to a maximum of independent Gaussians.
%$\bg_1,\dotsc,\bg_n$:
%\[
%\pr{ \max_{i \in [n]} y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \bx_i \geq 1 } \asymp \pr{ \sqrt{\text{Var}\paren{ y_1 y_{\setminus 1}^\T \bK_{\setminus 1}^{-1} \bX_{\setminus 1} \bx_1 }} \max_{i \in [n]} \bg_{i} \geq 1 }.
%\]
Furthermore, we characterize the rate at which the phase transition sharpens.
The following theorem shows that if the convergence $\tau \to 1$ is slow enough, then the asymptotic probabilities of SVP are degenerate and the width of the transition is bounded.

% \todo{eliminate $\ln$.} \navid{renewed the ln command so it should be ok}

\begin{restatable}[Sharp SVP phase transition]{theorem}{thmasymptotic}\label{thm:asymptotic}
  Let $(\bX,y)$ be an isotropic Gaussian sample.
  Let $(\eps_{n})_{n \ge 1}$ be any sequence of positive real numbers such that $\limsup_{n\to\infty} \eps_n < 2-c_1$ for some $c_1>0$ and $\liminf_{n \to \infty}{\eps_{n}\sqrt{\log{n}}} > C_2$ for some $C_2>0$ depending only on $c_1$.
  Then,
  \begin{equation*}
    \lim_{n \to \infty} \prl{\text{SVP occurs for $\ell_{2}$-SVM}} =
    \begin{cases}
      0 & \text{if $d = (2 - \eps_{n}) n \ln n $} , \\
      1 & \text{if $d = (2 + \eps_{n}) n \ln n $} .
    \end{cases}
  \end{equation*}
\end{restatable}

\begin{remark}\label{rmk:transition-width}
% \daniel{is this remark about $\delta$ and $1-\delta$ technically correct?} \navid{With the new formulation and rates it is correct right?}
% Given $\delta \in (0,\fracl{1}{2})$ let $w^{(\delta)}_{n}$ be the width of phase transition.
Theorem~\ref{thm:asymptotic} characterizes the width of the phase transition: the difference $w_n$ between the values of $d$ where the probability of SVP is (say) $0.9$ and $0.1$ satisfies $w_n = O(n \sqrt{\log{n}})$.
\end{remark}

%\begin{theorem}[Exact upper-bound on support vector proliferation]\label{thm:asymptotic-up}
% 	Consider training samples $\bX := [\bx_1 |  \dots | \bx_n]^T$, where each $\bx_i \sim \mathcal{N}(0, I_d)$ is independently drawn.
%    Let $\bX$ and $y$ be a Gaussian isotropic sample.
%	For all $\eps, \delta \in (0, 1)$, there exists a sufficiently large $n$ such that if $d = (2 + \eps) n \ln n$, then with %probability $1 - \delta$, every training sample is a support vector for the solution to the $\ell_2$ SVM problem.
%\end{theorem}

It remains an open problem to determine if this transition width estimate is sharp.
Specifically, the bound can be sharpened by exhibiting some sequence $\eps_n$ for which the asymptotic probability of support-vector proliferation is non-degenerate.

The proof of Theorem~\ref{thm:asymptotic} is given in Appendix~\ref{app:asymp-proofs}.
In the case where $d = (2  - \eps_n) n \ln n$, the proof mirrors that of Theorem~\ref{thm:anisotropic}, but deviates in the final step by using the limiting distribution of the maximum of independent Gaussians.
When $d = (2 + \eps_n) n \ln n$, we follow the basic argument in the proof of Theorem~\ref{thm:hmx-ub} from \cite{hmx20}, but we sharpen the analysis by taking advantage of Gaussianity to find the limiting probability as $n\to\infty$.

%\navid{do you think this is true? this is the only thing that came to my mind to motivate the width...}
%It does not appear coincidental that the required form of $\epsilon_n$ is of the same order as the asymptotic standard deviation of $\max_{i \in [n]} \bg_{i}$ (which is  $1/\sqrt{2\log n}$).
%The Central Limit Theorem used in Lemma~\ref{lemma:e3} does not give sufficiently tight anti-concentration bounds on approximately-Gaussian random variables to ensure a constant threshold; 


==> SVM NeurIPS (3)/asymptotic_old.tex <==
\section{Exact asymptotic rate for Gaussian case}\label{sec:asymptotic}

In Section~\ref{sec:nonasymp}, we observe that for training data with independent isotropic subgaussian components, support vector proliferation occurs with high probability if $d = \Omega(n \log n)$ and does not occur with high probability if $d = O(n \log n)$.
Here, we refine that analysis for the spherical Gaussian case to find an exact threshold. 
That is, if $d = \tau n \ln n$, as $n$ becomes large, support vector proliferation will occur when $\tau > 2$ and will not occur when $\tau < 2$.
The two following theorems jointly show this sharp threshold.

\todo{revise these theorems to say something about the width of confidence intervals}

\navid{can we combine both of the theorems into one?}

\begin{theorem}[Exact lower-bound on support vector proliferation]\label{thm:asymptotic-lb}
% 	Consider training samples $\bX := [\bx_1 |  \dots | \bx_n]^T$, where each $\bx_i \sim \mathcal{N}(0, I_d)$ is independently drawn.
	Let $\bX$ and $y$ be a Gaussian isotropic sample.
	For all $\eps, \delta \in (0, 1)$, there exists a sufficiently large $n$ such that if $d = (2 - \eps) n \ln n$ \clayton{something stupid about rounding and floors}, then with probability $1 - \delta$, at least one training sample is not a support vector for the solution to the $\ell_2$ SVM problem.
\end{theorem}

\begin{theorem}[Exact upper-bound on support vector proliferation]\label{thm:asymptotic-up}
% 	Consider training samples $\bX := [\bx_1 |  \dots | \bx_n]^T$, where each $\bx_i \sim \mathcal{N}(0, I_d)$ is independently drawn.
    Let $\bX$ and $y$ be a Gaussian isotropic sample.
	For all $\eps, \delta \in (0, 1)$, there exists a sufficiently large $n$ such that if $d = (2 + \eps) n \ln n$, then with probability $1 - \delta$, every training sample is a support vector for the solution to the $\ell_2$ SVM problem.
\end{theorem}


We relegate both proofs to Appendix~\ref{app:asymp-proofs}.
The proof of Theorem~\ref{thm:asymptotic-up} mirrors that of Theorem~\ref{thm:anisotropic}, but deviates in the final step.
The Central Limit Theorem used in Lemma~\ref{lemma:e3} does not give sufficiently tight anti-concentration bounds on approximately-Gaussian random variables to ensure a constant threshold; instead, the proof of Theorem~\ref{thm:asymptotic-lb} takes advantage of the Gaussianity assumption to make use of known concentration properties about the maximum of independent Gaussians.
The proof of Theorem~\ref{thm:asymptotic-up} relies only on Gaussian concentration bounds.

==> SVM NeurIPS (3)/asymptotic_proofs_new.tex <==
\section{Proofs for Section~\ref{sec:asymptotic}}\label{app:asymp-proofs}

In this section, we give the proof of Theorem~\ref{thm:asymptotic}.

\thmasymptotic*

We divide the proof into two cases, which we each prove in the two following subsections.

\subsection{Below the threshold}

We first consider the case where the dimension is below the threshold, specifically $d = (2-\eps_n) n \log n$.

Our proof follows the same strategy as that of Theorem~\ref{thm:anisotropic}.
Let $m :=  n / \log n$ and assume $n$ is sufficiently large so that $m \leq n/2$.
Using the equivalence from Proposition~\ref{prop:equiv}, it suffices to  show that the following event has probability tending to $1$:
\[
  \max_{i \in [m]}
  \bracket{
    y_i y_{\setminus i}^\T \paren{\bK_{\setminus i}^{-1}-\frac{1}{d} I_{n-1}} \bX_{\setminus i} \bx_i 
    + \frac{1}{d} y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i 
    + \frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{\setminus [m]} \bx_i
  } \geq 1
  .
\]

\begin{lemma} \label{lem:asymptotic-lb1}
  For any $C_0>0$ and $c_1 \in (0,2)$, there exists $C_2>0$ and $n_0 > 0$ such that the following statements hold for all $n \geq n_0$, and all $\eps_n$ satisfying $2-c_1 \geq \eps_n \geq C_2/\sqrt{\log n}$ for all $n \geq n_0$, with $d = (2-\eps_n)n\log n$:
  \begin{enumerate}
    \item $\displaystyle \pr{\bK_{\setminus i} \text{ is invertible,} \ \max_{i \in [m]} \abs{y_i y_{\setminus i}^\T \paren{ \bK_{\setminus i}^{-1} - \frac{1}{d} I_{n-1} } \bX_{\setminus i} \bx_i } \le \frac{\eps_{n}}{2C_0} } \geq 1 - \frac1n$.

    \item $\displaystyle \pr{ \max_{i \in [m]} \abs{\frac{1}{d} y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i} \leq \frac{\eps_{n}}{2C_0} } \geq 1 - \frac1n$.

  \end{enumerate}
\end{lemma}
\begin{proof}
  We start with the first claim.
  By Lemma~\ref{lemma:e1} and a union bound, we have with probability at least $1 - 1/n$, $\bK_{\setminus i}$ is invertible and
  \begin{align*}
    \max_{i \in [m]}
    \abs{ y_i y_{\setminus i}^\T \paren{ \bK_{\setminus i}^{-1} - \frac{1}{d} I_{n-1} } \bX_{\setminus i} \bx_i }
    & \le C \sqrt{\frac{n \log(mn)}{d}}
    \paren{ \sqrt{\frac{n + \log(mn)}{d}} + \frac{n + \log(mn)}{d} } .
  \end{align*}
  For sufficiently large $n$, we have $d \geq c_1 n \log n$ and
  \begin{align*}
    C \sqrt{\frac{n \log(mn)}{d}}
    \paren{ \sqrt{\frac{n + \log(mn)}{d}} + \frac{n + \log(mn)}{d} }
    & \leq
    2C \sqrt{\frac{n \log(mn)}{d}} \sqrt{\frac{n + \log(mn)}{d}} \\
    & \leq \frac{3Cn\sqrt{\log n}}{(2-\eps_n)n\log n} + \frac{4C\sqrt{n}\log n}{c_1 n\log n}
  .
  \end{align*}
  The second term on the right-hand side is at most $C_2/(4C_0\sqrt{\log n})$ for sufficiently large $n$, and hence at most $\eps_n/(4C_0)$.
  The first term on the right-hand side is also at most $\eps_n / (4C_0)$ provided that
  \begin{equation*}
    (2-\eps_n) \eps_n \geq \frac{12C_0 C}{\sqrt{\log n}} ,
  \end{equation*}
  which is equivalent to
  \begin{equation*}
    \eps_n \geq 1 - \sqrt{1 - \frac{12C_0 C}{\sqrt{\log n}}}
  \end{equation*}
  (since we already assume $\epsilon_n \leq 2-c_1$ for sufficiently large $n$).
  This is satisfied provided that $C_2 \geq 12C_0 C$.
  This proves the first claim.

  For the second claim, we have by Lemma~\ref{lemma:e2} (with $n$ in the statement of Lemma~\ref{lemma:e2} set to $m-1$) and a union bound, we have with probability at least $1 - 1/n$:
  \begin{align*}
    \max_{i \in [m]}
    \abs{\frac{1}{d} y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i}
    & \leq 
    C \paren{\sqrt{\frac{m \log{m} + m\log(mn)}{d}} + \frac{\sqrt{m} \log(mn)}{d} } \\
    & \leq \sqrt{\frac{C'n}{d}} +\frac{C'n}{d\log n}
  \end{align*}
  where the second inequality uses $m = n / \log n \leq n/2$ and holds for sufficiently large $n$, with $C'>0$ an absolute constant.
  The second term on the right-hand side is at most $C_2/(4C_0\sqrt{\log n})$ for sufficiently large $n$, and hence also at most $\eps_n/(4C_0)$.
  The first term on the right-hand side is also at most $\eps_n/(4C_0)$ provided that
  \begin{equation*}
    \frac{16C_0C'}{\log n} \leq (2-\eps_n) \eps_n^2 .
  \end{equation*}
  Since $\eps_n \leq 2-c_1$, the above condition holds as long as $C_2 \geq 4\sqrt{C_0C'/c_1}$.
  This proves the second claim.
\end{proof}

\begin{lemma} \label{lem:asymptotic-lb2}
  For any $C_0>4$ and $c_1 \in (0,2)$, there exists $C_2>0$ such that the following holds for all sequences $(\eps_n)$ satisfying $2-c_1 \geq \eps_n \geq C_2/\sqrt{\log n}$ for all large enough $n$, with $d = (2-\eps_n)n\log n$:
  \begin{equation*}
    \lim_{n\to\infty}
    \pr{
      \max_{i \in [m]}
      \frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i \geq 1 + \frac{\eps_{n}}{C_0}
    } = 1
    .
  \end{equation*}
\end{lemma}

\begin{proof}
  Observe that conditioned on $\bX_{\setminus [m]}$, the $m$ random variables
  \begin{equation*}
    \frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i , \quad i = 1,\dotsc,m
  \end{equation*}
  are distributed as independent mean-zero Gaussian random variables with variance
  \begin{equation*}
    \sigma^2 := \frac{1}{d^2} \norml[2]{y_{\setminus [m]}^\T \bX_{ \setminus [m]}}^2 .
  \end{equation*}
  Therefore, the claim is equivalent to
  \begin{equation*}
    \lim_{n\to\infty} \pr{ \max_{i \in [m]} \sigma \bg_i \geq 1 + \frac{\eps_{n}}{C_0}} = 1 ,
  \end{equation*}
  where $\sigma^2$ is as defined above, and $\bg_1,\dotsc,\bg_m$ are i.i.d.~standard Gaussian random variables, independent of $\sigma^2$.

  Observe that
  \begin{equation*}
    \bG := \frac{1}{\sqrt{n-m}} \bX_{\setminus [m]}^\T y_{\setminus [m]}
  \end{equation*}
  is a standard Gaussian random vector in $\R^d$.
  By Gaussian concentration of Lipschitz functions~\cite[page 41, 2.35]{ledoux2001concentration}, the following holds with probability at least $1-1/n$:
  \begin{align}
    \sigma
    & \geq \frac{\sqrt{n-m}}{d}
    \paren{ \E{ \norm[2]{\bG} } - \sqrt{2\log n} }
    \nonumber \\
    & \geq \frac{\sqrt{n-m}}{d}
    \paren{ \sqrt{d} - \frac1{2\sqrt{d}} - \sqrt{2\log n} }
    \nonumber \\
    & = \sqrt{\frac{n-m}{d}}
    \paren{ 1 - \frac1{2d} - \sqrt{\frac{2\log n}{d}} }
    \nonumber \\
    & =
    \frac1{\sqrt{2\log n}}
    \frac1{\sqrt{1 - \frac{\eps_n}{2}}}
    \sqrt{1-\frac1{\log n}}
    \paren{ 1 - \frac1{2d} - \sqrt{\frac{2\log n}{d}} }
    \label{eq:good-variance-proxy}
  \end{align}
  where the second inequality follows from standard approximations of the Gamma function, and the final inequality holds assuming $C_2 \geq 1$.

  Let $\mathsf{E}$ be the event in which \eqref{eq:good-variance-proxy} holds.
  Then
  \begin{align*}
    \pr{ \max_{i \in [m]} \sigma \bg_i \geq 1 + \frac{\eps_n}{C_0} }
    & \geq
    \pr{ \max_{i \in [m]} \sigma \bg_i \geq 1 + \frac{\eps_n}{C_0} \mid \mathsf{E} } \paren{ 1 - \frac1n } \\
    & \geq
    \pr{ \max_{i \in [m]} \bg_i \geq \alpha_n \sqrt{2\log n} } \paren{ 1 - \frac1n }
  \end{align*}
  where
  \begin{equation*}
    \alpha_n := 
    \frac{\paren{ 1 + \frac{\eps_n}{C_0} }\sqrt{1 - \frac{\eps_n}{2}}}
    { \sqrt{1 - \frac{1}{\log n}} \paren{ 1 - \frac1{2d} - \sqrt{\frac{2\log n}{d}} } }
    .
  \end{equation*}
  We claim that the probability on the right-hand side tends to $1$ with $n\to\infty$ as well.

  The distribution of the random variable $\max_{i \in [m]} \bg_i$ obeys a limiting Gumbel distribution; specifically, for all $x>0$,
  \begin{equation*}
    \lim_{m\to\infty} \pr{
      \max_{i \in [m]} \bg_i \geq \sqrt{2\log m} - \frac{x + C \log \log m}{\sqrt{\log m}}
    }
    = 1 - e^{-e^x}
  \end{equation*}
  where $C>0$ is an absolute constant~\cite{fisher1928limiting}.
  Therefore, it suffices to show that for all $x>0$, we have
  \begin{equation*}
    \sqrt{2\log m} - \frac{x + C \log \log m}{\sqrt{\log m}}
    - \alpha_n \sqrt{2\log n} \geq 0
  \end{equation*}
  for all sufficiently large $n$.
  Dividing through by $\sqrt{2\log n}$ and using $m = n /\log n$, the above inequality is implied by
  \begin{equation}
    \sqrt{1 - \frac{\log\log n}{\log n}} - \frac{x + C \log \log (n/2)}{\log n} \frac1{\sqrt{1 - \frac{\log\log n}{\log n}}}
    - \alpha_n \geq 0 .
    \label{eq:gumbel-limit-ineq}
  \end{equation}
  Since $0 \leq \eps_n \leq 2-c_1$, we have
  \begin{equation*}
    \paren{ 1 + \frac{\eps_n}{C_0} }\sqrt{1 - \frac{\eps_n}{2}}
    \leq 1 - \frac{C_0-4}{2C_0\sqrt{2c_1}} \cdot \eps_n
  \end{equation*}
  by a Taylor series argument.
  So, \eqref{eq:gumbel-limit-ineq} is implied by
  \begin{equation*}
    \frac{C_0-4}{2C_0\sqrt{2c_1}} \cdot \eps_n - T(n)
    \geq 0
  \end{equation*}
  where
  \begin{multline*}
    T(n) =
    \paren{
      \frac{\log\log n}{\log n} - \frac{x + C\log\log(n/2)}{\log n} \paren{ 1 + \frac{\log\log n}{\log n} }
    }
    \\
    \cdot
    \paren{
      \sqrt{1 - \frac{1}{\log n}} \paren{ 1 - \frac1{2d} - \sqrt{\frac{2\log n}{d}} }
    }
    .
  \end{multline*}
  Since $\eps_n \geq C_2/\sqrt{\log n}$ and $T(n) = o(1/\sqrt{\log n})$, we can choose $C_2$ large enough so that \eqref{eq:gumbel-limit-ineq} holds for all sufficiently large $n$.
\end{proof}

We conclude as in the proof of Theorem~\ref{thm:anisotropic}.
The event in which all of the following hold has probability approaching $1$ as $n\to\infty$ by combining Lemma~\ref{lem:asymptotic-lb1} and Lemma~\ref{lem:asymptotic-lb2} and a union bound:
\begin{enumerate}
  \item $\max_{i \in [m]} \abs{y_i y_{\setminus i}^\T \paren{ \bK_{\setminus i}^{-1} - \frac{1}{d} I_{n-1} } \bX_{\setminus i} \bx_i } \le \frac{\eps_{n}}{2C_0}$;

  \item $\max_{i \in [m]} \abs{\frac{1}{d} y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i} \leq \frac{\eps_{n}}{2C_0}$;

  \item $\max_{i \in [m]} \frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i \geq 1 + \frac{\eps_{n}}{C_0}$.

\end{enumerate}
In this event, there exists $i \in [m]$ such that
\begin{multline*}
  y_i y_{\setminus i}^\T \paren{\bK_{\setminus i}^{-1}-\frac{1}{d} I_{n-1}} \bX_{\setminus i} \bx_i 
  + \frac{1}{d} y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i 
  + \frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{\setminus [m]} \bx_i
  \\
  \geq 
  -\frac{\eps_n}{2C_0} - \frac{\eps_n}{2C_0} + 1 + \frac{\eps_n}{C_0} = 1 .
\end{multline*}

\subsection{Above the threshold}

Now we consider the case where the dimension is above the threshold, specifically $d = (2+\eps_n) n \log n$.

By Proposition~\ref{prop:equiv}, it suffices to show that
\begin{equation*}
  \lim_{n\to\infty} \pr{
    \exists i \in [n] \ \ \text{such that} \ \
    y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i} \bx_i \geq 1
  } = 0 .
\end{equation*}
This is implied by the following lemma combined with a union bound over all $i \in [n]$.

\begin{lemma}
  There exists $C_2>0$ and $n_0 > 0$ such that the following statement holds for all $n \geq n_0$, and all $\eps_n$ satisfying $\eps_n \geq C_2/\sqrt{\log n}$ for all $n \geq n_0$, with $d = (2+\eps_n)n\log n$:
  \begin{equation*}
    \text{for each $i \in [n]$:} \quad
    \pr{
      y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i} \bx_i \geq 1
    }
    \leq
    \frac1{2n\sqrt{\pi\log n}} + \frac1{n^2} .
  \end{equation*}
\end{lemma}
\begin{proof}
  Conditional on $\bX_{\setminus i}$ (and the probability $1$ event that $\bX_{\setminus i}$ has rank $n-1$), the distribution of
  \begin{equation*}
    y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i} \bx_i
  \end{equation*}
  is a mean-zero Gaussian with variance
  \begin{equation*}
    \sigma_i^2 := \norml[2]{y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i}}^2 = y_{\setminus i}^\T \bK_{\setminus i}^{-1}  y_{\setminus i} .
  \end{equation*}
  By Lemma~\ref{lemma:gram-evals}, we have for some absolute constant $C>0$ and sufficiently large $n$, with probability at least $1-1/n^2$,
  \begin{align*}
    \sigma_i^2
    & \leq n \cdot \mu_{\max}(\bK_{\setminus 1}^{-1})
    \\
    & \leq \frac{n}{d} \paren{ 1 + C \paren{ \sqrt{ \frac{n + 2 \log n}{d} } + \frac{n + 2 \log n}{d} } } \\
    & \leq \frac1{(2+\eps_n)\log n} \paren{ 1 + \frac{C'}{\sqrt{\log n}} } ,
  \end{align*}
  where $C'>0$ is a constant depending only on $C$.
  Let $\mathsf{E}$ be the aforementioned event.
  Then
  \begin{align}
    \pr{
      y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i} \bx_i \geq 1
    }
    & \leq
    \pr{
      y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i} \bx_i \geq 1 \mid \mathsf{E}
    } + \pr{ \neg \mathsf{E} }
    \nonumber \\
    & \leq
    1 - \Phi\paren{ \sqrt{\frac{(2+\eps_n)\log n}{1+C'/\sqrt{\log n}} } } + \frac1{n^2}
    \nonumber \\
    & \leq 
    \sqrt{\frac1{2\pi} \cdot \frac{1+C'/\sqrt{\log n}}{(2+\eps_n)\log n} }
    \exp\paren{ -\frac12 \cdot \frac{(2+\eps_n)\log n}{1+C'/\sqrt{\log n}} } + \frac1{n^2}
    \label{eq:asymp-ub}
  \end{align}
  where the final inequality follows by the Mills ratio bound (Fact~\ref{fact:mills}).
  By letting $C_2 \geq 2C'$, we have
  \begin{equation*}
    \frac{2+\eps_n}{1+C'/\sqrt{\log n}}
    \geq 2
  \end{equation*}
  (since we assume $\eps_n \geq C_2 / \sqrt{\log n}$), upon which bound in \eqref{eq:asymp-ub} is at most 
  \begin{equation*}
    \frac1{2n\sqrt{\pi\log n}} + \frac1{n^2}
  \end{equation*}
  as claimed.
\end{proof}


%\end{proof}


==> SVM NeurIPS (3)/asymptotic_proofs_old.tex <==
\section{Proofs for Section~\ref{sec:asymptotic}}\label{app:asymp-proofs}

\begin{proof}[Proof of Theorem~\ref{thm:asymptotic-lb}]
This proof is very similar to that of Theorem~\ref{thm:anisotropic}. 
Here, we let $m := \frac{n}{\log n} \leq \frac{n}{2}$.
Again, we break the argument down to three steps, which together prove the claim with Lemma~\ref{lemma:hmx-equivalence}:

\begin{enumerate}
    \item 
    By Lemma~\ref{lemma:e1} with $d_2 = d_{\infty} = d$ and $\delta := \frac{\delta}{3m}$, $\absl{y_i y_{\setminus i}^\T (\bK_{\setminus i}^{-1} - \frac{1}{d} I_{n-1}) \bX_{\setminus i} \bx_i } \leq \frac{\eps}{32}$ for all $i \in [m]$ with probability $1 - \frac{\delta}{3}$ as long as
    \[d = \Omega\paren{\frac{\sqrt{n d}}{\eps} + \frac{n}{\eps} \log \frac{1}{\delta}},\]
    which holds for sufficiently large $n$.

    \item By Lemma~\ref{lemma:e2}, $\frac{1}{d} y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i  \geq -\frac{\eps}{32}$ for all $i \in [m]$ holds with probability $1 - \frac{\delta}{3}$ as long as:
    \[d = d_{\infty} = \Omega(\frac{m}{\epsilon} \log \frac{m}{\delta})= \Omega(\frac{n}{\epsilon} \log \frac{1}{\delta})\]
    % \[n = \Omega\paren{\frac{\log{\frac{1}{\delta}}}{\epsilon^2}}.\]
    
    \item It remains to show that there exists some $i \in [m]$ such that $\frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i \geq 1 + \frac{\eps}{16}$ with probability $1- \frac{\delta}{3}$.
\end{enumerate}

The remainder of this proof shows why the third point holds. 

Observe that conditioned on $\bX_{\setminus [m]}$, $\frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i  \overset{\text{d}}{=} \sigma^{(m)} \mathbf{g}_{i}$ where $\sigma^{(m)} = \frac{1}{d} \norm[2]{y_{\setminus [m]}^\T \bX_{ \setminus [m]}}$ and $\mathbf{g}_{i}$ is a standard Gaussian.
We lower-bound the variance term with high probability. Expanding the term gives
\[\frac{1}{d^2} \norm[2]{y_{\setminus [m]}^\T \bX_{ \setminus [m]}}^2
= \frac{1}{d^2} y_{\setminus [m]}^\T \bK_{ \setminus [m]} y_{\setminus [m]}^\T
\geq \frac{n - m}{d^2} \mu_{\min}(\bK_{\setminus [m]}).\]
By Lemma~\ref{lemma:gram-evals}, $\mu_{\min}(\bK_{\setminus [m]}) \geq d(1 - c \sqrt{\fracl{(n-m)}{d}}) \geq d(1 - c \sqrt{\fracl{n}{2d}})$ with probability $1 - \frac{\delta}{6}$.
Thus, 
\[\sigma^{(m)} \geq \sqrt{\frac{(n-m)(1 - c \sqrt{\frac{n}{2d}})}{d}} \geq \sqrt{\frac{\paren{1 - \frac{1}{2\ln n}}\paren{1 -  \frac{c}{\sqrt{ \ln n}}}}{(2 - \eps) \ln n}}.\]
Similarly one can upper bound $\sigma^{(m)}$ using $\mu_{\max}(K_{\setminus [m]})$ and deduce that:
\[ \sigma^{(m)}\sqrt{2 \log(m)} \overset{\text{Pr.}}{\longrightarrow} \sqrt{\frac{2}{2-\epsilon}}
\]

Now since maximum is a 1-Lipschitz function of its input then for random variable $\bu = \max_{i \in [m]}{\frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i} \overset{\text{d}}{=} \sigma^{(m)} \max_{i \le m}{\mathbf{g}_{i}} $ we have:
\navid{This is not asymptotically sharp since it predicts constant variance for max of Gaussian, but it does the job, right?}
\[
\mathbf{P}[| \bu - \mathbf{E}[\bu \mid \bX_{\setminus [m]}] | \ge t \sigma^{(m)}  \mid  \bX_{\setminus [m]} ] \le 2 e^{\frac{-t^{2}}{2}} = \frac{\delta}{6}
\]
where $t = \sqrt{2 \log(\frac{12}{\delta})}$. Furthermore, it is a well known fact for Gaussian random variables:
\[
\lim_{m \to \infty} \frac{\mathbf{E}[\max_{i \le m}{\mathbf{g}_{i}}]}{\sqrt{2 \log(m)}} =
1
\Longrightarrow
\mathbf{E}[\bu \mid \bX_{\setminus [m]}] \overset{\text{Pr.}}{\longrightarrow} \sqrt{\frac{2}{2-\epsilon}}
\]
where the implication is based on Slutsky's Theorem. Moreover, since $t\sigma^{(m)} \overset{\text{Pr.}}{\longrightarrow} 0$ we can ensure the following event holds with probability $1-\frac{\delta}{6}$ for sufficiently large $n$:
\[
\mathbf{E}[\bu \mid \bX_{\setminus [m]}] \ge \sqrt{\frac{2}{2- \epsilon}} - \frac{\epsilon}{8} 
\ge 1 + \frac{\epsilon}{8}
\quad , \quad 
t \sigma^{(m)} \le \frac{\epsilon}{16}
\]
Combining all the above, by taking the $i \in [m]$ that realizes the maximum, then with probability at least $1 - \frac{\delta}{3}$: 
\[
    \frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i = \bu
    \geq \mathbf{E}[\bu \mid \bX_{\setminus [m]}] - t\sigma^{(m)}
    \geq 1 + \frac{\epsilon}{16}\qedhere
\]
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:asymptotic-up}]
Our goal is to show that for all $i \in [n]$, $y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i} \bx_i  < 1$.
To do so, we show that with probability at most $1 - \frac{\delta}{n}$, $y_1 y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  \bX_{\setminus 1} \bx_1  < 1$; the claim follows from a union bound.
Conditioned on $\bX_{\setminus 1}$, the quantity is a Gaussian of mean 0 and variance $\norml[2]{y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  \bX_{\setminus 1}}^2 = y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  y_{\setminus 1} \leq (n-1) \mu_{\max}(\bK_{\setminus 1}^{-1})$. 
By Lemma~\ref{lemma:gram-evals}, $\mu_{\max}(\bK_{\setminus 1}^{-1}) \leq \frac{1}{d} \paren{1 + c \sqrt{\frac{n}{d}}}$ with probability $1 - \frac{\delta}{2n}$. 
Therefore, the variance is at most 
\[\frac{n}{d} \paren{1 + c \sqrt{\frac{n}{d}}} \leq \frac{1}{(2 + \eps) \ln n} \paren{1 + c \sqrt{\frac{1}{\ln n}}}.\]
We can then upper-bound the probability that the term is no more than 1, conditioned on this variance bound for sufficiently large $n$:
\begin{align*}
    \pr{y_1 y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  \bX_{\setminus 1} \bx_1  \geq 1}
    &\leq \exp\paren{-\frac{(2 + \eps) \ln n}{2\paren{1 + c \sqrt{\frac{1}{\ln n}}}}} = n^{-\paren{\frac{1 + \fracl{\eps}{2}}{1 + c \sqrt{\frac{1}{\ln n}}}}} \leq \frac{\delta}{2n}.\qedhere
\end{align*}
\end{proof}

==> SVM NeurIPS (3)/experiments.tex <==
\section{Experimental validation of SVP phase transition and universality}\label{sec:experiments}

While Theorem~\ref{thm:asymptotic} identifies the exact SVP  phase transition for only isotropic Gaussian samples, we demonstrate experimentally that a similarly sharp cutoff occurs for a broader category of data distributions.
%While Theorem~\ref{thm:anisotropic} demonstrates that a broad class of subgaussian data distributions exhibit SVP, and Theorem~\ref{thm:asymptotic} characterizes the exact threshold boundary for the isotropic Gaussian case, we demonstrate experimentally that this sharp cutoff between support vector proliferation and non-proliferation occurs for a broad category of data distributions. 
These experiments suggest that the phase transition phenomenon extends beyond the distributions with independent subgaussian components considered in Theorem~\ref{thm:anisotropic}, and that it occurs at the same location ($d = 2 n \log n$), with the transition sharpening as $n \to \infty$.
%We further argue that the phenomenon is not limited to the setting studied in Theorem~\ref{thm:anisotropic} by showing that it holds even for non-subgaussian distributions, namely the Laplacian distribution.
%Furthermore, the phase transition for all the distributions tested occurs at the same location (when $d \approx 2 n \log n$), and the transition sharpens as $n$ and $d$ become increasingly large.

%\begin{table}[t]
%    \centering
%    \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%          Uniform & Bernoulli & Radamacher & Laplace & Gaussian & Gaussian Biased \\
%         \hline
%         Unif$[-1,1]$ & Bernoulli$(\frac{1}{2})$ & Radamacher$(\frac{1}{2})$ & Laplace$(0,1)$ & $\mathcal{N}(0,1)$ & $\mathcal{N}(1,1)$ \\
%         \hline
%    \end{tabular}
%    
%    \smallskip
%    
%    \caption{The suite of sample distributions used in the experiments.}
%    \label{tab:dist}
%\end{table}

Our simulation procedure is as follows.
We generate data sets $(\bX,y) \in \R^{n \times d} \times \flip^n$, where $y \in \flip^n$ is a fixed vector of labels with exactly $n/2$ positive labels, and $\bx_1,\dotsc,\bx_n \sim_{\text{i.i.d.}} \distr^{\otimes d}$ where $\distr$ is one of six sample distributions on $\R$.
For each data set, we check for SVP by solving the problem in~\eqref{eq:svm-restricted-primal-lp}, and checking if its solution additionally satisfies the constraints from~\eqref{eq:svm-primal-lp}.
Let $\hat\bp \coloneqq \hat\bp(n,d; \distr,M)$ denote the observed frequency of SVP in $M=400$ independent trials when $\bX \in \R^{n \times d}$ is generated using $\distr$.
(Full details are given in Appendix~\ref{app:exp-procedure}.)

Figure~\ref{fig:heatmap-different-distributions} shows a heat map of $\hat\bp(n,d; \distr,M)$ with $M=400$.
The striking similarity across the distributions suggests that SVP is a universal phenomenon for a broad class of sample distributions that vary qualitatively in different aspects: biased vs.\ unbiased, continuous vs.\ discrete, bounded vs.\ unbounded, and subgaussian vs.\ non-subgaussian.
%It suggests that the occurrence of SVP is insensitive to the distribution that samples are drawn from, so long as features have independent coordinates. 
Moreover, the boundary at which the sharp transition occurs is visibly indistinguishable across the different sample distributions.

\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.8]{unnamed-chunk-5-1.pdf}
    \caption{%
    \label{fig:heatmap-different-distributions}%
    The fraction of $M = 400$ trials where support vector proliferation occurs for $n$ samples, $d$ features, and six different sample distributions $\distr$.
    All distributions demonstrate sharp phase transitions near the theoretical boundary $n \mapsto 2n \log n$, illustrated by the red curve.} 
    % \todo{rademacher is misspelled. consider extending plots to left to show curvature of log?}}
%   \navid{corrected the spelling! Currently we are using equal aspect ratios but we can try extending the X-axis. But there isn't actually much curvature since it's only a log :-). Daniel what do you think?}\daniel{looks fine!}}
\end{figure}

%Determining the class of distributions under which the SVM proliferation property holds is an open problem and we leave it for future work. 

We also investigate the universality of SVP using statistical methodology inspired by \citet{donoho2009observed}.
Specifically, we model $\hat\bp$ using Probit regression to test our \emph{universality hypothesis}: that the occurrence of SVP for $\ell_2$-SVM on data with independent features matches the behavior under Gaussian features as $n$ and $d$ grow large.
Our model is
$M \cdot \hat\bp \sim \Binomial(p(n,d;\distr), M)$,
where
\begin{align*}
  p(n,d ; \distr)
  & = \Phi\paren{ \mu^{(0)}(n,\distr) + \mu^{(1)}(n, \distr) \times \tau + \mu^{(2)}(n,\distr) \times \log \tau  } \\
  \text{with} \quad
  \mu^{(i)}(n, \distr)
  & = \mu^{(i)}_{0}(\distr) + \frac{\mu^{(i)}_{1}(\distr)}{ \sqrt{n} } .
\end{align*}
% \todo{consider making $n$ and $\mathcal{D}$ be indices to avoid $\mu$ looking like a function.}
Here,
$\Phi(t)$ is the standard normal distribution function,
$\tau = d / (2n \log n)$,
and the model parameters are $\mu^{(i)}_0(\distr)$ and $\mu^{(i)}_1(\distr)$ for $i \in \{0,1,2\}$ and the six different distributions $\distr$ (shown in Table~\ref{tab:dist} in Appendix~\ref{app:exp-procedure}).
Figure~\ref{fig:constant-slice} visualizes the fitted Probit function $p$ for fixed $n$ and $\tau$ and demonstrates that the model provides a very accurate approximation of $\hat{\mathbf{p}}$. 

The universality hypothesis corresponds to the model in which the parameters $\mu^{(i)}_0(\distr)$ are ``tied together'' (i.e., forced to be the same) for all distributions $\distr$.
That is, only the parameters scaled down by a factor of $\sqrt{n}$, $\mu^{(i)}_1(\distr)$, are allowed to vary with $\distr$.
The scaling ensures that their effect tends to zero as $n \to \infty$.
The alternative (non-universality) hypothesis corresponds to the model in which all parameters
(both $\mu^{(i)}_0(n,\distr)$ and $\mu^{(i)}_1(n,\distr)$ for each $i$) are allowed to vary with $\distr$.
We compare the models' goodness-of-fit using analysis of deviance~\cite{hastie2017generalized}.
Our main finding is that the experimental data are consistent with the universality hypothesis (and also that we can reject a null hypothesis in which all parameters are ``tied together'' for all $\distr$).
The details and model diagnostics are given in Appendix~\ref{app-sub:universality}.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.48\textwidth]{unnamed-chunk-9-1.pdf} &
    \includegraphics[width=0.48\textwidth]{unnamed-chunk-9-2.pdf}
    \\
    (a) & (b)
    \end{tabular}
    \caption{%
    \label{fig:constant-slice}%
    Visualizations of SVP frequencies for constant slices of $n$ and $\tau$ for $d = 2\tau n \log n$.
    \emph{Left panel (a):}
    The points are $(\tau,\hat\bp)$ from the Gaussian samples, for fixing $n \in \{50,70,90\}$.
    The black vertical line corresponds to $\tau = 1$.
    The Probit model's predictions are overlaid, and shaded regions correspond to $\tau$ for which the model's predicted probabilities are between $0.1$ and $0.9$.
%    The shaded regions correspond to each slice's 0.1-transition zone. 
%    This demonstrates that $\hat{\mathbf{p}}$ is closely predicted by a Probit link function $p$, whose level curves are overlaid on the samples.
    \emph{Right panel (b):}
    The points show $(n,\Phi^{-1}(\hat\bp))$ from a Gaussian distribution, fixing $\tau$ to lie in one of 12 different intervals.
    The Probit model's predictions (averaged over all $\tau$ within an interval) are overlaid.
%    The $x$-axis is the sample count $n$ and the $y$-axis is $\Phi^{-1}(\hat{\mathbf{p}})$, the observed SVP frequency applied to the inverse of the Probit function, which is standard normal qunatile function. 
%    The $\tau$ values are grouped into small intervals to resemble a constant $\tau$ slice.
%    The trend lines overlaid are obtained from our proposed model $p$.}
}
\end{figure}

%\textbf{Universa%lity Hypothesis:} The occurrence of SVP for $\ell_{2}$-SVM under various distributions \navid{we should change this to well behaved or smt?}\clayton{``various distributions with independent components''?} matches the behaviour of SVP for Gaussian samples as $n$ and $d$ grows large.


% \clayton{Should we say something briefly about the width experiments? Maybe point people to a figure in the appendix?}

Finally, in Appendix~\ref{app-sub:width},
we provide empirical support for the generality of Remark~\ref{rmk:transition-width}, namely that the transition width is roughly $n \sqrt{\log n}$ for data models other than Gaussian ensembles. 



==> SVM NeurIPS (3)/intro.tex <==
\section{Introduction}
%\citet{muthukumar2020harmless}

The \emph{support vector machine} (SVM) and \emph{ordinary least squares} (OLS) are well-weathered approaches to fitting linear models, but they are associated with different learning tasks: classification and regression.
%and are defined by two different kinds of regularization.
In this paper, we study the case in which the models return exactly the same hypothesis for sufficiently high-dimensional data.
% This coincidence occurs if and only every training sample for the SVM is a support vector, a phenomenon we call \emph{support vector proliferation} (SVP). 

The hard-margin SVM is a linear classification model that finds the separating hyperplane that maximizes the minimum margin of error for every training sample. 
If the training data $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \flip$ are linearly separable, then the resulting linear classifier is $x \mapsto \sign{x^\T w_{\svm}}$, where $w_{\svm}$ is the solution to the following optimization problem: 
\begin{equation}\label{eq:svm-primal-l2}
    w_{\svm} = \argmin_{w \in \R^d} \norm[2]{w} \quad \text{such that} \quad y_i w^\T \bx_i \geq 1, \ \forall i \in [n].
\end{equation}
An example $\bx_i$ is a \emph{support vector} if the corresponding constraint is satisfied with equality, and the optimal solution $w_{\svm}$ is a linear combination of these support vectors.
%Although some classical generalization analyses for SVMs are based on the number of support vectors~\cite[e.g.,][]{vapnik1995nature,graepel2005pac,germain2011pac}, they become vacuous in certain high-dimensional regimes where the number of support vectors is very large.
%As a result, the generalization properties of high-dimensional support vector machines (which can be expected to have many support vectors) remain largely unknown.

Ordinary least squares regression finds the linear function that best fits the training data $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \R$ according to the sum of squared errors.
When the solution is not unique, it is natural to take the solution of minimum Euclidean norm; this is the convention we adopt.
Taking $\bX := [\bx_1 | \dots | \bx_n]^\T \in \R^{n \times d}$ and $y := (y_1, \dots, y_n)$, the solution is the hypothesis $x \mapsto w_{\ls}^\T x$ where $w_{\ls}$ is the solution to the following:
%\clayton{This isn't the right formulation, since this alone does not require that overparameterized models are norm-minimizing.}
%\begin{equation}\label{eq:ls-l2}
   $w_{\ls} = \argmin_{w \in \R^d} \norm[2]{w}$ such that
  % \quad \text{such that} \quad
  $\bX^\T \bX w = \bX^\T y$.
%    w_{\ls} = \argmin_{w \in \R^d} \norm[2]{\bX w - y}.
%\end{equation}
  In many high-dimensional settings (e.g., where $\bX$ has full row rank), the solution may in fact \emph{interpolate} the training data, i.e., %$\innerprod{w_{\ls}}{\bx_i} = y_i$ for all $i \in [n]$.
%In the high-dimensional regime where there exist many $w$ such that $\bX w = y$, the least squares problem finds the instance of $w$ with minimum norm:
\begin{equation}\label{eq:ls-l2-overparam}
    w_{\ls} = \argmin_{w \in \R^d} \norm[2]{w}  \quad \text{such that} \quad w^\T \bx_i = y_i, \ \forall i \in [n].
\end{equation}
%The generalization properties of such overparameterized least squares models that interpolate all training samples have been recently studied by \cite{bhx20,bllt20,hmrt19,muthukumar2020harmless}, among many others.
%These results demonstrate that the regularization enabled by using high-dimensional feature spaces enables favorable generalization properties and counters the long-standing narrative that interpolating models are too vulnerable to noise. 

Although the optimization problems in~\eqref{eq:svm-primal-l2} and~\eqref{eq:ls-l2-overparam} are very different,
they have been observed to coincide in very high-dimensional regimes.
The study of this \emph{support vector proliferation} (SVP) phenomenon---in which every training example is a support vector---was recently initiated by \citet{mnsbhs20} and \citet{hmx20}.
Roughly speaking, they show that SVP occurs when $d = \Omega( n \log n)$ for a broad class of sample distributions, and that SVP does not occur when $d = O(n)$ in an idealized isotropic Gaussian case.
%These results leave unanswered whether we can expect this phenomenon to occur when $d = \Theta(n)$ and how universal this phenomenon is.

SVP is a phenomenon that connects linear classification and linear regression, topics that have received renewed attention due to the break-down of classical analyses of these methods in high-dimensions.
For instance, some analyses of SVM that are based on the number of support vectors become vacuous when this number becomes large~\cite[e.g.,][]{vapnik1995nature,graepel2005pac,germain2011pac}.
Similarly, overparameterized linear regression is typically only studied in noisy settings with explicit regularization.
It was not until recently that SVM and OLS have been meaningfully analyzed in these regimes (see Section~\ref{sec:related}), and the connection between the two approaches via SVP has played an important analytical role~\cite{mnsbhs20,wang2021binary,cao2021risk}.


%Because the existence of support vector proliferation runs counter to the original motivation for the use of SVMs, where the model is expected to be defined by a very small fraction of samples.

%It also facilitates the analysis of maximum-margin solutions in high-dimensional settings, as explored in \cite{mnsbhs20,wang2021binary,cao2021risk}. \todo{say more about this}

In this work, we further examine support vector proliferation with the goal of broadly understanding when and why SVMs and OLS coincide. 
We pose and study the following questions:
\begin{enumerate}
    \item \emph{How general is the SVP phenomena? 
    What relationship between $d$ and $n$ determines if the solutions to \eqref{eq:svm-primal-l2} and \eqref{eq:ls-l2-overparam} coincide?}

    \smallskip
    We close the $\log n$ gap from the prior work of \citet{hmx20} by showing that $d \gtrsim n \log n$ is \emph{necessary} for SVP to occur under a model of independent subgaussian features, even with constant probability.
%    We strengthen the bounds of \citet{hmx20} to show that support vector proliferation occurs with high probability when $d \gg n \log n$ and \emph{does not} occur with high probability when $d \ll n \log n$.
    Our lower-bounds hold for a broad class of distributions over $\bx_i$, and they match the upper-bounds from \cite{hmx20}.
    This demonstrates that SVP is extremely unlikely to occur in the much-studied $d = \Theta(n)$ setting.

    \item \emph{Is there a sharp threshold separating the occurrence and non-occurrence of this phenomenon?
    Is this threshold universal across all ``reasonable'' distributions over each $\bx_i$?}

    \smallskip
    We hypothesize that a sharp phase transition occurs at $d = 2 n \log n$.
    We rigorously prove this hypothesis for isotropic Gaussian features and quantitatively bound the width of the transition.
    We experimentally observe the same transition for a wide range of other distributions.

    \item \emph{Is support vector proliferation specific to the $\ell_2$ SVM problem? 
    If \eqref{eq:svm-primal-l2} and \eqref{eq:ls-l2-overparam} are generalized to instead minimize $\ell_p$ norms, does this still occur at the same rate?}

    \smallskip
    We re-frame this question with a geometric characterization of the dual of the SVM optimization problem for $\ell_p$ norms.
    We conjecture that a similar phase transition occurs for $\ell_1$, but also that it requires much larger dimension $d$; this is supported by preliminary experiments.

\end{enumerate}

% \begin{enumerate}
%   \item SVM and LS are two well-weathered approaches method to fitting linear models. However, they are usually associated with two different prediction tasks (classification vs regression)
%     \begin{itemize}
%       \item (Either define SVM and LS formally here, or point to formal definitions in preliminaries section.)
%     \end{itemize}
%   \item Prior work shows that in certain data models, these two methods are likely to be equivalent in very high dimensions
%   \item (Significance)
%     \begin{itemize}
%       \item Their equivalence implies that every training example is a support vector, a phenomenon that runs counter to many of the original motivations for the use of SVMs
%       \item Technical significance: Used to facilitate analysis of max-margin solutions in very high dimensions

%     \end{itemize}
%   \item How general is this phenomenon?
%     \begin{itemize}
%       \item We show that it is a very high-dimensional phenomenon

%         \begin{itemize}
%           \item We give a tight lower-bound on the dimension in the same models as HMX
%           \item We further provide the exact phase transition in the Gaussian model
%           \item Numerical simulations \ldots
%         \end{itemize}

%       \item It is not specific to the (L2) SVM problem

%         \begin{itemize}
%           \item We give a new geometric characterization

%           \item L1 SVM: We give some analyses, simulations, conjectures \ldots

%         \end{itemize}
%     \end{itemize}

% \end{enumerate}


\subsection{Outline of our results}

Section~\ref{sec:prelim} introduces the SVM and OLS approaches in full generality, our $\lambda$-anisotropic subgaussian data model, and prior results about SVP.
Several equivalent characterizations of SVP are established (Proposition~\ref{prop:equiv}) for use in subsequent sections.
%The equivalence relies on a key technical lemma of \citet{hmx20}, but our proof of the proposition involves a different approach that relies on the geometric structure of SVP.

Section~\ref{sec:nonasymp} characterizes when SVP \emph{does not} occur for a broad range of distributions (Theorem~\ref{thm:anisotropic}).
Our lower-bound on the dimension required for SVP matches the upper-bounds from \cite{hmx20} in the isotropic Gaussian setting, resolving the open question from that work, and also gives new lower-bounds for anisotropic cases.
%Theorem~\ref{thm:anisotropic} does so by showing that SVP is very unlikely to occur when $d = O(n \log n)$ if the samples have independent subgaussian components. 
%($d_2$ is a dimension proxy that depends on the relative variances of each component of the random variable.)
%This sharply improves upon the lower-bounds of \citet{hmx20} (Theorem~\ref{thm:hmx-lb}), which hold with high probability only for spherical Gaussian samples when $d = O(n)$.
The proof works by tightly controlling the spectrum of the Gram matrix and establishing anti-concentration via the Berry-Esseen Theorem.

Section~\ref{sec:asymptotic} establishes a sharp threshold of $d = 2 n \ln n$ for SVP in the case of isotropic Gaussian samples, and also characterize the width of the phase transition (Theorem~\ref{thm:asymptotic}).
%Theorem~\ref{thm:asymptotic} also proves that the width of the phase transition decreases as $n$ and $d$ approach infinity.
%We consider only the spherical Gaussian case, where each $\bx_i$ is drawn from $\mathcal{N}(0, I_d)$.

Section~\ref{sec:experiments} provides empirical evidence that the sharp threshold observed in Section~\ref{sec:asymptotic} holds for a wide range of random variables.
%Indeed, even random variables with too heavy tails to be subgaussian (such as Laplacian random variables) demonstrate a sharp SVP threshold.
Rigorous statistical methodology inspired by
\citet{donoho2009observed} is used to test our ``universality hypothesis'' that the probability of SVP does not depend on the underlying sample distribution as $d$ and $n$ become large.

Section~\ref{sec:l1} asks the questions about SVP from the preceding sections in the context of $\ell_1$-SVM and minimum $\ell_1$-norm interpolation.
Specifically, the SVP threshold for $\ell_1$ is conjectured to occur for $d = \omega(n \log n)$.
Evidence for this conjecture is provided in a simulation study and in geometric arguments about random linear programs.
%We support this conjecture with empirical results and hypothesize that the conjecture could be resolved by studying the problem from a geometric lens and drawing on work about random linear programs. 

% \todo{
% - We characterize the phase transition in SV proliferation for high-dimensional SVMs; we found a sharp cut-off that holds up empirically and theoretically

% - We give lower-bounds that are tight with upper-bounds of \cite{hmx20} in same setting (subgaussian independent RVs, anisotropic) -- more general and tigther than LBs from their paper; extensions to general kernels?

% - We find the exact asymptotic rate of phase transition for Gaussian RV case

% - We find experimentally that this phase transition is sharp for small values of $n$ and $d$. Our experiments also suggest a universality that goes beyond subgaussian random variables

% - We examine a similar problem for $\ell_1$ SVM and experimentally find a different rate. We pose a tight characterization of this rate as an open problem
% }

\subsection{Related work}
\label{sec:related}

% \todo{Edit and integrate the following elaboration promised to reviewer FQDN: ``As we discussed in Section 1.2, the coincidence between SVM and OLS was already used in recent works to analyze linear classification in very high dimensions under different data distributions. For example, in [33], the authors studied a data model inspired by the spiked covariance model of Wang and Fan (2017), and they identified a regime of overparameterization where the hard-margin SVM classifier has good generalization behavior (i.e., classification risk going to 0) even when all training examples are support vectors. (Their result was strengthened by an improved characterization of SVP in [23].) Our new lower-bound (Theorem 3) can be viewed as establishing a limit on this approach to the analysis of SVM; specifically, if the (effective) dimension is not sufficiently large, the OLS and SVM solutions may not coincide.''}\clayton{ok?}

\paragraph{Prior works connecting SVP and generalization.}

\citet{mnsbhs20} initiate the study of SVP in part to facilitate generalization analysis of the SVM in very high-dimensional settings.
Their work, as well as the contemporaneous work of \citet{cl20}, shows that the SVM enjoys low test error in certain regimes where classical learning-theoretic analyses would otherwise yield vacuous error bounds.
(In fact, one of the settings in \cite{cl20} requires polynomially-higher dimension than is typically studied: $d = \Omega(n^2\log n)$.)
The coincidence between SVM and OLS identified by \citeauthor{mnsbhs20} was also more recently used by \citet{wang2021binary} and \citet{cao2021risk} for analyses of linear classification in very high dimensions under different data distributions.

The generalization analysis of \citeauthor{mnsbhs20} concerns a data model inspired by the spiked covariance model of \citet{wang2017asymptotics}.
They identify a regime of overparameterization where the hard-margin SVM classifier has good generalization (i.e., classification risk going to 0) even when all the training samples are supoort vectors. Our new lower bound can be regarded as establishing a limit on this approach to the analysis of SVM; specifically, if the (effective) dimension is not sufficiently large, the OLS and SVM solutions may not coincide.

\paragraph{Prior analyses of number of support vectors.}
Besides its relevance to generalization analysis, the number of support vectors in an SVM model is an interesting quantity to study in its own right.
\citet{hmx20} sharpen and extend the analysis of \citet{mnsbhs20} about SVP in the independent features model that we also adopt.
They prove that SVM on $n$ samples with $d$ independent subgaussian components coincides with OLS when $d = \Omega(n \log n)$ with probability tending to $1$.
They also give a converse result stating that the coincidence fails with constant probability when $d = O(n)$ in the isotropic Gaussian feature model.
(We give these results here as Theorems~\ref{thm:hmx-ub} and \ref{thm:hmx-lb} respectively.)
Our results generalize and tighten the latter bound to tell an asymptotically sharp story about the phase transition for both isotropic and anisotropic random vectors with subgaussian components.
Our specific analysis for the isotropic Gaussian case gives the exact point of the phase transition.

The number of support vectors is also studied in the context of variants of SVM~\cite{steinwart2003sparseness,bartlett2007sparseness}, including the soft-margin SVM~\cite{cortes1995support} and the $\nu$-SVM~\cite{scholkopf2000new}.
% However, these are primarily relevant for non-separable (noisy) data, whereas the setups we study are linearly separable.
% ^ swapped out above sentence based on reviews
In these cases, the asymptotic number of support vectors is shown to be related to the noise rate in the problem. The setups we study are linearly separable, which makes it possible to study the hard-margin SVM (without regularization).
%\purple{While the popularity of SVMs has diminished in the era of deep neural networks, they remain an object of theoretical interest because other models have implicit biases that favor hard-margin solutions; indeed, the iterates of gradient descent on the logistic loss objective for linear predictors converge to the hard-margin SVM solution \cite{shmgs18,ji2019implicit}.}
The hard-margin SVM is also of interest because it captures the implicit bias of gradient descent on the logistic loss objective for linear predictors~\cite{shmgs18,ji2019implicit}.

% \todo{Incorporate motivation for hinge loss: ``The iterates of gradient descent on the logistic loss objective for linear predictors converge to the hard-margin SVM solution, which makes the hard-margin SVM an object of interest even if one does not directly use hinge loss. See, for instance, "The implicit bias of gradient descent on separable data" by Soudry et al (2017).''}\clayton{ok?}

%\citet{mnsbhs20} also study the coincidence between SVMs and OLS methods in high-dimensional regimes; like \cite{hmx20}, they focus on exhibiting \emph{necessary} conditions for support vector proliferation instead of the \emph{sufficient} conditions focused on in this paper.
%Furthermore, our asymptotic results in Section~\ref{sec:asymptotic} obtain the exact threshold where the phenomenon begins to occur for large $n$ with the idealized model with isotropic Gaussian features, which improves upon the second part of their Theorem~1.
%They also prove that in some circumstances, the equivalence between very high-dimensional SVMs and LS gives favorable generalization properties for classification with SVMs, which differ from tradition SVM generalization bounds that mandate that few training samples be support vectors.

Phase transitions have been studied in the context of linear classification~\cite{cover1965geometrical,theisen2021good,candes2018phase,liang2020precise}, and SVMs in particular~\cite{dietrich1999statistical,malzahn2005statistical,liu2019exact,bg01}, but most study qualitative changes in behavior other than support vector proliferation.
The most relevant is the study of \citet{bg01}, who employ techniques from statistical physics to show the existence of phase transitions for the generalization error, margin size, and number of support vectors as $n$ and $d = \Theta(n)$ become arbitrarily large.
While they characterize the fraction of samples that are support vectors, they do not address our question about when \emph{all} samples are support vectors, not just a large fraction.
Indeed, our results demonstrate that their regime where $d$ grows linearly with $n$ will not exhibit support vector proliferation when $n$ and $d$ in the limit.

%Other recent work studies generalization in very high-dimensional regimes for SVMs.
%\citet{cl20} demonstrates empirically and theoretically that SVMs enjoy good generalization properties when classical learning theoretic analyses provide vacuous bounds. 
%They inhabit an even higher-dimension regime than we do, where $d = \Omega(n^2 \log n).$
%\citet{wang2021binary} and \citet{cao2021risk} also prove generalization bounds in even higher-dimensional regimes by combining the support vector proliferation bounds from \cite{mnsbhs20} with generalization bounds on minimum norm interpolation.

%\purple{Our results are directly applicable to settings with anisotropic subgaussian data distributions, where certain \emph{effective dimensions} completely take the place of the ambient dimension.
%  These same effective dimensions were empirically evaluated by \cite{hmx20} in some examples involving infinite-dimensional spaces induced by kernels, and they were found to inform the occurrence of SVP in those cases.
%  While our theoretical analyses do not directly apply in those examples, related notions of effective dimensions have played important roles in the study of interpolating kernel methods in certain asymptotic analyses~\cite{lrz19,lr20}.%
%%However, our notions of \textit{effective dimensionality} allows the phenomenon of SVP to be analyzed for (potentially infinite-dimensional) feature mappings with kernel matrices whose spectra can be bounded.
%%For instance, the effective dimensions $d_2$ and $d_\infty$ are analyzed and evaluated empirically by \citet{hmx20}, and these effective dimensions are shown to inform the occurrence of SVP in those settings.
%%The effective dimensions of various kernels can occasionally be characterized precisely by exact computation of the eigenvalues, for instance in the analysis of the Gaussian kernel on the sphere \cite{mny06}.
%%Because we show that SVP occurs when the effective dimension is substantially larger than the number of samples, a kernel must be tuned in such a way that its effective dimension increases as $n$ grows. 
%%Two ways to do so are to reduce the width of the kernel as $n$ grows or to increase the input dimension $d$ of the kernel.
%%These relationships between the dimension of a feature space and the effective dimensionality of its kernel are explored in the literature \cite{lrz19, lr20}.
%}

%\todo{Connect to results about effective dimensions of kernels mentioned by CcT8: \url{https://link.springer.com/content/pdf/10.1007/11776420_14.pdf}, \url{https://arxiv.org/abs/1808.00387}, \url{https://arxiv.org/abs/1908.10292}}\clayton{ok?}
%\daniel{are these in the $d \propto n$ asymptotic regime?}

\paragraph{Overparameterized linear regression.}
There has been a recent flurry of analyses of overparameterized linear regression models~ \cite[e.g.,][]{bhx20,bllt20,hmrt19,muthukumar2020harmless,mei2019generalization,mitra2019understanding,wang2017asymptotics,mahdaviyeh2019risk,mnsbhs20,xu2019number,huang2020dimensionality}.
Many of these analyses are carried out in the $d = \Theta(n)$ asymptotic regime, whereas our work studies a phase transition that occurs in a much higher-dimensional regime.
The notions of effective dimensions we use are present in the analyses of \citet{bllt20} and \citet{mnsbhs20}, and the latter work identifies regimes where SVM and OLS coincide and enjoy good performance for both classification and regression.

%however, the equivalence between solutions to linear regression and SVM classification may permit a similar generalization analysis of SVMs that perform interpolation, even when subject to noise.

\paragraph{High-dimensional geometry and universality.}
Our conjecture about support vector proliferation for $\ell_1$-SVMs derives inspiration from studies of high-dimensional geometric phase transitions, particularly those by \cite{ab12, almt14, donoho2009counting}.
These results consider the geometry of random polytopes.
\citet{ab12} establish phase transitions on the feasibility and boundedness of the solutions to random linear programs, \citet{almt14} extend these results to characterize when $\ell_1$-norm minimizing solutions to sparse recovery problems are exactly correct, and \citet{donoho2009counting} bound the number of faces of random polytopes. 
We also borrow heavily from \cite{donoho2009observed} when designing our experiments in Section~\ref{sec:experiments} to test the universality hypothesis.


% \todo{L1 regularization with interpolating linear regression: \url{https://arxiv.org/abs/1903.09139}. (What about linear classification?)}


%\todo{other linear classification stuff: \url{http://proceedings.mlr.press/v130/theisen21a.html}}

==> SVM NeurIPS (3)/junk.tex <==
\subsection{Junk Yard}
\navid{we should put more emphasis on this sentence I think} Note that we disregard the instances when the observed success rates are degenerate, that is there is ambiguity in defining Z-scores. We resolve this issue by restricting our attention to a narrower range of $n,d$. More precisely, we restrict $\tau \coloneqq \fracl{d}{\paren{2n\log n}}$ to be in the range [0.4,1.6] which will induce a negligible \navid{how should I argue here?} bias into our analysis. Unfortunately, this issue cannot be avoided by increasing the simulation size since actual probabilities of the desired events might be either exponentially small or exponentially close to one for some $n,d$ in our simulation range (see Theorem~\ref{thm:hmx-ub},\ref{thm:anisotropic}). 

As described in Section~\ref{sec:experiments} we attempt to show universality by computing Z-scores which assesses whether the underlying probability for which observed success rates are generated from are equal or not. More precisely, for distributions $\distr_{1}, \distr_{2}$ let us abbreviate $\hat{\mathbf{p}}_{1} = \hat{\mathbf{p}}(n,d; \distr_{1},M) ,\hat{\mathbf{p}}_{2} = \hat{\mathbf{p}}(n,d; \distr_{2},M)$ to be the observed success rates.
Therefore we can compute Z-scores between distributions using the following formula:
\[ 
\bZ (n,d; M,\distr) = \frac{\hat{\mathbf{p}}_{2} - \hat{\mathbf{p}}_{1}}{ \sqrt{ \frac{\paren{\hat{\mathbf{p}}_{2} + \hat{\mathbf{p}}_{1}} \paren{2 - \paren{\hat{\mathbf{p}}_{2} + \hat{\mathbf{p}}_{1}} } }{8 M} } }.
\]
In our analysis we fix $\distr_{1}$ to be the Gaussian ensemble. Under the null hypothesis of indifference between distributions for each $n,d$ one expects Z-scores to follow a standard normal distribution for large values of $M$. However, It might be naive to expect such hypothesis to hold true since phenomena at hand is an asymptotic statement and decaying deviations from the asymptotic behaviour should be expected non-asymptotically. Therefore, inspired by \cite{donoho2009observed} we instead form the following null-hypothesis and provide evidence for its significance. \navid{not sure whether we should say we don't reject this hypothesis or we show it's significance.}

\textbf{Universality Hypothesis:} For each $n,d$, Z-scores (defined above) follows a $\mathcal{N}\paren{\mu\paren{n, d; \distr},1}$ distribution where the mean decays to zero as $n, d$ grows large.

\begin{figure}[h]
    \begin{minipage}{\textwidth}
        \begin{minipage}{0.48\linewidth}
                \centering
                \includegraphics[width=\textwidth]{unnamed-chunk-10-1.pdf}
        \end{minipage}
        \hfill
        \begin{minipage}{0.48\linewidth}
                \centering
                \includegraphics[width=\textwidth]{unnamed-chunk-10-2.pdf}
        \end{minipage}
        \label{table:Z-scores}
        \caption{Comparing bulk distribution of Z-scores for suite of non-Gaussian distributions with Gaussian Ensemble. Note that white region corresponds to $\tau \notin [0.6,1.4]$ were Z-scores are ill-defined. \navid{Last sentence feel a bit ambiguous.}
        \clayton{These plots should be bigger. Maybe each needs their own figure?
        I'm also not very sure what the desired take-away here should be.}
        }
    \end{minipage}
\end{figure}

==> SVM NeurIPS (3)/l1.tex <==
\section{SVP phase transition for $\ell_1$-SVMs?}\label{sec:l1}
Because both the SVM and linear regression problems can be formulated for general $\ell_p$-norms, we can ask similar questions about when their solutions coincide.
Here, we examine the $\ell_1$ case: the coincidence of SVM with an $\ell_1$-penalty and $\ell_1$-norm minimizing interpolation (also called Basis Pursuit~\cite{chen1994basis}).
Linear models with $\ell_1$ regularization are often motivated by the desire for sparse weight vectors~\cite[e.g.,][]{chen1994basis,tibshirani1996regression,ng2004feature,muthukumar2020harmless}.
%\todo{Add citations for sparsity properties of $\ell_1$ regression. Are \cite{donoho2009counting} and \cite{almt14} appropriate?}
%If SVP occurs for $\ell_1$, then sparsity properties for $\ell_1$ linear regression may be inherited by $\ell_1$-SVMs (and vice versa).

Based on experimental evidence and the differences in high-dimensional geometry between $\ell_{\infty}$ and $\ell_2$ balls, we conjecture that SVP for $\ell_1$-SVMs only occurs in a much higher-dimensional regime.
\begin{conjecture}\label{main-conjecture}
% Let $\bA \in \mathbb{R}^{d \times n}$ be a Gaussian ensemble. 
  Let $(\bX,y) \in \R^{n \times d} \times \R^n$ be an isotropic Gaussian sample. 
Then, the probability of SVP occurring for an $\ell_{1}$-SVM with $\bX$ and $y$ undergoes a phase transition around $d = f(n)$, for some $f(n) = \omega(n \log n)$. Formally, there exist positive constants $c$ and $c'$ with $c \leq c'$ such that
\[
\lim_{n \to \infty} \pr{ \text{SVP occurs for $\ell_{1}$-SVM} } = \begin{cases}
  0  &  \text{if $d < c f(n)$} , \\
  1 &  \text{if $d > c' f(n)$} .
\end{cases} \]
\end{conjecture}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{unnamed-chunk-7-1.pdf}
    \caption{
    % Observed success rate of $\ell_{1}$-SVM compared to $\ell_{2}$ for various values of $n$ and $d$. %$\ell_{1}$-SVM proliferation requires much higher dimensions and the cut off seems wider than $\ell_{2}$ variant.
    The observed probabilities of support vector proliferation for $\ell_1$- and $\ell_2$-SVMs for $d$-dimensional isotropic Gaussian samples of size $n$. 
    }
    \label{fig:l1-l2-compare}
\end{figure}

Conjecture~\ref{main-conjecture} is consistent with our preliminary experimental findings, summarized in Figure~\ref{fig:l1-l2-compare}.
It shows larger values of $d$ relative to $n$ are needed to ensure SVP for $\ell_1$-SVMs and that the transition appears to be less sharp.
% This conjecture---if true---rejects the idea that $\Theta(n \log n)$ is a ``magic threshold'' that always separates high-dimensional regimes where SVMs and linear regression algorithms coincide from more standard regimes where they do not. \daniel{i would omit this first sentence, since i don't really know of $n \log n$ would've been considered by anyone as a magic threshold -- where else has it appeared?}
Indeed, the experiments indicate that the true phase transition may occur when $d$ is asymptotically \emph{much} larger than $n \log n$.
They do not rule out the possibility that the transition may even require $d = \exp(\Omega(n))$.
Further experimental details are given in Appendix~\ref{app-sub:l1-exp}.



%While it is impossible to ascertain an asymptotically precise of phase transition for the $\ell_1$ case without testing even larger values of $d$, the experiments exhibit a clear gap between $\ell_1$ and $\ell_2$, and suggest that the rate for $\ell_1$ may be exponential in $n$.
%Moreover, the transition appears to be wider and less sharp in the $\ell_1$ case.
%The experimental procedure for optimizing $\ell_1$ SVMs is described in Appendix~\ref{app-sub:l1-exp}.

% Based on View~\ref{itm:Q1} outlined in Section \ref{sec:prelim}, we are interested in determining whether the optimal solution to \eqref{eq:svm-restricted-dual-lp} problem lies in the positive orthant or not. 
Answering whether support vector proliferation occurs in the $\ell_1$ case is equivalent to determining whether the optimal solution $\alpha^*$ to \eqref{eq:svm-restricted-dual-lp} problem lies in the positive orthant $\R_+^n$.\footnote{While Proposition~\ref{prop:equiv} does not imply this equivalence for $\ell_1$-SVMs for arbitrary data, the results of the proposition are valid for isotropic Gaussian samples, because the corresponding $\ell_\infty$ projection $\proj$ in those cases is well-defined almost surely.}
In the $\ell_{1}$ case, we have $q = \infty$, so solving the problem amounts to characterizing the solutions to the following linear program for data matrix $\bA =\diag(y) \bX \in \R^{n \times d}$:
\begin{equation}
    \tag{Dual L1}
    \label{eq:svm-dual-l1}
    \begin{aligned}
    \max_{\alpha \in \R^n} & \quad \sum_{i=1}^{n}{\alpha_{i}}
    &
    \text{s.t.} & \quad -\mathbf{1} \leq  \bA^\T \alpha \leq \mathbf{1}.
    \end{aligned}
\end{equation}
There is a line of work that gives high probability guarantees about whether related random linear programs are feasible and where their solutions reside~\cite{ab12, almt14}.
Similar analyses of random linear programs may be useful for understanding how large $d$ must be to have $\alpha^* \in \R^n_+$, and we carry out a preliminary characterization in Appendix~\ref{app:l1}. 

Conjecture~\ref{main-conjecture} and the other questions raised in this work point to a broader scope of investigations about high-dimensional phenomena and universality concerning optimization problems commonly used in machine learning and statistics.
Our results, along with those from prior works, provide new analytic and empirical approaches that may prove useful in tackling these questions.

%We believe that further work in this space could resolve Conjecture~\ref{main-conjecture} and complement our detailed understanding of SVP for $\ell_2$-SVMs.
%While the previous sections of this paper demonstrate that some degree of universality exists for SVP in the $\ell_2$ setting, our experiments suggest that there is a more complex geometric story to be told by investigating when broader classes of SVMs and linear regression models coincide.
%\clayton{Is this ok? I don't love it}
% \clayton{Let's have a nice little sentence here to conclude things: optimism about how $\ell_1$ results can be used to complete the $\ell_2$ picture we paint here.}

% A rather intuitive justification can be given based on View \ref{itm:Q2}. Observe that $\bT^{+}$ (convex hull of rows of $\bA$) bluh bluh...
% \clayton{Navid, could you write out this paragraph? I'm not entirely sure what to say here. It would be great if this could say something about $\ell_q$}


==> SVM NeurIPS (3)/nonasymptotic.tex <==
\section{SVP threshold for anisotropic subgaussian samples}\label{sec:nonasymp}


% \todo{
% summarize argument: 
% (1) use Lemma~\ref{lemma:hmx-equivalence} for SVM equivalence, (2) show that $K \approx I_n$ for sufficiently large $d$ and $n$, (3) use anti-concentration properties/CLT to show lower-bound maximum WHP

% realistically, the proof will be kicked to the appendix}

We closely characterize when support vector proliferation does and does not occur through the following theorem, which serves as a converse to Theorem~\ref{thm:hmx-ub}.



\begin{restatable}[Lower-bound on SVP threshold for anisotropic subgaussians]{theorem}{thmanisotropic}\label{thm:anisotropic}
    Consider a $\lambda$-anisotropic subgaussian sample $(\bX,y)$ and any $\delta \in (0, \half)$.
	For absolute constants $\Ca, \Cb, \Cc, \Cd$, assume that $\lambda$ and $n$ satisfy
\begin{equation}\label{eq:3}
	  n \geq \Ca \paren{\log \frac{1}{\delta}}^2, \quad d_2 \leq \Cb n \log n, \quad
	  d_{\infty} \geq \Cc n \log\frac{1}{\delta}, \quad \text{and} \quad
	  d_{\infty}^2 \geq  \Cd d_2 n.
	 \end{equation}
	Then, SVP occurs for $\ell_2$-SVM with probability at most $\delta$.
\end{restatable}

% \todo{remark that general covariance matrices work instead}

% \todo{mention that other variance proxies of subgaussianity work too}

% \clayton{How's this?}
% \daniel{did some minor edit; looks good.}

\begin{remark}
    If each $\bx_i$ is drawn from a Gaussian distribution, then we could instead permit $\bx_i$ to have any positive semi-definite covariance matrix $\Sigma \in \R^{d \times d}$ with eigenvalues $\lambda_1, \dots, \lambda_d$ due to rotational invariance.
\end{remark}
\begin{remark}
    In addition, the result can be generalized to subgaussian $\bx_i$ with general variance proxies $\gamma\geq1$. We present the current version for the sake of simplicity and note that the generalization is straightforward. 
\end{remark}

% \begin{theorem}[Lower-bound on SVP threshold for anisotropic subgaussians]\label{thm:anisotropic}
%     Consider a $\lambda$-anisotropic subgaussian sample $(\bX,y)$ and any $\delta \in (0, \half)$.
% 	For absolute constants $\Ca, \Cb, \Cc, \Cd$, assume that $\lambda$ and $n$ satisfy
% \begin{equation}\label{eq:3}
% 	  n \geq \Ca \paren{\log \frac{1}{\delta}}^2, \quad d_2 \leq \Cb n \log n, \quad
% 	  d_{\infty} \geq \Cc n \log\frac{1}{\delta}, \quad \text{and} \quad
% 	  d_{\infty}^2 \geq  \Cd d_2 n.
% 	 \end{equation}
% 	Then, SVP occurs for $\ell_2$-SVM with probability at most $\delta$.
% \end{theorem}
In the case where $(\bX,y)$ is an isotropic subgaussian sample, Theorem~\ref{thm:anisotropic} and Theorem~\ref{thm:hmx-ub} (from \cite{hmx20}) together establish that the threshold for SVP occurs at $d = \Theta(n \log n)$. 
Theorem~\ref{thm:anisotropic} sharpens and generalizes the partial converse of \cite{hmx20} given in Theorem~\ref{thm:hmx-lb}.

Theorem~\ref{thm:anisotropic} does not depend explicitly on the ambient dimension $d$; instead, it only involves the effective dimension proxies $d_2$ and $d_\infty$, which can be finite even if $d$ is infinite.
Thus, the result readily extends to infinite-dimensional Hilbert spaces.

We prove the theorem in Appendix~\ref{app:lemmas} and briefly summarize the techniques here.
%\navid{Here maybe just say $K$ is invertible?}
By Proposition~\ref{prop:equiv}, it suffices to show that with probability $1 - \delta$, $\bK$ is invertible and
\begin{equation}\label{eq:1}
\max_{i \in [n]} y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \bx_i \geq 1,
\end{equation}
where $\bK_{\setminus i} := \bX_{\setminus i} \bX_{\setminus i}^\T$.
This same equivalence underlies the proof of Theorem~\ref{thm:hmx-lb} in \cite{hmx20}.
However, their application of this equivalence is limited because they avoid issues of dependence between random variables by instead lower-bounding the probability that $y_1 y_{\setminus 1}^\T \bK_{\setminus 1}^{-1} \bX_{\setminus 1} \bx_1 \geq 1$.
This forces their bound to hold only when $d = O(n)$.
We obtain a tighter bound by separating the first $m$ samples (denoted $\bX_{[m]}$) for some carefully chosen $m$ and relating the term to the maximum of $m$ independent random variables.
To do so, we lower-bound the left-hand side of \eqref{eq:1} with the following decomposition:
\[\max_{i \in [m]} \bracket{y_i y_{\setminus i}^\T \paren{\bK_{\setminus i}^{-1}-\frac{1}{\norm[1]{\lambda}} I_{n-1}} \bX_{\setminus i} \bx_i + \frac{1}{\norm[1]{\lambda}}y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i + \frac{1}{\norm[1]{\lambda}}y_i y_{\setminus [m]}^\T \bX_{\setminus [m]} \bx_i}.\]

We prove that this decomposition (and hence, also \eqref{eq:1}) is at least 1 with probability $1-\delta$ by lower-bounding the three terms with Lemmas~\ref{lemma:e1}, \ref{lemma:e2}, and \ref{lemma:e3} (given in Appendix~\ref{app:lemmas}).
We bound the first two terms for all $i\in [m]$ by employing standard concentration bounds for subgaussian and subexponential random variables and by tightly controlling the spectrum of $\bK_{\setminus i}$.
To bound the third term, we relate the quantity for each $i \in [m]$ to an independent univariate Gaussian with the Berry-Esseen theorem and apply standard lower-bounds on the maximum of $m$ independent Gaussians.

% We enforce that $m \leq \frac{n}{\ln n} \leq \frac{n}{2}$ by requiring that $d_2 \leq \frac{1}{576} n \ln n \leq \frac{1}{288} n(\ln n - \ln\ln n)$.

The assumptions in \eqref{eq:3} are all intuitive and necessary for our arguments.
The first assumption ensures that enough samples are drawn for high-probability concentration bounds to exist over collections of $n$ variables.
The second assumption guarantees the sub-sample size $m$ is sufficiently large to have predictable statistical properties; this is asymptotically tight with its counterpart in Theorem~\ref{thm:hmx-ub} up to a factor of $\log \frac{1}{\delta}$.
The third ensures that the variance of each $y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \bx_i$ term is sufficiently small.
The fourth assumption rules out $\lambda$-anisotropic subgaussian distributions with $\norml[2]{\lambda}^2 \ll \norml[\infty]{\lambda}^2 n$, where a single component of each $\bx_i$ is disproportionately large relative to others and causes unfavorable anti-concentration properties.



% \navid{
% Maybe it would be more readable to start by decomposing each term  
% $X = X_{1} + X_{2} + X_{3}$ and then explain what the contribution of each term is in broken down steps?
% }



==> SVM NeurIPS (3)/notes.tex <==
\todo{
\section*{Todo/things to resolve:}
\begin{itemize}
    \item For all-zero vectors, $\vec{0}, \mathbf{0}, 0$? \clayton{vote for $\vec{0}$}
    \item Standardize matrix row notation. ($\bA_{i,:}, \bA_{\cdot, j},$ etc.) \clayton{$\bA_i$ is the $i$th row, $\bA_{\cdot, j}$ is the $j$th column}
    % \item Standardize how we do citations: e.g. is it okay for say something like ``\cite{bhx20} proves \dots''? Also, if we do so, should we treat ``\cite{bhx}'' as singular or plural?
    \item What should we do about labels $y$ that depend on $\bX$? We could add a theorem for the case where $y$ corresponds to a true linear separator, but that might add unnecessary complexity 
    \clayton{mention briefly in intro}
    \item Numbered equations vs named equations? \clayton{New rule: important things that are referred to in different sections are named; less important equations are named}
    \item When referring to an equation, should we say ``Equation~\eqref{eq:3},'' ``equation~\eqref{eq:3},'' or ``\eqref{eq:3}?''
    \item When we prove things in the appendix, should we repeat the theorem there? \clayton{Hold off for now}
    \item Unify what we're calling samples (isotropic gaussian vs gaussian ensemble) \clayton{Sample = $(\bX, y)$, ensemble = $\bA$}
    \item Standardize $\ell_p$ SVMs and $\ell_q$ SVMs
    \item Be more consistent about $\bA$ and $\bX$. \clayton{Keep $\bA$ and $\bX$ separate, but take transpose of $\bA$ so that both $n \times d$.}
    \item Standardize $\R_+^d$, $\R_{\geq 0}^d$, $\text{int}(\R_+^d)$. \clayton{1 and 3, define int in intro}
    \item When do we use present vs past tense for discussing papers?
    \item $\log$ vs $\ln$ consistency \clayton{$\log$ everywhere, mention in notation that it's natural log}
\end{itemize}

}

==> SVM NeurIPS (3)/prelim-proofs.tex <==
\section{Proofs for Section~\ref{sec:prelim}}\label{app:prelim-proof}

\newcommand\lesscrazyparagraph[1]{\paragraph{\mbox{#1}}}

We restate and prove Proposition~\ref{prop:equiv}.


\propequiv*

\begin{proof}%[Proof of Proposition~\ref{prop:equiv}]
  The proof henceforth proceeds under the assumption that $\bK$ is invertible.
  Since $\bK$ is symmetric, the invertibility of $\bK$ implies that all of its principal minors (i.e., the $\bK_{\setminus i}$'s) are invertible.
%   \todo{Change this: PSD of $K$ implies invertibility of all principal minors of $K$. \navid{\checkmark}}

The equivalences between the first four statements follow from simple implications of the definition of support vector proliferation and the derivation of the dual optimization problems to \eqref{eq:svm-primal-lp} and \eqref{eq:svm-restricted-primal-lp}.
Lemma~1 of \cite{hmx20} proves the equivalence between (1) and (5) for the $\ell_2$ case and completes the argument.
We supplement the argument with an additional equivalence between (4) and (5) to show how the ``leave-one-out terms'' in (5) can be intuitively understood through the geometric framing of the dual problem.

\lesscrazyparagraph{(1) $\iff$ (2):}
This is immediate from the fact that the definition of SVP corresponds exactly to the equality constraints that are present in \eqref{eq:svm-restricted-primal-lp} and not in \eqref{eq:svm-primal-lp}.

\lesscrazyparagraph{(2) $\iff$ (3):}
%\sloppy
This equivalence follows by deriving the duals of the two optimization problems, \eqref{eq:svm-restricted-primal-lp} and \eqref{eq:svm-primal-lp}, and by noting that the only difference between the corresponding duals is that the latter has an additional requirement that $\alpha \in\R_+^d$.
%\fussy

By adding Lagrange multipliers $\alpha \in \mathbb{R}^{n}$, we obtain the dual of \eqref{eq:svm-restricted-primal-lp}:
\[
\max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} + \min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} -  w^\T \sum_{i=1}^{n}{\alpha_{i}y_{i}\bx_{i} }}.
\]
By Holder's inequality, if we take $q$ to be the dual of $p$ (i.e. $\frac{1}{p} + \frac{1}{q} = 1$), then $|w^\T u| \le \|w\|_{p} \|u\|_{q}$, with equality when $|u_{i}|^{q}$ is proportional to $|w_{i}|^{p}$.
Therefore,
\[\min_{w \in \mathbb{R}^{d}}  \|w\|_{p} - w^\T u = 
\begin{cases}
0 & \|u\|_{q} \le 1 \\
-\infty & \text{otherwise.}\\
\end{cases}
\]

We further denote $\bA =  \diag(y) \bX  \in \mathbb{R}^{n \times d}$, whose $i$th row is $y_{i}\bx_{i}$. We conclude that the dual of the optimization problem \eqref{eq:svm-restricted-primal-lp} is exactly \eqref{eq:svm-restricted-dual-lp}.
We similarly find that the dual of \eqref{eq:svm-primal-lp} is
\begin{equation*}\label{eq:svm-dual-lp}\tag{SVM Dual}
    \max_{\alpha \in \mathbb{R}^{n}_+} \sum_{i=1}^{n}{\alpha_{i}} \quad
    \text{such that}  \quad \|\bA^\T \alpha \|_{q} \le 1 .
\end{equation*}

Because \eqref{eq:svm-restricted-dual-lp} and \eqref{eq:svm-dual-lp} coincide if and only if the $\alpha$ that solves the former is in the positive orthant ($\alpha \in \R^d_+$), the equivalence follows.

\lesscrazyparagraph{(3) $\iff$ (4):} 
We reconfigure \eqref{eq:svm-restricted-dual-lp} to rewrite the optimization problem as a projection.
Let $\Pi_{\bT}$ and $\Pi_{\bT^+}$ be the $\ell_q$-norm minimizing projection operators onto $\bT$ and $\bT^+$, which are uniquely defined when $\bK$ is invertible. % (which we assume). 
Then the solution to \eqref{eq:svm-restricted-dual-lp} is:\footnote{
Note that \eqref{eq:svm-restricted-dual-lp} will never be optimized by $\vec{0}$, because there must always exist some $\alpha$ with strictly positive components such that $\norml[q]{\bA^\T \alpha} \leq 1$. Therefore, we need not worry about the projection being undefined.}
\begin{equation}
    \label{eq:projection-lq}
    \tag{Interpolation Projection}
    \min_{\alpha \in \mathbb{R}^{n}}{ \norm[q]{\bA^\T \frac{\alpha}{\sum_{i=1}^{n}{\alpha_{i}}}} 
    = \norm[q]{\Pi_{\bT}(\vec{0}) }}.
\end{equation}

By the definition of $\bT$ and $\bT^+$ and the fact that $\proj = \bA^\T \alpha^* / \vec{1}^\T \alpha^*$ for $\alpha^*$ optimizing \eqref{eq:projection-lq}, we have that $\alpha^* \in \R_+^d$ if and only if $\proj \in \bT^+$.

\lesscrazyparagraph{(4) $\iff$ (5):}
% \navid{I changed the proof to work even for the case $K$ is non-invertible. be more careful of whether there is a whole in the proof or not.}
% \clayton{change back :P}
% As defined in Section \ref{sec:prelim}, consider $\bA \in \mathbb{R}^{n \times d}$ to be the collection of $(y_{i}\bx_{i})_{i \le n}$ which is assumed to contain $\one$ in it's range which implies \eqref{eq:svm-restricted-primal-lp} problem is feasible. For convenience let us also define $\mathbf{T}_{\setminus i}$ to be the affine hull of rows of $\bA$ except the $i$th row. Further let $\proj = \fracl{\bA^\T \alpha^{*}}{\one^\T \alpha^{*}}$ where $\alpha^{*}$ is the unique optimal solution to \eqref{eq:svm-restricted-dual-lp}. 
By the \eqref{eq:projection-lq} formulation, $\proj$ can be alternatively interpreted as the projection of the origin onto the affine space $\mathbf{T}$. 
Therefore we have,
%\violet{ Since $\mathbf{T}$ does not contain the origin, one can express every point on $\mathbf{T}$ by an affine combination of points $(\bA_{i})_{i \le n}$ uniquely}; 
\begin{equation}\label{eq:projection-representation}
    \proj = \sum_{i=1}^{n}{ a^{*}_{i}\bA_{i} } = \arg \min_{u \in \mathbf{T}} \norm[2]{u}^{2}
\end{equation}
where $a^{*}_{i} \in \mathbb{R}$ is proportional to $\alpha_{i}^{*}$ such that $\sum_{i=1}^{n}{a^{*}_{i}} = 1$. 
This is possible because the optimal value of \eqref{eq:svm-restricted-primal-lp} is positive. %, hence $\sum_{i=1}^{n}{\alpha_{i}^{*}} > 0$.

The following steps show the equivalence:
\begin{enumerate}
    \item For every $i \in [n]$ we show,
    \begin{equation}\label{eq:coef-interpretation}
        a^{*}_{i} > 0 \quad \Longleftrightarrow \quad \bA_{i}^\T \projj{i}  < \norm[2]{\projj{i}}^{2}
    \end{equation}
    by leveraging the fact that $\ell_{2}$ space is equipped with inner product which allows us to decompose the contribution of each sample to the projection. 
    
    \item We find an explicit expression for $\proj$:
        \begin{equation}\label{eq:projection-explicit}
            \proj =  \frac{\bA^\T \paren{\bA\bA^\T}^{-1} \one }{\one^\T \paren{\bA\bA^\T}^{-1} \one }= \frac{\bX \paren{\bX^{\T}\bX}^{-1} y }{y^\T \paren{\bX^{\T}\bX}^{-1} y }.
        \end{equation}
        An analogous expression for $\projj{i}$ can be found for any fixed $i$ by the same method, which gives the desired equivalence by combining with \eqref{eq:coef-interpretation}.
\end{enumerate}

\emph{First Step:} Fix some index $i \in [n]$. Since $\Pi_{\mathbf{T}_{\setminus i}}(\bA_i)$ is on the affine space $\mathbf{T}_{\setminus i}$, which is closed under affine linear combination, one can express $\mathbf{T}$ in the following way:
\begin{align*}
    \mathbf{T} &= \Big\{ \sum_{j=1}^{n}{a_{j}\bA_j} : \sum_{j=1}^{n}{a_{j}} = 1 \Big\} \\
    &= \Big\{ a_{i} \paren{\bA_i - \Pi_{\mathbf{T}_{\setminus i}}(\bA_i)} + \Big(a_{i}  \Pi_{\mathbf{T}_{\setminus i}}(\bA_i) + \sum_{j \neq i}{a_{j}\bA_{j}}\big)  : \sum_{j \neq i}{a_{j}} = 1-a_{i} \ , a_{i}\in \mathbb{R} \Big\} \\
    &= \Big\{ a_{i} (\bA_i - \Pi_{\mathbf{T}_{\setminus i}}(\bA_i)) + u: u \in \mathbf{T}_{\setminus i} \ , a_{i}\in \mathbb{R} \Big\} .
\end{align*}

By the definition of the projection onto $\mathbf{T}$, we represent $\proj = a^{*}\paren{\bA_i - \Pi_{\mathbf{T}_{\setminus i}}(\bA_i)} + u^{*}$ where,
\[
(a^{*}, u^{*}) = \argmin_{(a, u) \in \mathbb{R} \times \mathbf{T}_{\setminus i}}  \norm[2]{ a( \bA_{i} - \Pi_{\mathbf{T}_{\setminus i}}(\bA_{i}) ) + u }^{2}.
\]
% \navid{we don't need the convention anymore bc we are assuming full rank A} with the convention that $a^{*} \coloneqq a_{i}^{*}$ when $\bA_i \in \mathbf{T}_{\setminus i}$. \navid{we don't need to do it case by case. we can just say we argue that $a^{*}$ should be interpreted as $a_{i}^{*}$ by uniqueness} 
It is straightforward to see that $a^{*} = a_{i}^{*}$ by comparing this representation with equation \eqref{eq:projection-representation} alongside with the fact that $\bA_i - \Pi_{\mathbf{T}_{\setminus i}}(\bA_i)$ is orthogonal to $\mathbf{T}_{\setminus i}$:

\[
\zero = \proj - \proj = \paren{a^{*} - a_{i}^{*}}\paren{\bA_i - \Pi_{\mathbf{T}_{\setminus i}}(\bA_i)} + \Big( u^{*} - \underbrace{\Big(\sum_{j \neq i}{a_{j}^{*} \bA_{j}} + a_{i}^{*} \projj{i}\Big)}_{ \in \mathbf{T}_{\setminus i}}  \Big).
\]

% \clayton{Maybe swap $a^*$ with something to make it clear that it depends on index? Maybe WLOG $i = 1$?}
To find $a^{*}$, we sequentially optimize over $u$, substitute its optimal value, and then optimize over $a$. 
It suffices to minimize $\norm[2]{u}^{2}$ because $ u^\T (\bA_i - \Pi_{\mathbf{T}_{\setminus i}}(\bA_i) )$ is constant for all $u \in \mathbf{T}_{\setminus i}$ due to orthogonality and the definition of $\mathbf{T}_{\setminus i}$.
Hence, $u^{*} = \projj{i}$ is optimal. 
Subsequently, by optimizing over $a$ and setting the derivative to zero, 
% \todo{$a^*$ is in the wrong place according a reviewer; rearrange?} \navid{\checkmark}
\[
( \bA_{i} - \Pi_{\mathbf{T}_{/i}}(\bA_{i}))^\T  \paren{a^{*} \paren{ \bA_{i} - \Pi_{\mathbf{T}_{/i}}(\bA_{i})} + \projj{i}} = 0
\]
or equivalently,
\[
a^{*} 
= \frac{(\Pi_{\mathbf{T}_{/i}}(\bA_{i}) - \bA_{i})^\T \projj{i}}{ \norm[2]{\bA_{i} - \Pi_{\mathbf{T}_{\setminus i}}(\bA_{i})}^{2} } 
= \frac{ \norm[2]{ \projj{i} }^{2} -  \bA_{i}^\T \projj{i} }{ \norm[2]{\bA_{i} - \Pi_{\mathbf{T}_{/i}}(\bA_{i})}^{2} }
\]
For the last step, we combine the facts that $ \projj{i}^\T u$ is constant over $\mathbf{T}_{\setminus i}$ and $\projj{i} \in \mathbf{T}_{\setminus i}$. 
Note that the denominator is non-zero because the invertibility of $\bK$ implies that $\bA_i$ will not lie on the span of the remaining rows $\bA_{\setminus i}$, and hence will not be in $\bT_{\setminus i}$.
This immediately proves \eqref{eq:coef-interpretation}. 
% \clayton{I don't quite follow this, probably because I've mixed up how $a^*$ and $a^*_i$ are defined.} 
% \clayton{Say that $\norm[2]{\bA_i - \Pi_{\mathbf{T}_{\setminus i}}(\bA_i)} > 0$.} 


\emph{Second Step:} We now shift our focus to expressing $\proj$ explicitly in terms of $\bA$. As discussed in Section \ref{sec:prelim}, the projection of the origin onto $\mathbf{T}$ for $\ell_{2}$-SVM can be expressed in an explicit way as $\proj = \bA^\T \fracl {\alpha^{*}}{ \one^{\T} \alpha^{*} }$, where $\alpha^{*}$ is the unique solution to \eqref{eq:svm-restricted-dual-lp} for $p=q=2$. In order to represent $\alpha^{*}$ explicitly one can reform \eqref{eq:svm-restricted-dual-lp} using a simple change of variables $\nu = \paren{\bA\bA^\T}^{\fracl{1}{2}}\alpha$ into,
\[
\nu^{*} = \argmax_{\nu \in \R^n} \nu^\T \paren{\bA\bA^\T}^{\fracl{-1}{2}} \one \quad \text{s.t. } \norm[2]{\nu} \le 1.
\]
This problem can be easily understood using a simple Cauchy-Schwarz inequality, 
\[
\alpha^{*} = \paren{\bA\bA^\T}^{\fracl{-1}{2}} \nu^{*} = \fracl{\paren{\bA\bA^\T}^{-1} \one}{ \sqrt{ \one^\T \paren{\bA\bA^\T}^{-1} \one } .}
\]
In conclusion, we can express the projection as,
\[
\proj = \frac{\bA^\T \alpha^{*}}{\one^\T \alpha^* } = \frac{\bA^\T \paren{\bA\bA^\T}^{-1} \one }{\one^\T \paren{\bA\bA^\T}^{-1} \one } = \frac{\bX^\T \paren{\bX\bX^\T}^{-1} y }{y^\T \paren{\bX\bX^\T}^{-1} y }.\qedhere
\]
%\navid{Should we state somewhere that invertiblity of $K$ implies invertiblity of $K_{\setminus i}$ (or any submatrix)}
\end{proof}



==> SVM NeurIPS (3)/prelim_old.tex <==
\section{Preliminaries}\label{sec:prelim}

\subsection{Notation}
For $\lambda\in \R_{+}^d$, define $d_2 := \fracl{\norml[1]{\lambda}^2}{\norml[2]{\lambda}^2}$ and $d_{\infty} := \fracl{\norml[1]{\lambda}}{\norml[\infty]{\lambda}}$, and note that $d \geq d_2 \geq d_{\infty}$.
$d_2$ and $d_{\infty}$ can differ substantially from one another:
If $\lambda = (1,\sqrt{d}, \dots, \sqrt{d})$, then $d_2 = \Theta(d)$ and $d_{\infty} = \Theta(\sqrt{d})$.

\todo{Notation for $\bX_{\setminus i}, \bX_{[m]}, \bx_{[m] \setminus i}, \bX_{\setminus [m]}$, etc}

Let $\mu_{\max}(A)$ and $\mu_{\min}(A)$ represent the largest and smallest eigenvalues of matrix $A$ respectively.

Let $[n] := \set{1, \dots,  n}$.

\subsection{Learning model}
\clayton{some of this will surely be moved to the introduction}

We consider the hard-margin support vector machine (SVM) optimization problem and ask under what conditions one may expect all the slackness conditions to be satisfied. 
We consider training samples $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \flip$ in a high-dimensional regime where $d \gg n$ and let $\bX := [\bx_1 | \dots | \bx_n]^\T \in \R^{n \times d}$ to represent the inputs collected into a matrix \todo{there's a name for this...} and $\bK = \bX \bX^\T \in \R^{n \times n}$ be the corresponding Gram matrix.
In full generality, the separating hyperplane corresponding to the $\ell_p$-norm SVM problem for some $p \geq 1$ is the solution to the following optimization problem:
\begin{equation}
    \tag{SVM Primal}
    \label{eq:svm-primal-lp}
    \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i \innerprod{w}{\bx_i} \geq 1, \ \forall i \in [n].
\end{equation}

It is worth mentioning that we are not concerned with feasibility issues since $w$ resides in a high dimensional world \navid{Somewhere probably we should mention about Cover's result}. Moreover, we call a training sample $(\bx_i, y_i)$ to be a \emph{support vector} if it lies exactly on the margin defined by separator $w$, or equivalently if $y_i \innerprod{w}{\bx_i} = 1$.
\todo{say something about alternate representation of $w$ as linear combination of support vectors}
We study the phenomenon of \emph{support vector proliferation}, which occurs when $(\bx_i, y_i)$ is a support vector for all $i \in [n]$.
This can be equivalently understood at the event that the solution to the \eqref{eq:svm-primal-lp} coincides exactly with that of
\begin{equation}
    \tag{Interpolation Primal}
    \label{eq:svm-restricted-primal-lp}
    \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i \innerprod{w}{\bx_i} = 1, \ \forall i \in [n].
\end{equation}

% \begin{center}
% \begin{minipage}{0.25\textwidth}
%     \begin{align*}
%     \min & \quad \|w\|_{p} \\
%     \text{s.t.} & \quad Y_{i} \langle w , X_{i} \rangle \ge 1 
%     \end{align*}
% \end{minipage}
% $\overset{?}{=}$
% \begin{minipage}{0.25\textwidth}
%     \begin{align*}
%     \min & \quad \|w\|_{p} \\
%     \text{s.t.} & \quad Y_{i} \langle w , X_{i} \rangle = 1 
%     \end{align*}
% \end{minipage}
% \end{center}

Moreover, we can translate this relation in the dual space by adding Lagrange multipliers $\alpha \in \mathbb{R}^{n}$, and obtain the dual of \eqref{eq:svm-restricted-primal-lp}:
\[
\max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} + \min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \innerprod{ w}{ \sum_{i=1}^{n}{\alpha_{i}y_{i}\bx_{i} }}}.
\]
Now using Holder's inequality if we take $q$ to be the dual of $p$ (i.e. $\frac{1}{p} + \frac{1}{q} = 1$) then $\langle w, u \rangle \le \|w\|_{p} \|u\|_{q}$ where equality holds when $|u_{i}|^{q} = |w_{i}|^{p}$ thus we have:

\[\min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \langle w, u \rangle} = 
\begin{cases}
0 & \|u\|_{q} \le 1 \\
-\infty & \text{otherwise.}\\
\end{cases}
\]
Let us further denote $\bA \in \mathbb{R}^{d \times n}$ where the $i$'th column is $y_{i}\bx_{i}$ then we conclude that the dual of optimization \eqref{eq:svm-primal-lp} is:
\begin{equation}
    \tag{Interpolation Dual}
    \label{eq:svm-restricted-dual-lp}
    \max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} \quad
    \text{such that}  \quad \|\bA\alpha \|_{q} \le 1 .
\end{equation}

Similarly one can find the dual of \eqref{eq:svm-primal-lp} to be analogous to \eqref{eq:svm-restricted-dual-lp} where the difference is excess restriction on $\alpha$ having non-negative coordinates, i.e. $\alpha \in \mathbb{R}_{+}^{n}$. To reiterate, we are interested in the event that this excessive constraints are in a sense redundant. In other words, support vector proliferation occurs if and only if $\alpha^{*}_i > 0$ for all $i \in [n]$ where $\alpha^{*}$ is an optimal solution for \eqref{eq:svm-restricted-dual-lp} problem \todo{ref to appropriate lemma here}.  It is fairly straightforward to see that optimal solutions of \eqref{eq:svm-restricted-dual-lp} are equivalent to the following problem:

\begin{equation}
    \label{eq:projection-lq}
    \min_{\alpha \in \mathbb{R}^{n} \setminus \{\mathbf{0}\}}{ \norm[q]{\bA \frac{\alpha}{\sum_{i=1}^{n}{\alpha_{i}}}} }
\end{equation}
\daniel{do you need to require $\sum \alpha_i \neq 0$?}

This formulation is intuitive at the very least for the $\ell_{2}$-case since it demonstrates a well known fact that separating hyperplane is obtained as  a linear combination of inputs. In order to provide a geometric interpretation of \eqref{eq:projection-lq} let us denote $T, T^{+}$ to respectively be the hyperplane passing through and convex hulls of columns of $A$. We may then interpret the optimization problem above as a projection of the origin onto the set $T = \{\sum_{i=1}^{n}{a_{i}A_{i}} : \sum_{i=1}^{n}{a_{i}} = 1\} \subset \mathbb{R}^{d}$ using $\ell_{q}$-norm. 

\textbf{Main Question:} Now that we have all the prerequisites we may form our main question in two alternative point of views roughly as the following:
\begin{itemize}
    \item Under which settings of input samples the optimal solution to \eqref{eq:svm-restricted-dual-lp} lies within the interior of $\mathbb{R}_{+}^{d}$?
    
    \item under which setting of input samples the projection of the origin onto $T$ denoted by $\Pi_{T}(0)$ lies inside $T^{+}$?
\end{itemize}
 


This dual framework gives an alternative geometric structure to consider for this problem, which is explored in detail for the $\ell_1$ case in Section~\ref{sec:l1}. Essentially, we use the fact that $\ell_{1}$-case boils down to an LP problem where the corner points of the constraint set determines the behaviour of our optimization problem.



%\begin{equation}
%    \label{eq:svm-dual-l1}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad -\vec{1} \leq \bA\alpha \leq \vec{1} .
%\end{equation}
%
%\begin{equation}
%    \label{eq:svm-dual-l2}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad 1 \leq \alpha^\T \diag(y) \bK \diag(y) %\alpha \leq 1.
%\end{equation}


\subsection{Data model}
We use the same data model of \cite{hmx20}, where every labeled sample $(\bx_i, y_i)$ has $\bx_i$ drawn from an anisotropic subgaussian distribution with independent components and arbitrary fixed labels $y_i$.
\todo{Say something about why linear separability won't be a problem for us}

\begin{definition}
    For some $\lambda\in \R_{\geq 0}^d$, let a \emph{$\lambda$-anisotropic sample} be $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \flip$ drawn as follows.
    Let $\bX := [\bx_1 |  \dots | \bx_n]^\T = \bZ \  \diag(\lambda)^{1/2} \in \R^{n \times d}$, where each $\bz_i$ has independent subgaussian components  with $\EEl{\bz_{i,j}} = 0$ and $\EEl{\bz_{i,j}^2} = 1$.
	Additionally, assume that $\bz_{i,j}$ is subgaussian for all $i \in [n], j \in [d]$.
	Let $y = (y_1, \dots, y_n)$ be arbitrary labels that do not depend on $\bX$.
\end{definition}

We also consider a simpler data model of isotropic Gaussian samples, which allows us to more tightly characterize the support vector proliferation threshold in Theorem~\ref{thm:asymptotic-lb} and \ref{thm:asymptotic-up}.

\begin{definition}
    A \emph{Gaussian isotropic sample} consists of independent $(\bx_1, y_1), \dots, (\bx_n, y_n) \sim \mathcal{N}(0, I_d)$ drawn as follows, which can be collected as $\bX := [\bx_1 |  \dots | \bx_n]^\T \in \R^{n \times d}$.
    Let $y = (y_1, \dots, y_n)$ be arbitrary labels that do not depend on $\bX$.
\end{definition}

\todo{Say something about random labels:

- we don't need to worry about linear separability for arbitrary labels because of Cover result

- we can also handle labels that depend on a ground truth linear classifier. banish this to the appendix or explain why it's easy? 
}

\subsection{Previous results}

We build on the upper- and lower-bounds presented in \cite{hmx20} for the support vector proliferation threshold. 
We give versions of their results that are directly comparable to our results in Sections~\ref{sec:nonasymp} and \ref{sec:asymptotic}.
\clayton{Is it okay that we rephrase them to have them in terms of $\delta$?}

\begin{theorem}[\cite{hmx20} Theorem~1: Upper-bound on SV proliferation threshold for anisotropic subgaussian]\label{thm:hmx-ub}
    Consider a $\lambda$-anisotropic sample $\bX$ and $y$ and some $\delta > 0$.
    If $d_{\infty} = \Omega(n \log (n) \log (\frac{1}{\delta}))$, then with every sample is a support vector for the $\ell_2$ SVM problem with probability $1 - \delta$.
\end{theorem}

\begin{theorem}[\cite{hmx20} Theorem~3: Lower-bound on SV proliferation threshold for isotropic Gaussian]\label{thm:hmx-lb}
    Consider an isotropic Gaussian sample $\bX$ and $y$. 
    If $d = O(n)$, then with constant probability, there exists some sample that is not a supprt vector for the $\ell_2$ SVM problem. 
\end{theorem}

The authors of \cite{hmx20} note the logarithmic separation between Theorems~\ref{thm:hmx-ub} and \ref{thm:hmx-lb} and the limited data model used in Theorem~\ref{thm:hmx-lb}, and pose an improvement to their lower-bound as an open problem.
We solve this problem for the $\ell_2$ case here by broadening Theorem~\ref{thm:hmx-lb} to handle $\lambda$-anisotropic samples and by eliminating the logarithmic separation in Theorem~\ref{thm:anisotropic}.
In addition, we show that the threshold can be precisely captured up to constant factor as $n$ and $d$ trend towards $\infty$ in the isotropic Gaussian setting in Theorems~\ref{thm:asymptotic-lb} and \ref{thm:asymptotic-up}.


We make extensive use of the deterministic equivalence given in \cite{hmx20}.
\begin{lemma}\label{lemma:hmx-equivalence}
    For samples $(\bx_1, y_1), \dots, (\bx_n, y_n)\in \R^d \times \flip$ such that $\bK$ and $\bK_{\setminus i} := \bX_{\setminus i} \bX_{\setminus i}^\T$ are non-singular for all $i \in [n]$, every training sample is a support vector for the solution to the $\ell_2$ SVM if and only if $y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \bx_i < 1$ for all $i \in [n]$.
\end{lemma}
We also offer an alternate proof the lemma in the appendix. \todo{do this and give geometric interpretation of lemma}

==> SVM NeurIPS (3)/prelim_temp.tex <==
\section{Preliminaries}\label{sec:prelim}

This section introduces notation, as well as the optimization problems and data models we consider.
We also define support vector proliferation and prove the equivalence of different formulations.

\subsection{Notation}
For $\lambda\in \R_{+}^d$, we define the $\ell_2$ and $\ell_{\infty}$ \emph{dimension proxies} as $d_2 := \fracl{\norml[1]{\lambda}^2}{\norml[2]{\lambda}^2}$ and $d_{\infty} := \fracl{\norml[1]{\lambda}}{\norml[\infty]{\lambda}}$
% , and note that $d \geq d_2 \geq d_{\infty}$.
% $d_2$ and $d_{\infty}$ can differ substantially from one another:
% If $\lambda = (1,\sqrt{d}, \dots, \sqrt{d})$, then $d_2 = \Theta(d)$ and $d_{\infty} = \Theta(\sqrt{d})$.
Let $[n] := \set{1, \dots,  n}$.
For some vector $w \in \R^n$ and matrix $A \in \R^{n \times d}$, we let $w_i$ and $A_i$ denote the $i$th element of $w$ and row of $A$ respectively; likewise, we let $A_\col{j} \in \R^n$ represent the $j$th column of $A$.
We abuse notation to let $w_{\setminus i} = (w_1, \dots, w_{i-1}, w_{i+1}, \dots, w_n) \in \R^{n-1}$, $w_{[m]} = (w_1, \dots, w_m) \in \R^m$, $w_{\setminus [m]} = (w_{m+1}, \dots, w_n) \in \R^{n-m}$, and $w_{[m] \setminus i} = (w_{[m]})_{\setminus i} \in \R^{m-1}$ for $i \in [m]$ and $m \in [n]$.
Analogous notation holds for $A_{\setminus i}$, $A_{[m]}$, $A_{\setminus [m]}$, and $A_{[m] \setminus i}$.
We frequently consider the Gram matrix $\bK := \bX \bX^\T \in \R^{n\times n}$ for feature matrix $\bX \in \R^{n \times d}$; for these matrices, we let $\bK_{\setminus i} = \bX_{\setminus i} \bX_{\setminus i}^\T \in \R^{(n-1)\times(n-1)}$ and analogously define $\bK_{[m]}$, $\bK_{\setminus [m]}$, and $\bK_{[m] \setminus i}$.
Let $\mu_{\max}(A)$ and $\mu_{\min}(A)$ represent the largest and smallest eigenvalues of the matrix $A$ respectively, and let $\norml{A}$ be the operator norm of $A$.
For some vector $y \in \R^n$, we let $\diag(y) \in \R^{n \times n}$ be a diagonal matrix with $(\diag(y))_{i,i} = y_i$.
Throughout, boldface characters refer to random variables.
%We define $O(\cdot)$, $o(\cdot)$, $\Omega(\cdot)$, $\omega(\cdot)$, and $\Theta(\cdot)$ as is standard for Bachmann-Landau (or ``Big-O'') notation . \daniel{do we actually use them all? if we don't use $\omega(\cdot)$ for instance, we shouldn't mention it here.}
%\todo{clarify big-O :P}\clayton{\checkmark}


% \subsection{Learning model}
% \clayton{some of this will surely be moved to the introduction}

% We consider the hard-margin support vector machine (SVM) optimization problem and ask under what conditions one may expect all the slackness conditions to be satisfied. 
% We consider training samples $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \flip$ in a high-dimensional regime where $d \gg n$ with design matrix $\bX := [\bx_1 | \dots | \bx_n]^\T \in \R^{n \times d}$ and Gram matrix $\bK = \bX \bX^\T \in \R^{n \times n}$.
% In full generality, the separating hyperplane corresponding to the $\ell_p$-norm SVM problem for some $p \geq 1$ is the solution to the following optimization problem:
% \begin{equation}
%     \tag{SVM Primal}
%     \label{eq:svm-primal-lp}
%     \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i \innerprod{w}{\bx_i} \geq 1, \ \forall i \in [n].
% \end{equation}

% It is worth mentioning that we are not concerned with feasibility issues since $w$ resides in a high dimensional world \navid{Somewhere probably we should mention about Cover's result}. A sample $(\bx_i, y_i)$ is called a \emph{support vector} if it lies exactly on the margin defined by separator $w$, or equivalently if $y_i \innerprod{w}{\bx_i} = 1$.
% \todo{say something about alternate representation of $w$ as linear combination of support vectors}
% We study the phenomenon of \emph{support vector proliferation} (SVP), which occurs when $(\bx_i, y_i)$ is a support vector for all $i \in [n]$.
% This can be equivalently understood at the event that the solution to the \eqref{eq:svm-primal-lp} coincides exactly with that of
% \begin{equation}
%     \tag{Interpolation Primal}
%     \label{eq:svm-restricted-primal-lp}
%     \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i \innerprod{w}{\bx_i} = 1, \ \forall i \in [n].
% \end{equation}

% % \begin{center}
% % \begin{minipage}{0.25\textwidth}
% %     \begin{align*}
% %     \min & \quad \|w\|_{p} \\
% %     \text{s.t.} & \quad Y_{i} \langle w , X_{i} \rangle \ge 1 
% %     \end{align*}
% % \end{minipage}
% % $\overset{?}{=}$
% % \begin{minipage}{0.25\textwidth}
% %     \begin{align*}
% %     \min & \quad \|w\|_{p} \\
% %     \text{s.t.} & \quad Y_{i} \langle w , X_{i} \rangle = 1 
% %     \end{align*}
% % \end{minipage}
% % \end{center}

% Moreover, we can translate this relation in the dual space by adding Lagrange multipliers $\alpha \in \mathbb{R}^{n}$, and obtain the dual of \eqref{eq:svm-restricted-primal-lp}:
% \[
% \max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} + \min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \innerprod{ w}{ \sum_{i=1}^{n}{\alpha_{i}y_{i}\bx_{i} }}}.
% \]
% Now using Holder's inequality if we take $q$ to be the dual of $p$ (i.e. $\frac{1}{p} + \frac{1}{q} = 1$) then $|\langle w, u \rangle| \le \|w\|_{p} \|u\|_{q}$ where equality holds when $|u_{i}|^{q}$ is proportional to $|w_{i}|^{p}$ which gives:

% \[\min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \langle w, u \rangle} = 
% \begin{cases}
% 0 & \|u\|_{q} \le 1 \\
% -\infty & \text{otherwise.}\\
% \end{cases}
% \]
% We further denote $\bA =  \diag(y) \bX  \in \mathbb{R}^{n \times d}$, whose $i$th row is $y_{i}\bx_{i}$. We conclude that the dual of optimization \eqref{eq:svm-restricted-primal-lp} is:
% \begin{equation}
%     \tag{Interpolation Dual}
%     \label{eq:svm-restricted-dual-lp}
%     \max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} \quad
%     \text{such that}  \quad \|\bA^\T \alpha \|_{q} \le 1 .
% \end{equation}

% Similarly one can find the dual of \eqref{eq:svm-primal-lp} to be analogous to \eqref{eq:svm-restricted-dual-lp} where the difference is excess restriction on $\alpha$ having non-negative coordinates, i.e. $\alpha \in \mathbb{R}_{+}^{n}$. To reiterate, we are interested in the event that this excessive constraints are in a sense redundant. In other words, support vector proliferation occurs if and only if $\alpha^{*}_i > 0$ for all $i \in [n]$ where $\alpha^{*}$ is an optimal solution for \eqref{eq:svm-restricted-dual-lp} problem \todo{ref to appropriate lemma here}.  It is fairly straightforward to see that optimal solutions of \eqref{eq:svm-restricted-dual-lp} are equivalent to the following problem:

% \begin{equation}
%     \label{eq:projection-lq}
%     \tag{Projection}
%     \min_{\alpha \in \mathbb{R}^{n} \setminus \{\zero\}}{ \norm[q]{\bA^\T \frac{\alpha}{\sum_{i=1}^{n}{\alpha_{i}}}} }
% \end{equation}
% \daniel{do you need to require $\sum \alpha_i \neq 0$?} \navid{Well the interpolation primal problem has a  positive optimal objective value so $\sum \alpha_i > 0$ should hold at optimal solutions right? but yes we should mention this condition probably.}

% This formulation is intuitive at the very least for the $\ell_{2}$-case since it demonstrates a well known fact that separating hyperplane is obtained as  a linear combination of inputs. In order to provide a geometric interpretation of \eqref{eq:projection-lq} let us denote $\mathbf{T}, \mathbf{T}^{+}$ to respectively be the plane passing through and convex hulls of rows of $\bA$. We may then interpret the optimization problem above as a projection of the origin onto the set $\mathbf{T} = \{\sum_{i=1}^{n}{a_{i}\bA_{i}} : \sum_{i=1}^{n}{a_{i}} = 1\} \subset \mathbb{R}^{d}$ using $\ell_{q}$-norm. 

% \textbf{Main Question:} Now that we have all the prerequisites we may form our main question in two alternative point of views roughly as the following:
% \begin{enumerate}
%     \item \label{itm:Q1} Under which settings of input samples the optimal solution to \eqref{eq:svm-restricted-dual-lp} lies within the interior of $\mathbb{R}_{+}^{d}$?
    
%     \item \label{itm:Q2} under which settings of input samples the projection of the origin onto $T$ denoted by $\Pi_{T}(0)$ lies inside $T^{+}$?
% \end{enumerate}


% This dual framework gives an alternative geometric structure to consider for this problem, which is explored in detail for the $\ell_1$ case in Section~\ref{sec:l1}. Essentially, we use the fact that $\ell_{1}$-case boils down to an LP problem where the corner points of the constraint set determines the behaviour of our optimization problem.



%\begin{equation}
%    \label{eq:svm-dual-l1}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad -\vec{1} \leq \bA\alpha \leq \vec{1} .
%\end{equation}
%
%\begin{equation}
%    \label{eq:svm-dual-l2}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad 1 \leq \alpha^\T \diag(y) \bK \diag(y) %\alpha \leq 1.
%\end{equation}

% \clayton{
% Thoughts on adding this to replace both the ``Main question'' and Lemma~\ref{lemma:hmx-equivalence}?
% \begin{proposition}
% The following are equivalent:
% \begin{enumerate}[label=(\arabic*)]
%     \item Support vector proliferation occurs for an SVM trained on $\bX$ and $y$.
%     \item The solutions $w$ to \ref{eq:svm-primal-lp} and \ref{eq:svm-restricted-primal-lp} are identical.
%     \item The optimal solution to \eqref{eq:svm-restricted-dual-lp} lies within the interior of $\mathbb{R}_{+}^{d}$.
%     \item Projection of the origin onto $\mathbf{T}$ denoted by $\proj$ lies inside $\mathbf{T}^{+}$.
% \end{enumerate}
% Moreover, if $p=2$, then properties (1) - (4) are also equivalent to the following:
% \begin{enumerate}[label=(\arabic*)]
%     \setcounter{enumi}{4}
%     \item  For all $i \in [n]$, $\langle y_{i}\bx_{i}, y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \rangle = \innerprod{ y_{i}\bx_{i}}{ \frac{\projj{i}}{\| \projj{i} \|_{2}^{2}}} < 1.$
% \end{enumerate}
% \end{proposition}
% }

\subsection{Optimization problems}

We consider the hard-margin support vector machine (SVM) optimization problem and ask under what conditions one may expect all the slackness conditions to be satisfied. 
We consider training samples $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \flip$ in a high-dimensional regime where $d \gg n$ with design matrix $\bX := [\bx_1 | \dots | \bx_n]^\T \in \R^{n \times d}$ and Gram matrix $\bK = \bX \bX^\T \in \R^{n \times n}$.
In full generality, the separating hyperplane corresponding to the $\ell_p$-SVM problem for some $p \geq 1$ is the solution to the following optimization problem:
\begin{equation}
    \tag{SVM Primal}
    \label{eq:svm-primal-lp}
    \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i w^\T\bx_i \geq 1, \ \forall i \in [n].
\end{equation}
Our results in Sections~\ref{sec:nonasymp}--\ref{sec:experiments} concern $p=2$, and we discuss $p=1$ in Section~\ref{sec:l1}.
It is worth mentioning that feasibility is not a concern in the settings we consider.\footnote{When $d \ge n$, we are always able to find a separating hyperplane since the features are linearly independent with high probability. In fact, a theorem of \citet{cover1965geometrical} shows that feasibility holds with high probability under mild distributional assumptions even for $d > \fracl{n}{2}$.}
%A theorem of \citet{cover1965geometrical} implies that, for any fixed set of $n$ labels, a random sample of $n$ features vectors from a continuous distribution in $\R^d$ will be linearly separable with high probability as soon as $d = \Omega(n)$.
%$n$ random samples with $d$-dimensional features from a continuous distribution and arbitrary fxied labels will be linearly separable with high probability when $d = \Omega(n)$.
%\clayton{verify that this is correct interpretation}
An example $(\bx_i, y_i)$ is called a \emph{support vector} if it lies exactly on the margin defined by separator $w$, or equivalently if $y_i w^\T {\bx_i} = 1$.
It is well-known that $w$ can be represented as a non-negative linear combination of all $y_i \bx_i$ where $\bx_i$ is a support vector~\cite{vapnik1982estimation}.

We contrast the weights of the classifier returned by \ref{eq:svm-primal-lp} with the weights of minimum $\ell_p$-norm that satisfy the normal equations of ordinary least squares (OLS).
In the case where the training data can be linearly interpolated, this optimization problem is:
\begin{equation}
    \tag{Interpolation Primal}
    \label{eq:svm-restricted-primal-lp}
    \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i w^\T{\bx_i} = 1, \ \forall i \in [n].
\end{equation}
Per the convention mentioned in the introduction,
the solution of \eqref{eq:svm-restricted-primal-lp} when $p=2$ is referred to as ordinary least squares.
Feasibility is ensured as long as the feature vectors $\bx_i$ are linearly independent.
%If $p = 2$, then  is the ordinary least squares regression in the interpolation regime.

\subsection{Equivalent formulations of SVP}

We study the phenomenon of \emph{support vector proliferation} (SVP), i.e., the occurrence in which every example $\bx_i$ is a support vector.
Because $\bx_i$ is a support vector if $y_i w^\T{\bx_i} = 1$, this occurs if and only if the solution of \eqref{eq:svm-primal-lp} coincides exactly with that of \eqref{eq:svm-restricted-primal-lp}.
Here, we analyze those formulations to show equivalent conditions needed for SVP, which we give in Proposition~\ref{prop:equiv}.
Before presenting the proposition, we introduce the notation needed to use the alternate formulations.

We translate the relationship between the two primal optimization problems into the dual space.
% By adding Lagrange multipliers $\alpha \in \mathbb{R}^{n}$, we obtain the dual of \eqref{eq:svm-restricted-primal-lp}:
% \[
% \max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} + \min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \innerprod{ w}{ \sum_{i=1}^{n}{\alpha_{i}y_{i}\bx_{i} }}}.
% \]
% By Holder's inequality, if we take $q$ to be the dual of $p$ (i.e. $\frac{1}{p} + \frac{1}{q} = 1$), then $|\langle w, u \rangle| \le \|w\|_{p} \|u\|_{q}$, with equality when $|u_{i}|^{q}$ is proportional to $|w_{i}|^{p}$.
% Therefore,
% \[\min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \langle w, u \rangle} = 
% \begin{cases}
% 0 & \|u\|_{q} \le 1 \\
% -\infty & \text{otherwise.}\\
% \end{cases}
% \]
Taking $\bA =  \diag(y) \bX  \in \mathbb{R}^{n \times d}$, the dual of the optimization problem \eqref{eq:svm-restricted-primal-lp} is:
\begin{equation}
    \tag{Interpolation Dual}
    \label{eq:svm-restricted-dual-lp}
    \max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} \quad
    \text{such that}  \quad \|\bA^\T \alpha \|_{q} \le 1 .
\end{equation}

The dual of \eqref{eq:svm-primal-lp} is \eqref{eq:svm-restricted-dual-lp} with an additional constraint that $\alpha \in \mathbb{R}_{+}^{n}$.
% To reiterate, SVP occurs when these extra constraints are redundant, or when $\alpha^{*}_i > 0$ for all $i \in [n]$, where $\alpha^{*}$ is an optimal solution for \eqref{eq:svm-restricted-dual-lp} problem \todo{ref to appropriate lemma here}. 

% We give a geometric reconfiguration of  \eqref{eq:svm-restricted-dual-lp} to show an equivalent condition for SVP.
Let $\bT = \set{\sum_{i=1}^n a_i \bA_i : \sum_{i=1}^n a_i = 1}$ denote the affine plane passing through the rows of $\bA$, and let $\bT^+ = \set{\sum_{i=1}^n a_i \bA_i : \sum_{i=1}^n a_i = 1, \ a_i \geq 0}$ be the convex hull of the rows of $\bA$.
In addition, for $i \in [n]$, let $\bT_{\setminus i} = \setl{\sum_{i'\neq i} a_{i'} \bA_{i'} : \sum_{i'\neq i} a_{i'} = 1}$.
We denote $\proj$ as the $\ell_q$-norm projection of the origin onto $\bT$, which is uniquely defined for $1 < q < \infty$.


% If $\Pi_{\bT}$ and $\Pi_{\bT^+}$ the $\ell_q$-norm minimizing projection operator onto $\bT$ and $\bT^+$, then the following equals the solution to \eqref{eq:svm-restricted-dual-lp}:\footnote{We include the requirement that $\alpha \neq \vec{0}$ in this formulation without losing the equivalence by noting that \ref{eq:svm-restricted-dual-lp} will never be optimized by $\vec{0}$, because there must always exist some $\alpha$ with strictly positive components such that $\norml[q]{\bA^\T \alpha} \leq 1$.}
% \clayton{Note that projection is uniquely defined if $\bK$ is invertible}

% \begin{equation}
%     \label{eq:projection-lq}
%     \tag{Interpolation Projection}
%     \min_{\alpha \in \mathbb{R}^{n} \setminus \{\zero\}}{ \norm[q]{\bA^\T \frac{\alpha}{\sum_{i=1}^{n}{\alpha_{i}}}} 
%     = \Pi_{\bT}(\vec{0}) }.
% \end{equation}
% \daniel{do you need to require $\sum \alpha_i \neq 0$?} \navid{Well the interpolation primal problem has a  positive optimal objective value so $\sum \alpha_i > 0$ should hold at optimal solutions right? but yes we should mention this condition probably.}

% In order to provide a geometric interpretation of \eqref{eq:projection-lq} let us denote $\mathbf{T}, \mathbf{T}^{+}$ to respectively be the plane passing through and convex hulls of rows of $\bA$. We may then interpret the optimization problem above as a projection of the origin onto the set $\mathbf{T} = \{\sum_{i=1}^{n}{a_{i}\bA_{i}} : \sum_{i=1}^{n}{a_{i}} = 1\} \subset \mathbb{R}^{d}$ using $\ell_{q}$-norm. 

% \textbf{Main Question:} Now that we have all the prerequisites we may form our main question in two alternative point of views roughly as the following:
% \begin{enumerate}
%     \item \label{itm:Q1} Under which settings of input samples the optimal solution to \eqref{eq:svm-restricted-dual-lp} lies within the interior of $\mathbb{R}_{+}^{d}$?
    
%     \item \label{itm:Q2} under which settings of input samples the projection of the origin onto $T$ denoted by $\Pi_{T}(0)$ lies inside $T^{+}$?
% \end{enumerate}





%\begin{equation}
%    \label{eq:svm-dual-l1}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad -\vec{1} \leq \bA\alpha \leq \vec{1} .
%\end{equation}
%
%\begin{equation}
%    \label{eq:svm-dual-l2}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad 1 \leq \alpha^\T \diag(y) \bK \diag(y) %\alpha \leq 1.
%\end{equation}

\begin{restatable}{proposition}{propequiv}\label{prop:equiv}
Let $1 < p < \infty$ and $q = (1-1/p)^{-1}$, and consider any $(\bX,y) \in \R^{n \times d} \times \flip^n$.
Suppose $\bK$ is invertible.
Then, the following are equivalent:
\begin{enumerate}[label=(\arabic*)]
    \item SVP occurs for $\ell_p$-SVM.
    \item The solutions $w$ to \eqref{eq:svm-primal-lp} and \eqref{eq:svm-restricted-primal-lp} are identical.
    \item The optimal solution to \eqref{eq:svm-restricted-dual-lp} lies within the interior of $\R_{+}^{d}$.
    \item $\proj \in \mathbf{T}^{+}$.
\end{enumerate}
Moreover, if $p=2$, then properties (1)--(4) are also equivalent to the following:
\begin{enumerate}[label=(\arabic*)]
    \setcounter{enumi}{4}
    \item  For all $i \in [n]$, $ y_{i} y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \bx_{i} =  y_{i}\projj{i}^\T \bx_{i} / \norml[2]{\projj{i}}^{2} < 1.$
\end{enumerate}
\end{restatable}


This dual framework in (3) and (4) gives an alternative geometric structure to consider for this problem.
For the $\ell_{2}$-case, this formulation draws from the fact that the separating hyperplane obtained from an SVM is represented as a linear combination of support vectors.
Although the $\ell_1$ case is not technically covered by Proposition~\ref{prop:equiv} (due to the non-strict convexity of $\ell_1$ norm), our analysis still gives useful insights, and we explore this case specifically in Section~\ref{sec:l1}. 
%Essentially, we use the fact that $\ell_{1}$-case boils down to a linear program problem where the corner points of the constraint set determine the behaviour of our optimization problem.

We prove Proposition~\ref{prop:equiv} in Appendix~\ref{app:prelim-proof}.
The equivalence between (1) and (5) in the $p=2$ case was proved by \citet[Lemma 1]{hmx20}.
Our alternative proof is based on establishing the equivalence of (4) and (5) and draws heavily from our geometric formulation of SVP.



\subsection{Data model}
We use the data model of \citet{hmx20}, where every labeled sample $(\bx_i, y_i)$ has $\bx_i$ drawn from an anisotropic subgaussian distribution with independent components and arbitrary fixed labels $y_i$.
% \clayton{We should compare our data model to those of \cite{cao2021risk, cl20, wang2021binary, mnsbhs20} as well}
% \todo{Say something about why linear separability won't be a problem for us. Maybe we can say this here and never again worry about $\bK$ being singular again?}

\begin{definition}
    For some $\lambda\in \R_{\geq 0}^d$, we say $(\bX, y) \in \R^{n \times d} \times \flip^n$ (as well as $(\bX,\bZ,y)\in \R^{n \times d} \times \R^{n \times d} \times \flip^n$) is a \emph{$\lambda$-anisotropic subgaussian sample} if:
    $y = (y_1,\dots,y_n) \in \flip^n$ are fixed (non-random) labels;
    $\bZ := [\bz_1 |  \dots | \bz_n]^\T \in \R^{n \times d}$ is a matrix of independent $1$-subgaussian random variables with
    $\EEl{\bz_{i,j}} = 0$ and $\EEl{\bz_{i,j}^2} = 1$; and
    $\bX := [\bx_1 |  \dots | \bx_n]^\T = \bZ \  \diag(\lambda)^{1/2} \in \R^{n \times d}$.
    We say $(\bX,y)$ is an \emph{isotropic subgaussian sample} if it is $\lambda$-anisotropic for $\lambda = (1,\dotsc,1)$.
    Finally, we say $(\bX,y)$ is an \emph{isotropic Gaussian sample} if it is isotropic subgaussian and each $\bx_i \sim \mathcal{N}(0,I_d)$.
\end{definition}
%This data model considers a narrower class of distributions than \cite{cao2021risk, cl20}, which permit linear combinations of draws from product distributions with subgaussian components that obey some variance matrix $\Sigma$.
%We rely on the having samples with independent components when proving the anti-concentration bounds in Lemma~\ref{lemma:e3} needed to prove Theorem~\ref{thm:anisotropic}, which mandates our more restrictive setting.
%It remains open to determine whether our bounds can be proved for this broader class of features.


%The bounds in this paper can also be adapted to consider SVP for infinite-dimensional RKHS features with independent components.
%Because our bounds in Theorem~\ref{thm:anisotropic} depend only on dimension proxies $d_2$ and $d_\infty$, one could consider $d = \infty$ as long as the two proxies are finite.

%We also consider a simpler data model of isotropic Gaussian samples, which allows us to more tightly characterize the SVP threshold in Theorem~\ref{thm:asymptotic}.
%
%\begin{definition}
%    $(\bX, y)$ is an \emph{isotropic Gaussian sample}  if $y = (y_1, \dots, y_n)$ are arbitrary labels that do not depend on $\bX$ and if $\bX := [\bx_1 |  \dots | \bx_n]^\T \in \R^{n \times d}$ is composed of independent samples $\bx_i \sim \mathcal{N}(0, I_d)$.
%\end{definition}
%
%In both models,
We only consider fixed labels $y$ that do not depend on $\bX$. 
However, we do not consider this to be a major limitation of this work.
As discussed before, \citet{cover1965geometrical} shows that linear separability is overwhelmingly likely in the high-dimensional regimes we consider.
Moreover, our results can be extended to a setting where $\by_i = \sign{v^\T{\bx_i}}$ for some fixed weight vector $v$.

\subsection{Previous results}

We tighten and generalize the characterization of the SVP threshold by \citet{hmx20}. 
We give versions of their results that are directly comparable to our results in Sections~\ref{sec:nonasymp} and \ref{sec:asymptotic}.
% \clayton{Is it okay that we rephrase them to have them in terms of $\delta$?}

\begin{theorem}
[Theorem~1 of \cite{hmx20}]%: Upper-bound on SV proliferation threshold for anisotropic subgaussian]
\label{thm:hmx-ub}
    Consider a $\lambda$-anisotropic subgaussian sample $(\bX, y)$ and any $\delta \in (0,1)$.
    If $d_{\infty} = \Omega(n \log (n) \log (\frac{1}{\delta}))$, then SVP occurs for $\ell_2$-SVM with probability at least $1 - \delta$.
\end{theorem}

\begin{theorem}
[Theorem~3 of \cite{hmx20}]%: Lower-bound on SV proliferation threshold for isotropic Gaussian]
\label{thm:hmx-lb}
    Consider an isotropic Gaussian sample $(\bX, y)$.
    For some constant $\delta \in (0,1)$, if $d = O(n)$, then SVP occurs for $\ell_2$-SVM with probability at most $\delta$. 
\end{theorem}

% \todo{unclear what ``with constant prob'' means}\clayton{this ok?} \navid{I think not introducing new constants would help the readability a lot! but if you want to stick to symbols can we maybe use $\delta$ so that it's unified with the previous theorem?}

They note the logarithmic separation between Theorems~\ref{thm:hmx-ub} and \ref{thm:hmx-lb} and the limitations of the data model used in Theorem~\ref{thm:hmx-lb}. 
The authors pose an improvement in generality and asymptotic tightness to their lower-bound as an open problem, which we resolve in the subsequent sections.
% We solve this problem for the $\ell_2$ case here by broadening Theorem~\ref{thm:hmx-lb} to handle $\lambda$-anisotropic samples and by eliminating the logarithmic separation in Theorem~\ref{thm:anisotropic}.
% In addition, we show that the threshold can be precisely captured up to constant factor as $n$ and $d$ trend towards $\infty$ in the isotropic Gaussian setting in Theorem~\ref{thm:asymptotic}.

% \clayton{We can get rid of all of this if we go with Prop~\ref{prop:equiv}}
% We make extensive use of the deterministic equivalence given by \cite{hmx20} and offer an alternate proof of the lemma in the appendix. This new approach could also be useful to extend the results to infinite dimensional Hilbert spaces. 
% \begin{lemma}\label{lemma:hmx-equivalence}
%     For samples $(\bx_1, y_1), \dots, (\bx_n, y_n)\in \R^d \times \flip$ let $T_{\setminus i}$ be the plane passing through $y_{j}\bx_{j}$ for $j \neq i$. Suppose, origin does not belong to $T$ or equivalently $\bK$ is non-singular. Then every training sample is a support vector for the solution to the $\ell_2$ SVM if and only if the following holds:
%     \[ 
%     \langle y_{i}\bx_{i}, y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \rangle = \innerprod{ y_{i}\bx_{i}}{ \frac{\Pi_{T_{\setminus i}}(\vec{0})}{\| \Pi_{T_{\setminus i}}(\vec{0}) \|_{2}^{2}}} < 1 \quad \forall i \in [n]
%     \]
%     In words, both the origin and $y_{i}\bx_{i}$ must lie on the same side of the hyperplane passing $T_{\setminus i}$ with normal vector $\Pi_{T_{\setminus i}}(0)$ for each $i \in [n]$.
% \end{lemma}


==> SVM NeurIPS (3)/supplementary_l1.tex <==
\section{Supplementary material for Section~\ref{sec:l1}}\label{app:l1}

\subsection{$\ell_1$ SVM experimental design}\label{app-sub:l1-exp}
To generate Figure~\ref{fig:l1-l2-compare}, we use $M=400$ Monte Carlo simulations for each pair $(n,d)$ for both $\ell_{1}$ and $\ell_{2}$ SVMs with Gaussian ensemble features $\bX$ and labels $y$ generated identically to what discussed in Appendix~\ref{app:supp-exp}. The range of values of $(n,d)$ for $\ell_{1}$-SVM is within $\{10,11,\dots,70\}\times \{80,85,\dots,1000\}$.
The remainder of the $\ell_1$ experiment is identical to the aforementioned $\ell_2$ experiments.
We determine whether SVP occurs for the $\ell_1$ case by solving the \eqref{eq:svm-dual-l1} linear program for a $\bX$ and $y$ and identifying whether the resulting $\alpha^{*}$ is in $\R_{+}^{n}$. 
We use the linear program solver in CVXOPT~\cite{vandenberghe2010cvxopt} with the default configuration (\texttt{absolute tolerance} $= 10^{-7}$, \texttt{relative tolerance} $= 10^{-6}$, \texttt{feasibility tolerance} $= 10^{-7}$).

\subsection{A geometric interpretation of $\ell_1$ SVM proliferation}\label{app-sub:l1-geometric}

% Throughout the statistics and machine learning literature, $\ell_{1}$ penalties are frequently employed in classification and regression tasks to obtain favorable statistical properties by inducing sparsity \navid{citation needed}. 
% One such application is \emph{exact sparse recovery}, which uses various $\ell_{1}$ methods. 
% In this literature, the model is based on the assumption that there exists an underlying truth for which sparsity assumptions are made. 
% Given a design matrix and a linear observation, one aims to recover the underlying truth by solving a convex optimization problem.
% In \cite{donoho2009counting}, Donoho and Tanner propose a phase transition phenomenon for sparse recovery problem and managed to determine the transition boundary for Gaussian random design matrices. 
% Following that work, \cite{almt14} show that the prevalence of the phase transition phenomena occurring in linear inverse problems are deeply rooted in stochastic geometry by translating optimality conditions into a geometrical question as to whether two cones do share a ray or not. 
% Following along this line, we translate the $\ell_{1}$ SVM into an equivalent linear program that has a meaningful geometric interpretation.
% Most of these results rely heavily on rotational invariant assumptions for theoretical purposes; we also prove a weak upper bound on the rate of the phase transition by taking advantage of these assumptions. 

A persistent line of work in the statistics and machine learning literature studies phenomena with $\ell_1$ constraints by geometrically analyzing the random mathematical programs.
One such application is \emph{exact sparse recovery}, which assumes the existence of a sparse ``ground truth'' that one aims to recover using linear observations by solving a convex optimization problem.
\citet{donoho2009counting} and \citet{almt14} show the existence of a phase transition in this and similar problems by translating the optimality conditions into a geometrical question as to whether two cones share a ray. 
Motivated by this line of work, we believe that Conjecture \ref{main-conjecture} at its core is a geometric phenomenon.
Along those lines, we translate the problem of determining whether $\alpha \in \R_+^n$ into a geometric problem that aims to characterize the faces of a random polytope.

%The problem \eqref{eq:svm-restricted-dual-lp} is the following linear program for data matrix $\bA =\diag(y) \bX \in \R^{n \times d}$:
%\begin{equation}
%    \tag{Dual L1}
%    \label{eq:svm-dual-l1}
%    \begin{aligned}
%    \max_{\alpha \in \R^n} & \quad \sum_{i=1}^{n}{\alpha_{i}}
%    &
%    \text{s.t.} & \quad -\mathbf{1} \leq  \bA^\T \alpha \leq \mathbf{1}.
%    \end{aligned}
%\end{equation}
By the Fundamental Theorem of Linear Programming, the optimal solution(s) to \eqref{eq:svm-dual-l1} lie on corner points of the polytope \[ \mathcal{C}^{*} = \{ \alpha \in \mathbb{R}^{n} : \|\bA^\T \alpha \|_{\infty} \le 1\} \]
in the dual space. 
% We now cast the optimality condition of \eqref{eq:svm-dual-l1} in a geometric way by analyzing the dual polytope of $\mathcal{C}^{*}$. 
The following lemma provides an alternate characterization the optimal solution $\alpha^*$ to the linear program by relating the corner points of $\mathcal{C}^*$ to the faces of its dual polytope, $\mathcal{C}$.

\begin{lemma}
\label{lem:l1-optimality}
 Suppose $\bA \in \mathbb{R}^{n \times d}$ is a full rank matrix for $d > n$. 
 Then $\alpha^{*}$ is an optimal solution to \eqref{eq:svm-dual-l1} iff it is perpendicular to a facet of $\mathcal{C}=\operatorname{Conv}\{\pm \bA_{.,i} : i \in [d]  \}$ which intersects with the ray passing through origin and $\mathbf{1} \in \mathbb{R}^{n}$. 
\end{lemma}

As a result of Lemma~\ref{lem:l1-optimality}, we can determine whether $\ell_1$ support vector proliferation occurs by instead determining whether the ray in the direction of $\one$ passes through a facet of $\mathcal{C}$ whose closest point to the origin lies in $\R_+^n$. 
This reduces the problem to understanding the geometry of the facets of random polytope $\mathcal{C}$. If there are sufficiently many facets relative to $2^n$ and most facets cover a very small number of orthants, then it becomes increasingly likely that the facet intersected by the $\one$ ray will also have its projection from $\zero$ lie in the positive orthant and support vector proliferation is likely to occur. This intuition can be supported from Dvortzky-Milman Theorem \cite{dvoredsky1961some} since for a Gaussian ensemble $\bA$ one expects the convex hull of its columns to be isomorphic to a sphere when $d = \exp\paren{\Omega(n)}$. This geometric approach informs our conjecture that the phase transition is likely to occur at the rate $f(n) = \exp\paren{\Theta(n)}$.

Figure~\ref{fig:l1-example} for a Gaussian Ensemble with $n=2$ and $d=1500$ and illustrates the relationships between $\mathcal{C}$, $\mathcal{C}^*$, $\alpha^*$, and $\bA_{.,i}$. 
The geometric intuition conveyed in the figure is limited by its low value of $n$; we expect qualitatively different behavior to arise when $n$ is large, particularly when considering the geometry of the facets of $\mathcal{C}$.
% because it depicts a situation in the dual space where number of points $d$ (each of which corresponds to a constraint in \eqref{eq:svm-primal-lp}) is exponentially large compared to dimension of the dual space $n$.
For instance, when $n = 2$, very few samples correspond to corners of the convex hull, and the vast majority lie in the interior.
When $n$ is larger, almost all of the samples will be corners of the convex hull, unless $d$ grows exponentially with $n$.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/l1_svm.png}
    \caption{%
    \label{fig:l1-example}%
    Depiction of the dual space. 
        Blue points correspond to rows of a Gaussian ensemble and their reflections with respect to origin, i.e. $\pm \bA_{i,:}$. The outer red convex hull represents $\mathcal{C}$.
        Blue lines are corner points of $\mathcal{C}^{*}$, which are perpendicular to the faces of $\mathcal{C}$, and the black line is the direction of the optimal solution $\alpha^{*}$. 
        Green points indicate the active constraints where the inner product with $\alpha^{*}$ is equal to one.
        }
\end{figure}

To prove Lemma~\ref{lem:l1-optimality}, we make use of several useful facts about the geometric properties of dual polytopes, which are immediate consequences of Farkas' Lemma~\cite[see][]{matousek2013lectures}.

\begin{fact}%[Dual polytopes]
    \label{fact:polytope-duality}
    Let $\mathcal{C} = \operatorname{Conv}\{\pm A_{.,i} : i \in [d]\}$ and $\mathcal{C}^{*}$ defined as above. 
    Then for a full rank matrix $\bA \in \mathbb{R}^{n \times d}$ the following holds:
    \begin{itemize}
        \item The origin $\zero$ is in the interior of $\mathcal{C}$ and $\mathcal{C}^{*}$.
        \item $\mathcal{C} = (\mathcal{C}^{*})^{*} \coloneqq \{\alpha \in \mathbb{R}^{n} : \langle \alpha^{\prime} , \alpha \rangle \leq 1  , \ \forall \alpha^{\prime}  \in \mathcal{C}^{*} \}$, in words $\mathcal{C}$ and $\mathcal{C}^{*}$ are polar.
        \item Corner points of $\mathcal{C}^{*}$ are perpendicular to facets (boundary hyperplanes) of $\mathcal{C}$.
    \end{itemize}
\end{fact}
%\begin{proof}
%The proof is a simple application of Farkas Lemma (see \cite{matousek2013lectures}).
%\end{proof}

Now, we are ready to prove Lemma~\ref{lem:l1-optimality}.

\begin{proof}[Proof of Lemma~\ref{lem:l1-optimality}]
We consider the \eqref{eq:svm-dual-l1} optimization problem and move constraints into the objective for some Lagrange multiplier $\beta \in \mathbb{R}_{+}$:
\[
\max_{\alpha \in \mathbb{R}^{n}}
\mathbf{1}^\T \alpha + \beta\left( 1 - \max_{i \le 2d}{ \bB_{i}^\T \alpha } \right)
\]
where $\bB_{i} = -\bB_{i+d} = \bA_{\cdot,i} \in \R^n$ is the $i$th column of $\bA$.

If $\alpha^*$ is an optimal solution, then zero must be a subgradient of the objective at $\alpha^*$.
Since the set of subgradients of $\alpha \mapsto \max_{i \in [2d]} \bB_i^\T \alpha$ at $\alpha$ is $\operatorname{Conv}\{ \bB_i : i \in I_{\alpha} \}$, where $I_{\alpha} = \{i \in [2d] : \langle \bB_{i}, \alpha \rangle = \max_{i' \in [2d]}{ \langle \bB_{i'}, \alpha \rangle }) \}$ denotes the set of active constraints at $\alpha$, an optimal solution $\alpha^*$ must satisfy
%For some $f: \R^d \to \R$, we let $\partial f(x)$ represent the set of subgradients of $f$ at some $x$.
%Hence for $\alpha^{*}$ an optimal solution to \eqref{eq:svm-dual-l1}, we have: \clayton{Do we need to justify this step, or is it obvious? (Daniel plz help)}
\[
\frac{1}{\beta}\mathbf{1} \in \operatorname{Conv}\{ \bB_{i} : i \in I_{\alpha^{*}}\}.
\] 
This convex hull is a face of $\mathcal{C}$ since $\langle \bB_{j}, \alpha^{*} \rangle < \langle \bB_{i}, \alpha^{*} \rangle = 1$ for any $j \notin I_{\alpha^{*}}$ and $i \in I_{\alpha^{*}}$. 
Moreover, since $\alpha^{*}$ is also a corner point of $\mathcal{C}^{*}$ we have $|I_{\alpha^{*}}| = n$. 
Combining with Fact~\ref{fact:polytope-duality}, we conclude that $\alpha^{*}$ must be perpendicular to the facet of $\mathcal{C}$ that intersects with the ray passing through $\mathbf{1}$. Existence of such a facet is ensured by the fact that origin is in the interior of $\mathcal{C}$. 
\end{proof}


\subsection{Lower-bound on dimension needed for $\ell_1$ SVP}\label{app-sub:l1-loose}
%\clayton{Consider omitting E.3}

Based on the previous relationship between support vector proliferation and the faces of a random convex polytope, we can prove a very loose bound on the minimum dimension $d$ needed for support vector proliferation to occur by bounding the number of faces of the polytope.
When $d = O\paren{n}$, the polytope will have far fewer than $2^{n}$ facets, which makes it impossible for most orthants to to be covered by projections from $\zero$ onto facets. This (along with rotational invariance of the standard Gaussian distribution) allows us to show that support vector proliferation occurs with a negligibly small probability in this regime.

\begin{theorem}\label{thm:weak-ub}
    Let $\bA \in \mathbb{R}^{n \times d}$ be a matrix of i.i.d.~$\mathcal{N}(0,1)$ random variables with $d \geq n$.
    Let $\mathbf{S}$ denote the set of maximizers of \eqref{eq:svm-dual-l1}.
    If $d < C n$ for some universal constant $C>1$, then
    \[
    \limsup_{n \to \infty}{ \pr{\mathbf{S} \cap \operatorname{int}(\mathbb{R}_{+}^{n}) \neq \emptyset }} = 0 
    .
    \]
\end{theorem}

%\todo{Something about uniqueness of Gaussian minimizer to Dual L1}

A key geometric insight for the proof is supplied by \cite{donoho2009counting}.
Let $k^*$ be the maximum integer $k$ such that every $k$ points from among $\{ \pm \bA_{\cdot,i} : i \in [d] \}$ spans a $k$-dimensional face of $\mathcal{C}$ (i.e., their convex hull is a $k$-dimensional face of $\mathcal{C}$).
Then $k^{*}= \Omega_{\mathbf{P}}(\frac{n}{\log(d/n)})$ for large enough values of $n$ and $d$.
Hence, it is plausible to expect that every selection of $n$ points spans a facet of $\mathcal{C}$.

% We use this intuition to prove the following theorem. 
% \navid{This is certainly overselling a simple theorem!!}
%\clayton{I'm a bit confused how this factors in. Should the proof refer back to $k^*$?} \navid{oh no we just use the conclusion to justify our last step in the proof. Otherwise $k^{*}$ is redundant.}


\begin{proof}
Let $F$ denote the facets of $\mathcal{C}$, and to each facet $f \in F$, we associate a corner point $\alpha^{(f)}$ of $\mathcal{C}^*$.
Also let $\bU \in \R^{n \times n}$ denote a uniformly random rotation matrix, independent of $\bA$.
%Let $(\alpha_{i})_{i \le f}$ be the sequence of the corner points of $\mathcal{C}^{*}$ (i.e. perpendicular to facets of $\mathcal{C}$ where $f$ is the total number of facets) and $\bU \in \mathbb{R}^{n \times n}$ a random rotation matrix independent from the initial dataset.
Note that the collection $(\alpha^{(f)})_{f \in F}$ will also have a rotational invariant distribution.
Since $\bA$ has rank $n$ almost surely, Lemma~\ref{lem:l1-optimality} implies that an optimal solution $\alpha^*$ to \eqref{eq:svm-dual-l1} must be one of these corner points $\alpha^{(f)}$.
Thus, we can upper bound the event that any given optimal solution $\alpha^*$ to \eqref{eq:svm-dual-l1} lies in the positive orthant as follows: %\navid{mention about rank}
\begin{align*}
    \pr{\alpha^{*} \in \operatorname{int}(\mathbb{R}_{+}^{n})}
    & \le \pr{
        \bigcup_{f \in F}
        \{ \alpha^{(f)} \in \operatorname{int}(\mathbb{R}_{+}^{n}) \}
    }
    \\
    & =
    \E{
        \pr{
            \bigcup_{f \in F}
            \{ \bU\alpha^{(f)} \subset \mathbb{R}_{+}^{n} \}
            \,\Big\vert\, (\alpha^{(f)})_{f \in F}
        }
    } \\
    & \leq
    \E{
        \sum_{f \in F}
        \pr{
            \{ \bU\alpha^{(f)} \subset \mathbb{R}_{+}^{n} \}
            \,\Big\vert\, (\alpha^{(f)})_{f \in F}
        }
    } \\
    & \le \frac{\E{|F|}}{2^{n}}
    .
\end{align*}
The second inequality is a union bound, and the final inequality uses the fact that $\mathbf{P}[\bU\alpha \in \mathbb{R}_{+}^{n}] = 1/2^{n}$ for any fixed $\alpha$.
A crude upper bound of $\binom{d}{n}$ on the number of facets gives
\[
\mathbf{P}[\alpha^{*} \in \mathbb{R}_{+}^{n}] \le \frac{{d \choose n}}{2^{n}} .
\]
The right-hand side converges to zero as $n \to \infty$ provided that $d < Cn$ for some absolute constant $C \approx 1.29$.
%This probability converges to zero so long as $d < C n$ for some absolute constant $C>1$.
\end{proof}

Needless to say, the gap between Theorem~\ref{thm:weak-ub} and the $\ell_1$ support vector proliferation threshold exhibited in Figure~\ref{fig:l1-l2-compare} is substantial.
Indeed, if Theorem~\ref{thm:weak-ub} were tight, it would imply that support vector proliferation would occur for \emph{smaller} values of $d$ for $\ell_1$ than $\ell_2$, which contradicts our experimental results and geometric intuition.
We believe that union bound corresponding to the first inequality in our proof accounts for that looseness.
That inequality would be tight only if the existence of some $\alpha^{(f)} \in \operatorname{int}(\R_+^n)$ implies that $\alpha^* \in \operatorname{int}(\R_+^n)$; however, this ignores the possibility that facets span many different orthants and that the facet intersecting the ray through $\one$ may be ``close to the origin'' in many orthants simultaneously.
We believe that a more precise understanding of the geometry of the faces of random high-dimensional polytopes could tighten this bound and hence elucidate the $\ell_1$ support vector proliferation phenomenon.


% Specifically, we hypothesize that the number of features $d$ must be exponential in the number of samples $n$ for proliferation to occur and provide a weak \navid{linear} upper bound.
% This conjecture is informed by both experiments that contrast $\ell_1$ from $\ell_2$ and intuition from the geometric framing of the problem. 
% \navid{We defer details surrounding the intuitive justification to the Appendix \ref{app:l1}.}





% \clayton{Some thoughts on high-level structure:

% Since we only have a page or two, I think we want to make sure to prioritize the empirical results, the explicit conjecture, and the most basic geometric intuition.
% An appendix can have the rest, along with various kinds of speculation about why we think this will work.
% Here's a rough outline:

% - Open with the kind of summary I jotted down below that describes what we do and compares it to the $\ell_2$ results. Give the (Dual L1) problem

% - Give our figure that compares $\ell_1$ and $\ell_2$; observe that there's a clear gap between the two and give the conjecture

% - Explain that we think that the gap can be explained by a geometric framing. Give Lemma 8 (without proof) and explain how solving this geometric problem will solve the SV proliferation problem

% - Give a brief summary of what we have in the appendix

% - In the appendix, give further background about \cite{donoho2009counting}; give Lemma 7; prove Lemma 8; explain how one approach involves analyzing the number of faces and give/prove Theorem 9
% }

% \clayton{Problem, conjecture, experiments, geometric intuition}


% Similar to Section \ref{sec:experiments}, we use an empirical simulation by solving \eqref{eq:svm-dual-l1} linear program where $\bA \in \mathbb{R}^{d \times n}$ is a Gaussian ensemble and compare the frequency of support vector proliferation for $\ell_{1}$ with $\ell_{2}$ SVMs. Figure~\ref{fig:l1-l2-compare} demonstrates that $\ell_1$ case requires much larger values of $d$ relative to $n$ for the phase transition to occur. Moreover, the expansion of transition width also suggests that the rate of phase transition may be much larger than $d = \Theta(n \log n)$. 


==> SVM NeurIPS (3)/supplementary_material.tex <==
\section{Supplementary material for Section~\ref{sec:experiments}}
\label{app:supp-exp}

This appendix gives a refined statistical analysis of our hypothesis that SVP is universal for $\ell_{2}$-SVMs under the assumption that features are drawn identically and independently. 
We visually assert this universality with Figures~\ref{fig:heatmap-different-distributions} and \ref{fig:quantiles}, and formally test our hypothesis using a parametric statistical approach, borrowing several ideas from \citet{donoho2009observed}.

% Although, these figures adds non-formal evidence that location of the phase transition is insensitive to sample distributions, but it's rather difficult to design an inferential framework to quantify this claim. 
% To do so, one can opt either a parametric or non-parametric approach. 
%This claim can be formalized using a parametric or non-parametric statistical approach.
As described in Section~\ref{sec:experiments}, we show the significance of this universality by providing a parametric model that complies with the given universality hypothesis and fits well to the observed rates of SVP.
That is, this model permits slight difference for different sample distributions, as long as this difference decays to zero with $n$. 
Furthermore, we show that the model becomes statistically insignificant if we incorporate extra parameters to allow non-decaying dependence on sample distributions to conclude universality.

Alongside these universality results, we experimentally support the universality of the bounds on transition width, which are proved for the isotropic Gaussian sample case in Section~\ref{sec:asymptotic}. 

These analyses are implemented in Python and R. 
Our code-base can be found on Github at \url{https://github.com/scO0rpion/SVM-Proliferation-NIPS2021}.
%%% Submission version
%Our codebase is included in the supplemental material.
%%% arXiv version
% Our codebase is available at \url{https://github.com/scO0rpion/SVM-Proliferation-NIPS2021}.


\subsection{Experimental procedures} 
\label{app:exp-procedure}

We conduct a Monte Carlo simulation in order to validate our theoretical results and grasp their generality to distributions with different tail distributions. 
For the range $(n,d) \in \{40,42,\dots,100\} \times \{100,110,\dots,1000\}$ we study our problem in the following way:
\begin{itemize}
    \item We generate features $\bX \in \mathbb{R}^{n \times d}$ by drawing each $\bx_i$ independently from the suite of distributions shown in Table~\ref{tab:dist}.
    Subsequently, we generate a balanced set of labels $y \in \flip^{n}$ where the first $ \lfloor \frac{n}{2} \rfloor$ samples are assigned class $+1$ and the rest $-1$. 

    \item We used the quadratic program solver from CVXOPT~\cite{vandenberghe2010cvxopt}\footnote{CVXOPT is distributed at \url{https://cvxopt.org/} under a GPLv3 license.} to solve \eqref{eq:svm-restricted-dual-lp} with $p=q=2$ to tolerance level $10^{-7}$.
    
    \item We deem that SVP occurs for an instance of the simulation if the optimizer's output lies in the interior of $\mathbb{R}_{+}^{n}$.

    \item We report the fraction $\hat\bp$ of $M$ trials that exhibit SVP. Based on Figure~\ref{fig:Nsim-sensitivity}, we choose the simulation size value $M=400$ as an appropriate choice for having small enough variance for our range of $(n,d)$. 
    Throughout this section, we run $M = 400$ simulations unless stated otherwise. 
\end{itemize}


%\begin{table}[t]
%    \centering
%    \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%          Uniform & Bernoulli & Rademacher & Laplacian & Gaussian & Gaussian Biased \\
%         \hline
%         Unif$[-1,1]$ & Bernoulli$(\frac{1}{2})$ & Rademacher$(\frac{1}{2})$ & Laplace$(0,1)$ & $\mathcal{N}(0,1)$ & $\mathcal{N}(1,1)$ \\
%         \hline
%    \end{tabular}
%    
%    \smallskip
%    
%    \caption{%
%    \label{tab:dist}
%    The suite of distributions used in experiments. 
%    Features $\bx_i \in \R^d$ are drawn from a product distribution of one of the above}
%\end{table}

\begin{table}[t]
    \centering
    \def\arraystretch{1.2}
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \textbf{Name}
         & \textbf{Support}
         & \textbf{Mean}
         & \textbf{Variance}
         & \textbf{Subgaussian?} \\
         \hline
         Uniform
         & $[-1,1]$
         & $0$
         & $1/3$
         & Yes \\
         \hline
         Bernoulli
         & $\{0,1\}$
         & $1/2$
         & $1/4$
         & Yes \\
         \hline
         Rademacher
         & $\{-1,1\}$
         & $0$
         & $1$
         & Yes \\
         \hline
         Laplacian
         & $\R$
         & $0$
         & $2$
         & No \\
         \hline
         Gaussian
         & $\R$
         & $0$
         & $1$
         & Yes \\
         \hline
         Gaussian Biased
         & $\R$
         & $1$
         & $1$
         & Yes
         \\
         \hline
    \end{tabular}
    
    \smallskip

    \caption{\label{tab:dist}
    The suite of distributions used in experiments.
    Features $\bx_i \in \R^d$ are drawn from a product distribution $\distr^{\otimes d}$ of one of the distributions $\distr$ in this table.}
\end{table}

Our computing environment was a shared high-performance cluster, where a standard node has two Intel Xeon Gold 6226 2.9 GHz CPUs (each with 16 cores) and 192 GB memory.
It took roughly eight hours to run all SVP simulations for $\ell_2$-SVMs on a single node.
The simulations for $\ell_1$-SVMs for Figure~\ref{fig:l1-l2-compare} (Appendix~\ref{app:l1}) took two days to run on the cluster, again just on a single node.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{unnamed-chunk-4-1.pdf}
    \caption{
    \label{fig:Nsim-sensitivity}
    The sensitivity of the experiments to simulation size $M$. 
    The blue curves are 0.1, 0.4, 0.6, and 0.9 quantile contours respectively for the observed rate of SVP for Gaussian samples.
    The red curve is limiting phase transition boundary, i.e., $n \mapsto 2 n \log(n)$}.
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.6]{unnamed-chunk-5-2.pdf}
    \caption{%
    \label{fig:quantiles}%
    Quantile plots. 
    The observed rates of SVP $\hat{\bp}$ are similar for all simulated distributions. 
    The quantile plots visualize the dimension $d$ needed for SVP to occur on a 0.2, 0.4, 0.6, 0.8, and 0.9 fraction of the trials for a fixed umber of samples $n$. %levels curves respectively from below to top for observed success rates. 
    % The right graph reduces the noise of the left by applying non-parametric spline smoothing to the observed rates and computing the same level curves. 
    The red line corresponds to the asymptotic boundary $n \mapsto 2n\log n$, which closely aligns to the level curve corresponding to a 0.8 fraction of trials exhibiting SVP.
    % One can visually observe that level curves are at the same location for all the distributions in our simulation. 
    }
\end{figure}

\subsection{Observed universality}\label{app-sub:universality}

Let $\hat{\mathbf{p}} \coloneqq \hat{\mathbf{p}}(n,d; \distr,M) \sim \text{Binom}(p(n,d; \distr), M)$ be the observed SVP rate corresponding to a sample distribution $\distr$ with independent components and with simulation size $M$. Due to the log-linear dependence of the dimension $d$ of SVP threshold occurs on $n$ from Theorem~\ref{thm:asymptotic}, we parameterize the probability of SVP as a function of $n$ and $\tau \coloneqq \fracl{d}{\paren{2n\log n}}$ instead. The objective here is to provide a reasonable parametric model for $\hat{\mathbf{p}}(n,d; \distr)$ as an inferential tool to test the universality hypothesis. To do so, we translate our universality hypothesis in the language of our parametric model and ensure that necessary statistical assumptions hold to make inferential claims.


\paragraph{Model:} 
We use Probit regression (a generalized linear model with Probit link function) to explain the transition behavior and allow the coefficients to depend explicitly on the distribution $\distr$ under which sample components are drawn from. 
We justify this specific choice of link function at the end of this subsection.
We propose the following parametric model; we motivate the terms in the model at the end of the subsection as well.
\begin{equation}
    \label{eq:model}
    p(n,d ; \distr) = \probit\paren{ \mu^{(0)}(n,\distr) + \mu^{(1)}(n, \distr) \tau + \mu^{(2)}(n,\distr) \log \tau  },
\end{equation}
where
\[
\mu^{(i)}(n, \distr) = \mu^{(i)}_{0}(\distr) + \frac{\mu^{(i)}_{1}(\distr)}{ \sqrt{n} },
\]
and
\[ \probit(t) = \int_{-\infty}^t \frac1{\sqrt{2\pi}} e^{-x^2/2} \operatorname{d}\! x \]
is the Probit link function (i.e., the standard normal distribution function).

% Under the model described by \eqref{eq:model} one can translate the universality hypothesis in a testing framework by requiring $\mu^{(i)}_{0}(\distr)$ to not depend on the underlying distribution $\distr$.
The universality hypothesis can be translated to a testing framework under the model described \eqref{eq:model} by prohibiting $\mu^{(i)}_{0}(\distr)$ from depending on the underlying distribution $\distr$. 
% We tend to generate a stronger universality hypothesis in the following:
% We give two variants of this hypothesis below:
\begin{itemize}
\item \textbf{Universality Hypothesis:} $\mu^{(1)}_0(\distr)$ are identical for each distribution $\distr$, and $\mu^{(1)}_0(\distr) = \mu^{(2)}_0(\distr) = 0$.
        
\item \textbf{Alternative Hypothesis:} $\mu^{(i)}_0(\distr)$ depends on the underlying distribution $\distr$ for some $i \in \{0,1,2\}$.
\end{itemize}

The Universality Hypothesis permits differences from the ground mean (which must decay to zero as $n$ grows large), but requires that other terms be identical.
The Alternative Hypothesis instead permits non-decaying difference among distributions. 
We show that our model \textbf{does not reject} the Universality Hypothesis. 
%In fact we show even more by arguing that $\mu^{(i)}_{1}(\distr)$ also does not depend on $\distr$ for $i=1, 2$. Indeed, we can motivate this model by highlighting a series of observations.

\paragraph{Inference:} We perform Probit regressions on observed SVP rates $\hat{\bp}$ sequentially on three different models, each of which is a sub-model of its successor. 
The second and third models correspond to the Universality Hypothesis and the Alternative Hypothesis respectively.
We compare their goodness-of-fit using analysis of deviance (ANOVA) to assess whether each subsequent model restriction meaningfully improves on its predecessor's ability to fit the data~\cite{hastie2017generalized}.

\begin{itemize}
    \item \textbf{Model~1:} Does not allow any deviations for different distributions; i.e., $\mu^{(i)}(n,\distr)$ does not depend on $\distr$ for $i \in \{0,1,2\}$. 
    \item \textbf{Model~2:} Allows deviations in bias that decay to zero; i.e., only $\mu^{(i)}_{1}(n,\distr)$ may vary with $\distr$.
    \item \textbf{Model~3:} Full model described in Equation~\eqref{eq:model}.
\end{itemize}

\begin{table}[t]
    \centering
    \def\arraystretch{1.2}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \textbf{Models Compared}
    & \textbf{Degrees of Freedom}
    & \textbf{Deviance}
    & \textbf{P-Value} \\
    \hline
    1 vs.~2 & 5 & 1695.46 & $2\cdot10^{-16}$\\
    \hline
    2 vs.~3 & 25 & 29.25  & 0.253 \\
    \hline
    \end{tabular}

    \smallskip

    \caption{%
    \label{tab:anova}%
    Analysis of deviance for the sequence of three Probit models. P-Values are computed based on Chi-squared tails.}
\end{table}

% Note that second and third models correspond to Universality and the Alternative Hypothesis respectively. 
Based on this sequential test given in Table~\ref{tab:anova}, we find that \textbf{Model~1} should be rejected, because \textbf{Model~2} substantially improves on it in a statistically significant manner. 
Furthermore, no statistical significance were detected for rejecting \textbf{Model~2}, and nearly all the excessive parameters (for \textbf{Model~3}) were statistically insignificant.
Therefore, we accept \textbf{Model~2}, which complies with the Universality Hypothesis.

Assuming that the Probit model is well-specified (e.g., the residuals satisfy the usual assumptions), we conclude that \textbf{Model 2} is significant.
The remainder of the section argues that the Probit model is the most appropriate for this setting. 
A full analysis of all three fitted models, including the fitted model parameters and p-values for these parameters, can be found in the code repository.
%In addition to the outcome of this sequential test, we also provide summary tables for second and third models which indicates almost all of excessive parameters in \textbf{Model 3} are insignificant in contrast to \textbf{Model 2}. \navid{How should I include the summaries? just print them?} 

%\clayton{I think we need to say something else about what we're doing precisely before giving the observations. Maybe some sentence like: ``we fit the model for each choice of distribution $\mathcal{D}$ and compare the parameters\dots Figure 5 shows the fitted probit function both  as a function of $\tau$ for fixed $n$ and as a a function of $n$ for fixed $\tau$. The figure illustrates the following\dots''}

%\daniel{we need something to transition to this itemized list \ldots}

\paragraph{Motivating the model:} The proposed model \eqref{eq:model} is supported by a series of  empirical observations about the SVP rate $\hat{\bp}$:

\begin{itemize}
    \item $\hat{\bp}$ increases as $\tau$ increases and is mostly unaffected as $n$ changes (left panel (a) of Figure~\ref{fig:constant-slice}). 
    Therefore, the dependence on $n$ should be negligible.
    \item $\hat{\bp}$ is asymmetric around the theoretical boundary $\tau = 1$ (left panel (a) of Figure~\ref{fig:constant-slice}).
    This behavior motivates the non-linear term in our proposed model and likely originates from the asymmetry of the limiting Gumbel distribution in Section~\ref{sec:asymptotic}. 
    \item As $\tau$ varies, the slope of $n \mapsto p(n,\tau;\distr)$ changes, which motivates including terms that manage the interaction between $n$ and $\tau$ (right panel (b) in Figure \ref{fig:constant-slice}).
    % Right panel (b) in Figure \ref{fig:constant-slice} tends to capture the behaviour of $n \mapsto p(n,\tau;\distr)$ which motivates interaction terms between $n$ and $\tau$ since the slope changes as $\tau$ varies. %It further provides a visual characterization of our claim that interactive terms do not depend on the underlying distribution, i.e. $\mu^{(i)}_{1}(\distr)$ is independent of $\distr$ for $i=1,2$.
    \item As suggested by \citet{donoho2009observed}, including a dependence on $\fracl{1}{\sqrt{n}}$ is motivated by the theory of Edgeworth expansions, which states that the non-asymptotic behaviour of a random Gaussian problem decays to its asymptotic behavior by some power of the ``problem size.''
    % As suggested in \cite{donoho2009observed}, dependence on $\fracl{1}{\sqrt{n}}$ can also be motivated by the Theory of Edgeworth expansions which states that non-asymptotic behaviour of a random Gaussian problem decays with some power of the ``problem size'' to its asymptotic behaviour.
\end{itemize}


\paragraph{Model diagnostics:} 
While our proposed model yields formal evidence of universality, it remains to show that the model is correct, particularly because even wrong models are often statistically significant.
To avoid this pitfall, we validate the underlying assumptions required to make inferential claims in our logistic regression model. 
Figure~\ref{fig:diagnostics} demonstrates that \textbf{Model 2} accurately approximates the observed probabilities $\hat{\bp}$ when the probabilities are not too close to one or zero.\footnote{ 
These extreme cases are not concerning because we are primarily interested in values of $d$ and $n$ where the asymptotic probabilities are non-degenerate. 
The significance of \textbf{Model~2} continues to hold, even if we restricted attention to a smaller region with non-degenerate SVP rates $\hat{\bp}$, such as $\tau \in [0.4,1.6]$.} 
The figure further shows that the residuals approximately follow a standard normal distribution and do not seem to correlate with the fitted values. 
Therefore, the residuals corresponding to this model satisfy the usual assumptions necessary for regression.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.48\textwidth]{unnamed-chunk-10-1.png} &
        \includegraphics[width=0.48\textwidth]{unnamed-chunk-10-2.png} \\
        (a) & (b) \\
    \end{tabular}
    \caption{%
    Diagnostic plots.
    \emph{Left panel (a):} The relationship between logistic regression residuals and fitted probabilities for \textbf{Model 2} applied to the inverse link function. 
    The red curve is LOESS smoothing to illustrate the trend. 
    The observed probabilities drop to zero faster than tails of Probit function.
    \emph{Right panel (b):} Quantile plot of the residuals.
    The red line corresponds to standard normal quantiles.%
    \label{fig:diagnostics}
    }
\end{figure}


\paragraph{Justification for the link function and log:} We test three link functions for \textbf{Model 2} to choose an appropriate one for our parametric model~\eqref{eq:model}:
\begin{align*}
    \operatorname{Cauchit}(t) & = \frac1\pi \left[ \tan^{-1}(t) + \frac\pi2 \right] ,
    & \operatorname{Logit}(t) & = \frac1{1+e^{-t}} ,
    & \operatorname{Probit}(t) & = \Phi(t) .
\end{align*}
%Cauchy, Logit, and Probit, which are built-in functions in R. 
We justify the use of $\log{\tau}$ as a non-linear term in \eqref{eq:model} by substituting the logarithmic term with the \emph{Cox-Box transform} of $\tau$, i.e., $\fracl{\paren{\tau^{\gamma} - 1}}{\gamma}$ and cross-fitting various link functions with different exponents $\gamma = 0.2, 0.4, 0.5, 1$. 
The diagnostic plots in Figure~\ref{fig:appropriate-link-diagnostic-res-vs-fitted} indicate that the Probit link function fits best. 
Moreover, smaller values of $\gamma$ fit observed probabilities better by comparing the deviance r-squares in Table~\ref{table:Rsquared-link} as a measure of goodness of fit. 
Hence, we use the $\log \tau$, which is the limit of the Cox-Box transform when $\gamma \to 0$.

\begin{figure}[t]
    \centering
    \begin{tabular}{cc}
    \includegraphics[width=0.48\textwidth]{regression-1.png}
    &
    \includegraphics[width=0.48\textwidth]{regression-2.png}
    \\
    (a) & (b)
    \end{tabular}
    \caption{
    \label{fig:appropriate-link-diagnostic-res-vs-fitted}
    Diagnostic plots for Gaussian distribution.
    \emph{Left panel (a):} The relationships between the fitted values from logistic regression and the residuals for various link functions and exponents. We use LOESS smoothing to visualize the trend and plot it in blue. Asymptotically, the residuals should appear independent of the fitted values; hence, bumpy blue curves indicate non-compliant behaviour with model assumptions.
    \emph{Right panel (b):} Residual QQ-plots. One expects residuals to asymptotically follow a normal distribution (with a perfect fit corresponding to the overlaid red line), so smaller deviations from a normal distribution is desired.}
\end{figure}


\begin{table}[t]
    \centering
    \def\arraystretch{1.2}
\begin{tabular}{cc|c|c|c|}
\cline{3-5}
\multicolumn{1}{l}{}                                         & \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{\textbf{Link}}                  \\ \cline{3-5} 
\multicolumn{1}{l}{}                                         & \multicolumn{1}{l|}{} & \textbf{Cauchit} & \textbf{Logit} & \textbf{Probit} \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{$\boldsymbol{\gamma}$}} & \textbf{0.10}         & 0.9606           & 0.9953         & 0.9971          \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \textbf{0.25} & 0.9602 & 0.9950 & 0.9969 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \textbf{0.50} & 0.9595 & 0.9946 & 0.9967 \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \textbf{1.00} & 0.9501 & 0.9771 & 0.9722 \\ \hline
\end{tabular}


%    \begin{tabular}{|ccc|c|c|}
%        \hline
%        & & \multicolumn{3}{c|}{\textbf{Link}} \\
%        \cline{3-5}
%        & & \multicolumn{1}{|c|}{\textbf{Cauchit}} & \textbf{Logit} & \textbf{Probit} \\
%        \cline{2-5}
%        \multirow{4}{*}{$\boldsymbol{\gamma}$} &
%        \multicolumn{1}{|c|}{\textbf{0.10}} & 0.9606 & 0.9953 & 0.9971\\
%        \cline{2-5}
%        & \multicolumn{1}{|c|}{\textbf{0.25}} & 0.9602 & 0.9950 & 0.9969\\
%        \cline{2-5}
%        & \multicolumn{1}{|c|}{\textbf{0.50}} & 0.9595 & 0.9946 & 0.9967\\
%        \cline{2-5}
%        & \multicolumn{1}{|c|}{\textbf{1.00}} & 0.9501 & 0.9771 & 0.9722\\
%        \hline
%    \end{tabular}
    
    \smallskip
    
    \caption{%
    \label{table:Rsquared-link}
    $R^{2}$ values computed from on the fraction between the null deviance and the fitted deviance for different link functions and exponents. The Probit link function with  $\gamma=0.1$ has the best fit.}
\end{table}


\subsection{Width of transition}\label{app-sub:width}

\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.7]{unnamed-chunk-6-1.pdf}
    \caption{
    \label{fig:transition-width}
    The estimated scaled transition widths for variety of distributions. 
    Note that $\hat{\tau}_{q}$ and $\hat{\tau}_{1-q}$ are computed with both observed probabilities and non-parametric smoothing spline versions of probabilities which are shown in left and right panels respectively.
    The overall trend is overlaid using a linear regression applied to the scale width.}
\end{figure}

To estimate the width of the phase transaction, we adopt a non-parametric approach. 
For $q < \fracl{1}{2}$ and fixed $n$ we define the \emph{$q$-transition zone} to be the range $[\tau_{q},\tau_{1-q}]$, where $\tau_q$ and $\tau_{1-q}$ correspond to the ratio $\fracl{d}{\paren{2n \ln n}}$ for smallest and largest value of $d$ where support vector proliferation occurs with probability $q$ and $1-q$ respectively. In other words, within this range, the corresponding probabilities are inside $[q, 1-q]$ interval. 

Formally, we define \emph{scaled $q$-transition width estimate} as,
\[
\hat{w}_{q}(n,d) = \frac{ \hat{\tau}_{1-q} - \hat{\tau}_{q} }{ \probit^{-1}(1-q) - \probit^{-1}(q) } \sqrt{\log n},    
\]
where $\probit$ is the Probit link function introduced in \eqref{eq:model} and $\hat{\tau}_{q}$ and $\hat{\tau}_{1-q}$ are plug-in estimates of $\tau_{q}$ and $\tau_{1-q}$.  
We plot $\hat{w}_{q}(n,d)$ with $n$ in Figure~\ref{fig:transition-width}.

%Figure~\ref{fig:transition-width} illustrates a downward trend for the \emph{scaled 0.1-transition width estimate} which can be interpreted as $\hat{w}_{q}(n,d) = o\paren{1}$. \navid{I guess we don't want this right?}
%Equivalently, the non-scaled transition width is $o\paren{n \sqrt{\log n}}$.




%\subsection{Figures and Tables}








==> SVM NeurIPS (3)/supporting_lemmas.tex <==
\section{Proofs for Section~\ref{sec:asymptotic}}\label{app:lemmas}

We prove Theorem~\ref{thm:anisotropic}, which we restate below.

\thmanisotropic*

\begin{proof}%[Proof of Theorem~\ref{thm:anisotropic}]

As discussed in Section~\ref{sec:nonasymp}, it suffices to prove that $\bK_{\setminus i}$ is invertible for all $i$ and
\[
\max_{i \in [m]} \bracket{y_i y_{\setminus i}^\T \paren{\bK_{\setminus i}^{-1}-\frac{1}{\norm[1]{\lambda}} I_{n-1}} \bX_{\setminus i} \bx_i 
+ \frac{1}{\norm[1]{\lambda}}y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i 
+ \frac{1}{\norm[1]{\lambda}}y_i y_{\setminus [m]}^\T \bX_{\setminus [m]} \bx_i} \geq 1
\]
with probability $1-\delta$ for some $m \leq n$.
We do so by showing that the following three events each hold with probability $1 - \frac{\delta}{3}$:
\begin{align*}
    &\max_{i \in [m]} \abs{y_i y_{\setminus i}^\T \paren{\bK_{\setminus i}^{-1}-\frac{1}{\norm[1]{\lambda}} I_{n-1}} \bX_{\setminus i} \bx_i} \leq 1, \\
    &\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}} \abs{y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i} \leq 1,  \ \text{and} \\
    &\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}}y_i y_{\setminus [m]}^\T \bX_{\setminus [m]} \bx_i \geq 3.
\end{align*}

It remains to plug in the results of Lemmas~\ref{lemma:e1}, \ref{lemma:e2}, and \ref{lemma:e3} to show that the three events occur with high probability given the conditions imposed on $n$, $d_2$, $d_{\infty}$, and $\delta$ in \eqref{eq:3}.
Let $m := \ceill{\exp(\frac{d_2}{2\Cb n})}$. 
By \eqref{eq:3}, $m \leq \sqrt{n}+1 \leq \frac{n}{\ln n} \leq \frac{n}{2}$ for sufficiently small constant $\Ca$.

%\todo{Make more explicit why these inequalities work; copy from note in the reviews: \url{https://openreview.net/forum?id=9bqxRuRwBlu}.}\clayton{Are these ok?}

\begin{enumerate}
    \item 
    By Lemma~\ref{lemma:e1} in Appendix~\ref{asec:e1} with $\delta := \frac{\delta}{3m}$, it follows that for any fixed $i \in [m]$, $\bK_{\setminus i}$ is invertible and
    \[\abs{y_i y_{\setminus i}^\T \paren{\bK_{\setminus i}^{-1} - \frac{1}{\norml[1]{\lambda}} I_{n-1} } \bX_{\setminus i} \bx_i } \leq 1\] with probability at least $1 - \frac{\delta}{3m}$ as long as the following conditions hold:
    \begin{align}
      d_{\infty} & \geq \cc'\paren{n\paren{\log\frac{3m}{\delta}}^{1/3} + n^{1/3} \log \frac{3m}{\delta}} ,
      \label{eq:proof-anisotropic-cond1}
      \\
      d_2 d_{\infty} & \geq \cd n \log \frac{3m}{\delta} \paren{n + \log \frac{3m}{\delta}}.
      \label{eq:proof-anisotropic-cond2}
    \end{align}
    We show that the inequalities in
    \eqref{eq:proof-anisotropic-cond1}
    and
    \eqref{eq:proof-anisotropic-cond2}
    are implied by the preconditions of Theorem~\ref{thm:anisotropic} in
    \eqref{eq:3} by choosing sufficiently large constants $C_1$, $C_3$, and $C_4$.
    For \eqref{eq:proof-anisotropic-cond1},
    \begin{align*}
        n \paren{\log \frac{3m}{\delta}}^{1/3} + n^{1/3} \log \frac{3m}{\delta} 
        &\leq n \paren{\frac{d_2}{C_2 n} + \log \frac{3}{\delta}}^{1/3} + n^{1/3}\log \frac{3n}{2\delta} \\
        &\leq \frac{n^{2/3}d_2^{1/3}}{C_2}  + n \paren{\log\frac{3}{\delta}}^{1/3}  + n \log \frac{3}{\delta} \\
        &\leq \frac{n^{1/3} d_\infty^{2/3}}{C_2 C_4^{1/3}}+ 2 n \log \frac{3}{\delta} ,
    \end{align*}
    which implies the desired inequality.
%    We conclude by applying the third inequality of \eqref{eq:3}.
    To establish \eqref{eq:proof-anisotropic-cond2}:
%    The second inequality is similar:
% 
    \begin{align*}
        n \log \frac{3m}{\delta} \paren{n + \log \frac{3m}{\delta}}
        &\leq \frac{d_2}{C_2} \paren{n + \log \frac{3n}{2\delta}} 
        \leq  \frac{d_2}{C_2} \paren{2n + \log \frac{1}{\delta}} \leq \frac{d_2}{C_2} \cdot \frac{3d_\infty}{C_3}.
    \end{align*}
    
    % which can be ensured by choosing large enough constants $\Ca$, $\Cc$, and $\Cd$.
    By applying a union bound to all $m$ events, they all occur with probability at least $1 - \frac{\delta}{3}$.

	\item 
	By applying Lemma~\ref{lemma:e2} in Appendix~\ref{asec:e2} for all $i \in [m]$ with $\delta$ as before and union-bounding over the corresponding events, with probability $1  - \frac{\delta}{3}$, \[\frac{1}{\norml[1]{\lambda}}   y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i \geq -1\] for all $i \in [m]$ as long as
	 \[d_2 \geq \ca m \log \frac{3m}{\delta}
	 \quad \text{and} \quad 
	 d_\infty \geq \cb \sqrt{m} \log \frac{3m}{\delta}.
    \]
    % which follows from the definition of $m$ for sufficiently large $\Cc$ and $\Cd$.
    Both inequalities follow from the third inequality of \eqref{eq:3} for sufficiently large $C_3$ and by $m \leq \frac{n}{\log n}$.

	\item By Lemma~\ref{lemma:e3} in Appendix~\ref{asec:e3} with $t := 3$, 
	\[\max_{i \in [m]} \frac{1}{\norml[1]{\lambda}} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i \geq 3\]
	with probability $1 - \frac{\delta}{3}$, if
	\begin{align*}
	     & n-m \geq \ca \paren{\log \frac{3}{\delta}}^2, &&
     \exp\paren{\frac{9 d_2}{\cb (n-m)}} \leq m \leq (n-m), \\
    & d_2 \geq \cc (n-m) \log \log \frac{3}{\delta},
    && \text{and} \quad
    d_{\infty}^2 \geq\cd d_{2} (n-m).
    \end{align*}
    The inequalities are satisfied as immediate consequences of \eqref{eq:3} and the fact that $m = \ceill{\exp(\frac{d_2}{2C_2n})} \leq \frac{n}{2}$ for sufficiently small $C_2$. \qedhere
    % follows by the definition of $m$ and by choosing sufficiently large absolute constants.\qedhere
\end{enumerate}
\end{proof}

In the subsequent three sections, we prove Lemmas~\ref{lemma:e1}, \ref{lemma:e2}, and \ref{lemma:e3}.



\subsection{Bounded difference between leave-one-out terms with $\bK^{-1}$ and scaled identity}\label{asec:e1}

\begin{lemma}\label{lemma:e1}
    Let $(\bX, y) \in \R^{n \times d} \times \R^n$ and $(\bx', y') \in \R^{d} \times \R$ be $\lambda$-anisotropic subgaussian samples that are independent of one another with $\bK = \bX \bX^\T$.
    Pick any $\delta \in (0, \frac{1}{2})$.
    There exist universal constants $\cc, \ccc$ such that if $d_{\infty} \geq \cc(n + \log \frac{1}{\delta})$,
    then with probability $1 - \delta$, $\bK$ is invertible and
    \[\abs{y^\T \paren{\bK^{-1} - \frac{1}{\norm[1]{\lambda}} I_{n}} \bX \bx' } \leq c\sqrt{\frac{n \log \frac{1}{\delta}}{d_{\infty}}}\paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}}.\]
\end{lemma}
\begin{remark}
    To guarantee that $\absl{y^\T \parenl{\bK^{-1} - \norm[1]{\lambda}^{-1} I_{n}} \bX \bx' } \leq \eps$
    with probability $1 - \delta$ for some $\eps > 0$,
    it suffices to show that 
    \[d_\infty \geq \cc' \cdot \frac{n \paren{\log \frac{1}{\delta}}^{1/3} + n^{1/3} \log \frac{1}{\delta}}{\eps^{2/3}} 
    \quad \text{and} \quad
    d_2 d_\infty \geq \cd \cdot \frac{n \log \frac{1}{\delta} \paren{n + \log \frac{1}{\delta}}}{\eps^2},\]
    for universal constants $\cc'$ and $\cd$.
\end{remark}

The proof of Lemma~\ref{lemma:e1} relies heavily on a concentration bound on the eigenvalues of the Gram matrix $\bK$, which draws from a technical lemma of \citet{hmx20}. 
We present and prove this result below and then use it to prove Lemma~\ref{lemma:e1}.

\begin{lemma}\label{lemma:gram-evals}
	Let $(\bX, y) \in \R^{n \times d} \times \R$ be $\lambda$-anisotropic subgaussian samples with Gram matrix $\bK := \bX \bX^\T \in \R^{n \times n}$.
	Pick any $\delta \in (0, \half)$.
	For some universal constant $\ccc$, with probability $1-\delta$,
	\begin{equation}
	\label{eq:K-norm-bound}
	    \normop{\bK - \norm[1]{\lambda} I_n} \leq \ccc \norm[1]{\lambda} \paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}} ,
	\end{equation}
  where $\normop{\cdot}$ denotes the spectral (operator) norm.
	If additionally $d_\infty \geq \cc (n + \log \frac{1}{\delta})$ for some universal constant $\cc$, then for the same event, $\bK$ is invertible and
  %\todo{clarify that this is spectral norm} \navid{should we use operational norm? $\| \|_{op}$}
	\begin{equation}
	\label{eq:Kinv-norm-bound}
	\norm{\bK^{-1} - \frac{1}{\norm[1]{\lambda}} I_n} \leq  \frac{\ccc}{\norm[1]{\lambda}} \paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}} .
	\end{equation}
\end{lemma}
\begin{proof}

Equation~\eqref{eq:K-norm-bound} follows from Lemma~8 of \citet{hmx20}.
For some universal constant $\cp$ and sufficiently large $\ccc$, we have the following:
\begin{align*}
    &\pr{ \normop{\bK - \norm[1]{\lambda} I_n} \geq \ccc \norm[1]{\lambda} \paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}}}\\
    &\quad\leq 2 \cdot 9^n \cdot \exp\paren{-\cp\min\paren{\frac{\ccc^2\norm[1]{\lambda}^2(n + \log \frac{1}{\delta})}{\norm[2]{\lambda}^2 d_2},\frac{\ccc\norm[1]{\lambda}(n + \log \frac{1}{\delta})}{\norm[\infty]{\lambda} d_{\infty}}}}\\
    &\quad \leq 2 \exp\paren{n\log 9 - \cp \min(\ccc^2, \ccc) \paren{n + \log \frac{1}{\delta}}} \leq \delta.
\end{align*}

If equation~\eqref{eq:Kinv-norm-bound} holds and $\cc$ is sufficiently large, then all eigenvalues of $\bK$ are strictly positive and $\bK$ is invertible.
We now derive equation~\eqref{eq:Kinv-norm-bound} by bounding the eigenvalues of $\bK^{-1}$, assuming that the event in equation~\eqref{eq:K-norm-bound} occurs, and rescaling $\ccc$:
\begin{align*}
\lefteqn{
    \normop{\bK^{-1} - \frac{1}{\norm[1]{\lambda}} I_n}
    } \\
    &\leq \max\paren{\mu_{\max}(\bK^{-1}) - \frac{1}{\norm[1]{\lambda}}, - \mu_{\min}(\bK^{-1}) + \frac{1}{\norm[1]{\lambda}}} \\
    &= \max\paren{\frac{1}{\mu_{\min}(\bK)} - \frac{1}{\norm[1]{\lambda}}, - \frac{1}{\mu_{\max}(\bK)} + \frac{1}{\norm[1]{\lambda}}} \\
    &\leq \frac{1}{\norm[1]{\lambda}} \max\paren{\frac{1}{1 - \ccc  \paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}}} - 1, 1- \frac{1}{1 + \ccc  \paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}}}} \\
    &\leq \frac{1}{\norm[1]{\lambda}}\cdot 2\ccc\paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}}.\qedhere
\end{align*}
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lemma:e1}]
Conditioned on $\bX$, $y^\T (\bK^{-1} - \norml[1]{\lambda}^{-1} I_{n}) \bX \bx'$ is a univariate subgaussian random variable with mean 0 and variance proxy at most $\norml{y^\T (\bK^{-1} - \norml[1]{\lambda}^{-1} I_{n}) \bX}^2 \norml[\infty]{\lambda}$, as long as $\bK$ is invertible.
We bound the variance proxy and show that $\bK$ is invertible with high probability by applying Lemma~\ref{lemma:gram-evals} for some universal $\cp$ with probability $1 - \frac{\delta}{2}$:
\begin{align*}
    \norm{y^\T (\bK^{-1} - \frac{1}{\norm[1]{\lambda}} I_{n}) \bX}^2 \norm[\infty]{\lambda}
    &\leq \norm[2]{y}^2 \norm{\bK^{-1} - \frac{1}{\norm[1]{\lambda}} I_{n}}^2 \norm{\bK} \norm[\infty]{\lambda} \\
    &\leq n \cdot \frac{\cp}{\norm[1]{\lambda}^2} \paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}}^2 \cdot 2 \norm[1]{\lambda} \norm[\infty]{\lambda} \\
    &=  \frac{2\cp n}{d_\infty} \paren{\sqrt{\frac{n + \log \frac{1}{\delta}}{d_2}} + \frac{n + \log \frac{1}{\delta}}{d_\infty}}^2 
\end{align*}
    We observe that the bound holds for a proper choice of $\ccc$ for a standard concentration bound for a subgaussian random variable.
\end{proof}




\subsection{Concentration of leave-one-out terms}\label{asec:e2}


\begin{lemma}\label{lemma:e2}
    Let $(\bX, \bZ, y) \in \R^{n \times d} \times \R^{n \times d} \times \R^n$ and $(\bx', \bz', y') \in \R^d \times \R^{d} \times \R$ be $\lambda$-anisotropic subgaussian samples that are independent of one another.
    Pick any $\delta \in (0, \half)$.
    There exists a universal constant $\ccc$ such that with probability $1 - \delta$,
    \[\frac{1}{\norm[1]{\lambda}} \abs{y^\T \bX \bx'} \leq c \paren{\sqrt{\frac{n \log \frac{1}{\delta}}{d_2}} + \frac{\sqrt{n} \log \frac{1}{\delta}}{d_\infty}}.\]
\end{lemma}
\begin{remark}
    To ensure that $\norm[1]{\lambda}^{-1} \absl{y^\T \bX \bx'} \leq \eps$ with probability $1 - \delta$ for some $\eps > 0$, it suffices to show that
    \[d_2 \geq \frac{\ca n \log \frac{1}{\delta}}{\eps^2}
    \quad \text{and} \quad
    d_\infty \geq \frac{\cb \sqrt{n} \log \frac{1}{\delta}}{\eps}\]
    for universal constants $\ca, \cb$.
\end{remark}

% The proof relies on the following fact, which we give and prove.

% \begin{fact}\label{fact:subexp}
%     Let $\bx$ and $\by$ be independent 1-subgaussian random variables with $\EEl{\bx} = \EEl{\by} = 0$.
%     Then, $\bx \by$ is $(8,2)$-subexponential.
% \end{fact}
% \begin{proof}
%     We bound the moment generating function for $\bx \by$. 
%     For any fixed $\eta \in \R$:
%     \begin{align*}
%         \EE{\exp(\eta\bx\by) }
%         &= \EE{\EE{\exp(\eta\bx\by) \mid \by}} 
%         \leq \EE{\exp\paren{\frac{\eta^2 \by^2}{2}}}
%         = \EE{\sum_{k=0}^\infty \frac{1}{k!} \paren{\frac{\eta\by}{\sqrt{2}}}^{2k}}  \\
%         &= \sum_{k=0}^\infty \frac{1}{k!} \paren{\frac{\eta}{\sqrt{2}}}^{2k} \EE{\by^{2k}}
%         \leq \sum_{k=0}^\infty \frac{1}{k!} \paren{\frac{\eta}{\sqrt{2}}}^{2k} \cdot k! 2^{2k} 
%         = \sum_{k=0}^\infty \paren{2\eta^2}^{k}.
%     \end{align*}
%     If $\eta \leq \frac{1}{2}$, then we can bound the above term:
%     \begin{align*}
%         \EE{\exp(\eta\bx\by) }
%         &\leq \frac{1}{1- 2\eta^2}
%         = 1 + \frac{2\eta^2}{1- 2\eta^2}
%         \leq 1 + 4 \eta^2 
%         \leq \exp\paren{\frac{8\eta^2}{2}}.
%     \end{align*}
%     Thus, $\bx\by$ is $(8,2)$-subexponential.
% \end{proof}

% \begin{proof}[Proof of Lemma~\ref{lemma:e2}]
\begin{proof}
    We can rewrite $y^\T \bX \bx'$ for some vector of 1-subgaussian random variables $\tilde{\bz} \in \R^d$.
    \begin{align*}
        y^\T \bX \bx'
        &= y^\T \bZ \diag(\lambda) \bz'
        = \sqrt{n} \tilde{\bz}^\T \diag(\lambda) \bz'
        = \sqrt{n} \sum_{i=1}^d \lambda_i \tilde{\bz}_i \bz'_i.
    \end{align*}
    % By Fact~\ref{fact:subexp}, each $\tilde{\bz}_i \bz'_i$ is an independent $(8,2)$-subexponential random variable.
    % Thus, $\sum_{i=1}^d \lambda_i \tilde{\bz}_i \bz'_i$ is $(8 \norml[2]{\lambda}^2, 2 \norml[\infty]{\lambda})$-subexponential, and with probability $1 - \delta$,
    By Lemma~2.7.7 of \cite{vershynin14}, each $\tilde{\bz}_i \bz'_i$ is an independent $(1,2)$-subexponential random variable.
    Thus, $\sum_{i=1}^d \lambda_i \tilde{\bz}_i \bz'_i$ is $( \norml[2]{\lambda}^2, 2 \norml[\infty]{\lambda})$-subexponential, and with probability $1 - \delta$,
    \[\abs{ y^\T \bX \bx'} \leq \sqrt{n} \ccc \paren{\sqrt{\norm[2]{\lambda}^2 \log \frac{1}{\delta}} + \norm[\infty]{\lambda} \log \frac{1}{\delta}}.\]
    We have the claim by dividing by $\norml[1]{\lambda}$.
\end{proof}


\subsection{Anti-concentration for independent leave-one-out terms}\label{asec:e3}

% \begin{lemma}\label{lemma:e3}
%   Let $(\bX,\bZ,y) \in \R^{n \times d} \times \R^{n \times d} \times \R^n$
%   and
%   $(\bX',\bZ',y') \in \R^{m \times d} \times \R^{m \times d} \times \R^m$
%   be $\lambda$-anisotropic subgaussian samples that are independent of each other.
%   Pick any $t>0$ and $\delta \in (0, \half)$. 
%     For universal constants $\ca$, $\cb$, $\cd$, and $\ce$, if 
%     \[
%     n \geq \ca \log \frac{1}{\delta},
%     \quad
%      \exp\paren{\frac{t^2 d_2}{\cb n}} \leq m \leq n,
%     \quad
%     d_2 \geq \cc n \log \log \frac{1}{\delta},
%     \quad \text{and} \quad
%     d_{\infty}^2 \geq\cd d_{2} n,\]
%     then with probability $1 - \delta$
%     \[\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}}  y^\T \bX \bx_i' \geq t.\]
% \end{lemma}


% \begin{proof}
% \newcommand{\bxig}{\text{$\bX$ is good}}
% \newcommand{\bxing}{\text{$\bX$ is not good}}


% Let $\bq_{j} := \norml[1]{\lambda}^{-1} y^\T \bZ_{\cdot, j}$ for all $j \in [d]$, where $\bZ_{\cdot, j} = (\bz_{1,j}, \dots, \bz_{n,j}) \in \R^n$.
% Note that 
% \[\frac{1}{\norm[1]{\lambda}}  y^\T \bX \bx_i' = \sum_{j=1}^d  \bq_{j} \lambda_j  \bz_{i,j}'\] and all $\bq_{j}$ and $\bz_{i,j}'$ are independent and that $\bq_j$ is subgaussian with variance proxy $\fracl{n}{\norml[1]{\lambda}^2}$.
% The proof of the claim is powered by the Berry-Esseen theorem and comes in two parts:
% \begin{itemize}
%     \item We first show that $\bX$ is well-behaved with high probability; we say that $\bX$ is \emph{good} if the following hold:
%     \begin{equation}\label{eq:good-max}
%          \max_j \abs{\lambda_j \bq_j} \leq c_0 \sqrt{\frac{\log n}{d_2}},
%     \end{equation}
%     \begin{equation}\label{eq:good-norm}
%          \sum_{j=1}^d \lambda_j^2 \bq_j^2 \geq \frac{n}{16 d_2}.
%     \end{equation}
%     We prove that $\prl{\bxig} \geq 1 - \frac{2\delta}{3}$.

%     \item 
%     Then, we use the Berry-Esseen Theorem to show that, for each $i \in [m]$,
%     \[\pr{\frac{1}{\norm[1]{\lambda}} y^{\T} \bX \bx_i' \leq t \mid \bxig } \leq \paren{\frac{\delta}{3}}^{1/m} . \] %for all $i \in [m]$ if $\bX$ is good. 
% \end{itemize}
% Because $\norm[1]{\lambda}^{-1} y_i' y^\T \bX \bx_i'$ for $i \in [m]$ are conditionally independent given $\bX$, we obtain the desired statement:
% \begin{align*}
%     \pr{\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}} y_i' y^\T \bX \bx_i' \leq t}
%     &\leq \pr{\bxing} + \pr{\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}} y_i' y^\T \bX \bx_i' \leq t \mid \bxig} \\
%     & \leq \frac{2\delta}{3} + \prod_{i=1}^m \pr{ \frac{1}{\norm[1]{\lambda}} y_i' y^\T \bX \bx_i' \leq t \mid \bxig} \leq \delta .
% \end{align*}


% \paragraph{$\bX$ is good with high probability.}
% To prove both bounds necessary to show that $\bX$ is good, we introduce a different sequence of random variables $\br_1, \dots, \br_{\ell}$ for some $\ell \in [n, 2n]$ to eliminate any dependence on $d$.
% Set $0 = k_0 < k_1 < \dots < k_{\ell} = d$ such that for all $i \in [\ell]$, 
% \[\sum_{j=k_{i-1}+1}^{k_{i}} \lambda_j^2 \in  \bracket{\frac{\norm[2]{\lambda}^2}{2\ell}, \frac{\norm[2]{\lambda}^2}{\ell}}.\]
% Such a partition is possible because we can require that $\norml[\infty]{\lambda}^2 \leq \fracl{\norml[2]{\lambda}^2}{\ell}$, which follows by requiring that $\cd \geq 2$.
% Let \[\br_i = \sum_{j=k_{i-1}+1}^{k_{i}} \lambda_j^2 \bq_j^2\] for all $i \in [\ell]$. 
% Note that all $\br_i$ are independent and that \[\sum_{j=1}^d \lambda_j^2 \bq_j^2 = \sum_{i=1}^{\ell} \br_i.\] 
% Because $\EEl{\bq_j} = 0$ and $\EEl{\bq_j^2} = \fracl{n}{\norml[1]{\lambda}^2}$, we can bound $\EEl{\br_i}$:
% \[	\EE{\br_i} 
% 		\in \bracket{\frac{n\norm[2]{\lambda}^2}{2 \ell \norm[1]{\lambda}^2}, \frac{n\norm[2]{\lambda}^2}{ \ell \norm[1]{\lambda}^2}} 
% 		\subseteq \bracket{\frac{1}{4d_2}, \frac{1}{d_2}}. \]
		
% We upper-bound $\max_j \absl{\lambda_j \bq_j}$ by noting that $\max_j \absl{\lambda_j \bq_j} \leq \max_i \sqrt{\br_i}$.
% Note that the quantity $\sqrt{\br_i}$ is subgaussian with variance proxy $\EE{\br_i} \leq \fracl{1}{d_2}$.
% By a standard concentration argument for $n \geq 2$ from \cite{vershynin14},
% % \clayton{Should I mention that this comes from Exercise 2.5.10?}, 
% \[\pr{\max_{i\in [n]} \sqrt{\br_i} \leq \cp \sqrt{\frac{\ln (n)}{d_2}}} \geq 1 - \frac{\delta}{3}\]
% for some absolute constant $\cp$.

% \clayton{Replace this with Hanson-Wright}
% The lower-bound on $\sum_{j=1}^d \lambda_j^2 \bq_j^2 = \sum_{i=1}^{\ell} \br_i$ is more involved.
% We upper-bound the variance of each $\br_i$ with Chebyshev's inequality, and apply a Chernoff bound to show that sufficiently many of the $\br_i$ terms are sufficiently large.
% To bound the variance of $\br_i$, we first compute the fourth moment of $\bq_j$.
% Because every $\bz_{i,j}$ is sub-Gaussian, let $\EEl{\bz_{i,j}^4} \leq \omega = O(1)$.
% \[\EEl{\bq_j^4} \leq \frac{n \omega +  n(n-1)}{\norm[1]{\lambda}^4} = \frac{n(\omega -1) + n^2}{\norm[1]{\lambda}^4}.\]
% Then, if $n$ is sufficiently large such that $n \geq 256 \omega = \Omega(1)$,
% 	\begin{align*}
% 		\Var{\br_i}
% 		&= \sum_{j=k_{i-1}+1}^{k_i } \lambda_j^4 \paren{\EE{\bq_j^4} - \EE{\bq_j^2}^2} 
% 		= \frac{n(\omega -1)}{\norm[1]{\lambda}^4} \sum_{j=k_{i-1}+1}^{k_i} \lambda_j^4 \\
% 		&\leq \frac{n^2}{256\norm[1]{\lambda}^4} \paren{\sum_{j=k_{i-1}+1}^{k_i } \lambda_j^2}^2 
% 		\leq \frac{n^2}{256 d_2^2 \ell^2} \leq \frac{1}{256 d_2^2}.
% 	\end{align*}

% 	We apply Chebyshev's inequality and obtain a lower-bound on every $\br_i$.
% 	\begin{align*}
% 		\pr{\br_i \leq \frac{1}{8 d_2}}
% 		&\leq \pr{\abs{\br_i - \EE{\br_i}} \geq \frac{1}{8 d_2}} \\
% 		&\leq  \pr{\abs{\br_i - \EE{\br_i}} \geq 2 \sqrt{\Var{\br_i}}} \leq \frac{1}{4}.
% 	\end{align*}
	
% 	By applying a Chernoff bound for sufficiently large $n \geq \Omega(\log \frac{1}{\delta})$, we can argue that there exist at least $\frac{n}{2}$ values of $i \in [\ell]$ such that $\br_i \geq \frac{1}{8 d_2}$ with probability at least $1 - \frac{\delta}{3}$.
% 	Therefore, it also follows that \[\sum_{j=1}^d \lambda_j^2 \bq_j^2 = \sum_{i=1}^{\ell} \br_i \geq \frac{n}{16 d_2}.\]


% \paragraph{Bound on term given good $\bX$.}
% We use the Berry-Esseen theorem \cite{berry41} to relate the maximization over $\norml[1]{\lambda}^{-1} y^\T \bX \bx_1'$ to a maximization over standard Gaussians.
% Consider some fixed good $\bX$ (and hence, fixed $\bq_j$ for all $j \in [d]$). Then, for some absolute constant $\ccc$ and for univariate standard Gaussian $\bg$,
% \[\sup_{t \in \R} \abs{\pr{\frac{\norm[1]{\lambda}^{-1} y^\T \bX \bx_1'}{\sqrt{\sum_{j=1}^d \bq_j^2\lambda_j^2 \EE{ \bz_{i,j}^{\prime2}}}} \leq t} - \pr{\bg \leq t}} 
% \leq \frac{\ccc}{\sqrt{\sum_{j=1}^d \bq_j^2\lambda_j^2 \EE{ \bz_{i,j}^{\prime2}}}} \cdot \max_{j \in [d] }\frac{\abs{\bq_{j}^3}\lambda_j^3\EE{\abs{\bz_{i,j}^{\prime3}} }}{\bq_{j}^2\lambda_j^2\EE{\bz_{i,j}^{\prime2} }}.\]

% Because each $\bz_{i,j}$ is subgaussian, $\EEl{\bz_{i,j}^3} \leq \rho = O(1)$ for some $\rho$. 
% We simplify the expression by plugging in the second and third moments of $\bz_{i,j}'$ and rescaling $t$:
% \[ \sup_{t \in \R}\abs{\pr{\frac{1}{\norm[1]{\lambda}} y^\T \bX \bx_1' \leq t} - \pr{\bg \leq \frac{t}{\sqrt{\sum_{j=1}^d \lambda_j^2 \bq_j^2}}}} \leq \frac{\ccc \rho}{\sqrt{\sum_{j=1}^d \lambda_j^2\bq_j^2  }} \cdot \max_{j \in [d] } \abs{\bq_j\lambda_j}.\]

% Because we assume that $\bX$ is good, we plug in our upper-bound on $\max_j \lambda_j \bq_j$ and lower-bound on $\sum_{j=1}^d \lambda_j^2 \bq_j^2$.
% \begin{align*}
% 	\pr{\frac{1}{\norm[1]{\lambda}} y^\T \bX \bx_1' \leq t}
% 	&\leq \pr{\bg \leq \frac{t}{\sqrt{\sum_{j=1}^d \lambda_j^2 \bq_j^2}}} + \frac{\ccc \rho}{\sqrt{\sum_{j=1}^d \lambda_j^2 \bq_j^2 }} \cdot \max_{j \in [d] } \abs{\lambda_j \bq_j} \\
% 	&\leq \pr{\bg \leq \frac{t\sqrt{16d_2}}{\sqrt{n}}} + \frac{ \ccc \rho \sqrt{16d_2}}{\sqrt{n}} \cdot \cp \sqrt{\frac{\log n}{d_2} } \\
% 	&\leq \pr{\bg \leq \frac{t\sqrt{d_2}}{\sqrt{n}}} + 4 \ccc \cp \rho \sqrt{\frac{ \log n}{n}}
% \end{align*}
	
% We now bound the first term by invoking a standard bound on a Gaussian CDF with the assumption that $\cb \leq \frac{1}{32}$.
% The remainder of the inequalities follow by enforcing that $\ca$ and $\cb$ be sufficiently large and small respectively.
% \begin{align*}
% 	\pr{\bg \leq \frac{t\sqrt{16d_2}}{\sqrt{n}}}
% 	&\leq \pr{\bg \leq \sqrt{\frac{1}{2}\log m}}
% 	\leq 1 - \paren{\frac{1}{\sqrt{\log (m) / 2}} - \frac{1}{(\log(m) / 2)^{3/2}}} \exp\paren{-\frac{\log m}{4}} \\
% 	&\leq 1 - \frac{1}{m^{1/3}}
% 	\leq 1 - \frac{1}{\sqrt{m}} -  4 \ccc \cp  \rho \sqrt{\frac{ \log n}{n}}.
% \end{align*}


% 	Therefore, 
% 	\[\pr{\frac{1}{\norm[1]{\lambda}} y^\T \bX \bx_1' \leq t \mid \bX, \bxig} \leq 1 - \frac{1}{\sqrt{m}} \leq \exp\paren{-\frac{1}{\sqrt{m}}} \leq \paren{\frac{\delta}{3}}^{1/m},\]
% 	which above holds when $m \geq \parenl{\log \frac{\delta}{3}}^2$ and is ensured by a sufficiently large choice of $\cc$.
% \end{proof}





\begin{lemma}\label{lemma:e3}
  Let $(\bX,\bZ,y) \in \R^{n \times d} \times \R^{n \times d} \times \R^n$
  and
  $(\bX',\bZ',y') \in \R^{m \times d} \times \R^{m \times d} \times \R^m$
  be $\lambda$-anisotropic subgaussian samples that are independent of each other.
  Pick any $t>0$ and $\delta \in (0, \half)$. 
    For universal constants $\ca$, $\cb$, $\cc$, and $\cd$, if 
    \[
    n \geq \ca \paren{\log \frac{1}{\delta}}^2,
    \quad
     \exp\paren{\frac{t^2 d_2}{\cb n}} \leq m \leq n,
    \quad
    d_2 \geq \cc n \log \log \frac{1}{\delta},
    \quad \text{and} \quad
    d_{\infty}^2 \geq\cd d_{2} n,\]
    then with probability $1 - \delta$
    \[\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}}  y^\T \bX \bx_i' \geq t.\]
\end{lemma}


\begin{proof}
\newcommand{\bxig}{\text{$\bX$ is good}}
\newcommand{\bxing}{\text{$\bX$ is not good}}


Let $\bq_{j} := \norml[1]{\lambda}^{-1} y^\T \bZ_{\cdot, j}$ for $j \in [d]$, where $\bZ_{\cdot, j} = (\bz_{1,j}, \dots, \bz_{n,j}) \in \R^n$.
Note that 
\[\frac{1}{\norm[1]{\lambda}}  y^\T \bX \bx_i' = \sum_{j=1}^d  \bq_{j} \lambda_j  \bz_{i,j}'\] and all $\bq_{j}$ and $\bz_{i,j}'$ are independent and that $\bq_j$ is subgaussian with variance proxy $\fracl{n}{\norml[1]{\lambda}^2}$.
The proof of the claim is powered by the Berry-Esseen theorem and comes in two parts:
\begin{itemize}
    \item We first show that $\bX$ is well-behaved with high probability; we say that $\bX$ is \emph{good} if the following hold:
    \begin{equation}\label{eq:good-norm}
         \sum_{j=1}^d \lambda_j^2 \bq_j^2 \geq \frac{n}{2 d_2},
    \end{equation}
    \begin{equation}\label{eq:good-max}
         \max_j \abs{\lambda_j \bq_j} \leq \frac{n^{1/4}}{\sqrt{d_2}}.
    \end{equation}
    We prove that $\prl{\bxig} \geq 1 - \frac{2\delta}{3}$.

    \item 
    Then, we use the Berry-Esseen Theorem to show that, for each $i \in [m]$,
    \[\pr{\frac{1}{\norm[1]{\lambda}} y^{\T} \bX \bx_i' \leq t \mid \bxig } \leq \paren{\frac{\delta}{3}}^{1/m} . \] %for all $i \in [m]$ if $\bX$ is good. 
\end{itemize}
Because $\norm[1]{\lambda}^{-1} y_i' y^\T \bX \bx_i'$ for $i \in [m]$ are conditionally independent given $\bX$, we obtain the desired statement:
\begin{align*}
    \pr{\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}} y_i' y^\T \bX \bx_i' \leq t}
    &\leq \pr{\bxing} + \pr{\max_{i \in [m]} \frac{1}{\norm[1]{\lambda}} y_i' y^\T \bX \bx_i' \leq t \mid \bxig} \\
    & \leq \frac{2\delta}{3} + \prod_{i=1}^m \pr{ \frac{1}{\norm[1]{\lambda}} y_i' y^\T \bX \bx_i' \leq t \mid \bxig} \leq \delta .
\end{align*}

\paragraph{$\bX$ satisfies \eqref{eq:good-norm} with high probability.}
The claim follows from the Hanson-Wright inequality \cite{vershynin14}, the lower-bound on $n$ with respect to $\delta$, the assumption $d_\infty^2 \geq c_4 d_2 n$, and the fact $\norm[4]{\lambda}^4 \leq \norm[2]{\lambda}^2 \norm[\infty]{\lambda}^2$.
\begin{align*}
    \pr{\sum_{j=1}^d \lambda_j^2 \bq_j^2 \leq \frac{n}{2d_2}}
    &\leq \pr{\abs{\sum_{j=1}^d \lambda_j^2 \bq_j^2 - \EE{\sum_{j=1}^d \lambda_j^2 \bq_j^2}} \leq \frac{n}{2d_2}} \\
    &\leq 2 \exp\paren{-c'' \min\paren{\frac{n^2}{4d_2^2} \cdot \frac{\norm[1]{\lambda}^4}{n^2} \cdot \frac{1}{\norm[4]{\lambda}^4}, \ \frac{n}{2d_2} \cdot \frac{\norm[1]{\lambda}^2}{n} \cdot \frac{1}{\norm[\infty]{\lambda}^2}}} \\
    &\leq 2\exp\paren{- \frac{c'' d_\infty^2}{4d_2}} 
    \leq 2\exp\paren{- \frac{c'' c_4 n}{4}}
    \leq \frac{\delta}{3},
\end{align*}
for sufficiently large absolute constant $c_4$.

\paragraph{$\bX$ satisfies \eqref{eq:good-max} with high probability.}

We introduce a different sequence of random variables $\br_1, \dots, \br_{n}$ to eliminate any dependence on $d$.
Set $0 = k_0 < k_1 < \dots < k_{n} = d$ such that for all $i \in [n]$, 
\[\sum_{j=k_{i-1}+1}^{k_{i}} \lambda_j^2 \leq \frac{2\norm[2]{\lambda}^2}{n}.\]
Such a partition is possible because we can require that $\norml[\infty]{\lambda}^2 \leq \fracl{\norml[2]{\lambda}^2}{n}$ by assuming $\cd$ is large enough.
Let \[\br_i = \sum_{j=k_{i-1}+1}^{k_{i}} \lambda_j^2 \bq_j^2.\]  
Note that all $\br_i$ are independent and that \[\sum_{j=1}^d \lambda_j^2 \bq_j^2 = \sum_{i=1}^{n} \br_i.\] 
Because $\EEl{\bq_j} = 0$ and $\EEl{\bq_j^2} = \fracl{n}{\norml[1]{\lambda}^2}$, we can bound $\EEl{\br_i}$:
\[	\EE{\br_i} 
		\leq \frac{2n\norm[2]{\lambda}^2}{ n \norm[1]{\lambda}^2}
		\leq \frac{2}{d_2}. \]
		
We upper-bound $\max_j \absl{\lambda_j \bq_j}$ by noting that $\max_j \absl{\lambda_j \bq_j} \leq \max_i \sqrt{\br_i}$.
By the Hanson-Wright inequality, the subgaussianity of $\bq_i$, and the lower-bound on $n$ with respect to $\delta$,
\begin{align*}
    \pr{\br_i \geq \frac{ \sqrt{n}}{d_2}}
    &\leq \pr{\br_i \geq \EE{\br_i} + \frac{\sqrt{n}}{2 d_2}} \\
    % &\leq 2\exp\paren{-c' \min\paren{\frac{ n \norm[1]{\lambda}^4}{4 d_2^2 n^2\sum_{j=k_{i-1}+1}^{k_i} \lambda_j^4}, \frac{ \sqrt{n} \norm[1]{\lambda}^2}{2 d_2 n \max_{k_{i-1} < j \leq k_i} \lambda_j^2}}} \\
    &\leq 2\exp\paren{-c' \min\paren{\frac{ n}{4d_2^2}\cdot \frac{ \norm[1]{\lambda}^4}{ n^2} \cdot \frac{1}{\sum_{j=k_{i-1}+1}^{k_i} \lambda_j^4}, \frac{ \sqrt{n}}{2 d_2}\frac{ \norm[1]{\lambda}^2}{n} \frac{1}{\max_{k_{i-1} < j \leq k_i} \lambda_j^2}}} \\
    &\leq 2\exp\paren{-c' \min \paren{ \frac{n}{4}, \frac{\sqrt{n}}{2}}} 
    \leq \frac{\delta}{3n}
\end{align*}
for some absolute constants $c'$ and for a sufficiently large setting of $c_1$.
Thus, \eqref{eq:good-max} is satisfied with probability $1 - \frac{\delta}{3}$ by a union bound.

\paragraph{Bound on term given good $\bX$.}
We use the Berry-Esseen theorem \cite{berry41} to relate the maximization over $\norml[1]{\lambda}^{-1} y^\T \bX \bx_1'$ to a maximization over standard Gaussians.
Consider some fixed good $\bX$ (and hence, fixed $\bq_j$ for all $j \in [d]$). Then, for some absolute constant $\ccc$ and for univariate standard Gaussian $\bg$,
\[\sup_{t \in \R} \abs{\pr{\frac{\norm[1]{\lambda}^{-1} y^\T \bX \bx_1'}{\sqrt{\sum_{j=1}^d \bq_j^2\lambda_j^2 \EE{ \bz_{i,j}^{\prime2}}}} \leq t} - \pr{\bg \leq t}} 
\leq \frac{\ccc}{\sqrt{\sum_{j=1}^d \bq_j^2\lambda_j^2 \EE{ \bz_{i,j}^{\prime2}}}} \cdot \max_{j \in [d] }\frac{\abs{\bq_{j}^3}\lambda_j^3\EE{\abs{\bz_{i,j}^{\prime3}} }}{\bq_{j}^2\lambda_j^2\EE{\bz_{i,j}^{\prime2} }}.\]

Because each $\bz_{i,j}$ is subgaussian, $\EEl{\bz_{i,j}^3} \leq \rho = O(1)$ for some $\rho$. 
We simplify the expression by plugging in the second and third moments of $\bz_{i,j}'$ and rescaling $t$:
\[ \sup_{t \in \R}\abs{\pr{\frac{1}{\norm[1]{\lambda}} y^\T \bX \bx_1' \leq t} - \pr{\bg \leq \frac{t}{\sqrt{\sum_{j=1}^d \lambda_j^2 \bq_j^2}}}} \leq \frac{\ccc \rho}{\sqrt{\sum_{j=1}^d \lambda_j^2\bq_j^2  }} \cdot \max_{j \in [d] } \abs{\bq_j\lambda_j}.\]

Because we assume that $\bX$ is good, we plug in our upper-bound on $\max_j \absl{\lambda_j \bq_j}$ and lower-bound on $\sum_{j=1}^d \lambda_j^2 \bq_j^2$.
\begin{align*}
	\pr{\frac{1}{\norm[1]{\lambda}} y^\T \bX \bx_1' \leq t}
	&\leq \pr{\bg \leq \frac{t}{\sqrt{\sum_{j=1}^d \lambda_j^2 \bq_j^2}}} + \frac{\ccc \rho}{\sqrt{\sum_{j=1}^d \lambda_j^2 \bq_j^2 }} \cdot \max_{j \in [d] } \abs{\lambda_j \bq_j} \\
	&\leq \pr{\bg \leq \frac{t\sqrt{2d_2}}{\sqrt{n}}} + \frac{ \ccc \rho \sqrt{2d_2}}{\sqrt{n}} \cdot   \frac{n^{1/4}}{\sqrt{d_2}} \\
	&\leq \pr{\bg \leq \frac{t\sqrt{2d_2}}{\sqrt{n}}} + \frac{\sqrt{2}c \rho}{n^{1/4}}
\end{align*}
	
We now bound the first term by invoking the
Mills ratio bound for the Gaussian distribution function (Fact~\ref{fact:mills})
%a standard bound on a Gaussian distribution function
with the assumption that $\cb \leq \frac{1}{8}$.
The remainder of the inequalities follow by enforcing that $\ca$ and $\cb$ be sufficiently large and small respectively:
\begin{align*}
	\pr{\bg \leq \frac{t\sqrt{2d_2}}{\sqrt{n}}}
	&\leq \pr{\bg \leq \sqrt{\frac{1}{4}\log m}}\\
	& 
	\leq 1 - \frac1{\sqrt{2\pi}} \paren{\frac{1}{\sqrt{\log (m) / 4}} - \frac{1}{(\log(m) / 4)^{3/2}}} \exp\paren{-\frac{\log m}{8}} \\
	&\leq 1 - \frac{1}{m^{1/6}}
	\leq 1 - \frac{1}{\sqrt{m}} -  \frac{\sqrt{2}c \rho}{n^{1/4}}.
\end{align*}


	Therefore, 
	\[\pr{\frac{1}{\norm[1]{\lambda}} y^\T \bX \bx_1' \leq t \mid \bxig} \leq 1 - \frac{1}{\sqrt{m}} \leq \exp\paren{-\frac{1}{\sqrt{m}}} \leq \paren{\frac{\delta}{3}}^{1/m},\]
	which above holds when $m \geq \parenl{\log \frac{3}{\delta}}^2$ and is ensured by a sufficiently large choice of $\cc$.
\end{proof}

The following well-known fact is the Mills ratio bound.
\begin{fact} \label{fact:mills}
Let $\Phi$ denote the standard Gaussian distribution function. Then for any $t \geq 0$,
\[ \left( \frac1t - \frac1{t^3} \right)  \cdot \frac1{\sqrt{2\pi}} e^{-t^2/2} \leq 1 - \Phi(t) \leq \frac1t \cdot \frac1{\sqrt{2\pi}} e^{-t^2/2} . \]
\end{fact}

\subsection{Modification of Theorem~\ref{thm:anisotropic} to support dependent labels}\label{assec:dependent-labels}

While an apparent weakness of Theorem~\ref{thm:anisotropic} is the fixed labels $y$, this can be surmounted.
Here, we outline how the proof can be easily modified to include labels $\by_i = \sign{v^\T \bx_i}$ for some unit vector $v$ for the isotropic Gaussian case; we believe this can be further generalized, but we present this version for the sake of simplicity.

\begin{theorem}[Lower-bound on SVP threshold with dependent labels]\label{thm:dependent-labels}
    Fix any $v \in \R^d$ with $\norml{v} = 1$, and consider an isotropic Gaussian sample $(\bX,\by)$ where each $\by_i = v^\T \bx_i$ and any $\delta \in (0, \half)$
	For absolute constants $\Ca, \Cb, \Cc, \Cd$, assume that $d$ and $n$ satisfy
\begin{equation}
	  n \geq \Ca \paren{\log \frac{1}{\delta}}^2, \quad d \leq \Cb n \log n, \quad \text{and} \quad
	  d \geq \Cc n \log\frac{1}{\delta}, 
	 \end{equation}
	Then\footnote{The fourth constraint is omitted because $d_2 = d_\infty = d$ in the isotropic case.}, SVP occurs for $\ell_2$-SVM with probability at most $\delta$.
\end{theorem}

The proof of the theorem relies on the same decomposition as Theorem~\ref{thm:anisotropic}.
The first step (Lemma~\ref{lemma:e1}) proceeds identically, because the proof of the lemma uses no other properties of the $\by$ besides the fact that it belongs to $\flip^n$.
The following inequality allows the remainder of the proof to proceed identically by fixing $y = \vec{1}$. 
For all $t \in \R$ and $i \in [n]$,
\[\pr{\by_i \by_{\setminus i}^\T \bX_{\setminus i} \bx_i \geq t} \geq \pr{\vec{1}^\T \bX_{\setminus i} \bx_i \geq t}.\]
%
We can prove this fact for the simple Gaussian setting by taking advantage of the fact that orthogonal components of a spherical Gaussian are independent.
For all $i$, we write $\bx_i = (v^\T \bx_i) v + \bx_i'$ where $v^\T \bx_i' = 0$.
Then
\begin{align*}
    \by_i \by_{\setminus i}^\T \bX_{\setminus i} \bx_i
    &= \sum_{j\neq i} (\by_j \bx_j)^\T(\by_i \bx_i)
    = \sum_{j\neq i} \sign{v^\T \bx_j v^\T \bx_i} [v^\T \bx_j v^\T \bx_i \norml[2]{v}^2 + \bx_j^{\prime \T} \bx_i'] \\
    &= \sum_{j\neq i}[\absl{v^\T \bx_j v^\T \bx_i} + \sign{v^\T \bx_j v^\T \bx_i}\bx_j^{\prime \T} \bx_i']
    \geq \sum_{j\neq i}[{v^\T \bx_j v^\T \bx_i} + \sign{v^\T \bx_j v^\T \bx_i}\bx_j^{\prime \T} \bx_i'].
\end{align*}

By independence and symmetry, each term in the last sum is distributed identically to ${v^\T \bx_j v^\T \bx_i} + \bx_j^{\prime \T} \bx_i' = \bx_j^\T \bx_i$. This gives the claim.


==> asymptotic_old.tex <==
\section{Exact asymptotic rate for Gaussian case}\label{sec:asymptotic}

In Section~\ref{sec:nonasymp}, we observe that for training data with independent isotropic subgaussian components, support vector proliferation occurs with high probability if $d = \Omega(n \log n)$ and does not occur with high probability if $d = O(n \log n)$.
Here, we refine that analysis for the spherical Gaussian case to find an exact threshold. 
That is, if $d = \tau n \ln n$, as $n$ becomes large, support vector proliferation will occur when $\tau > 2$ and will not occur when $\tau < 2$.
The two following theorems jointly show this sharp threshold.

\todo{revise these theorems to say something about the width of confidence intervals}

\navid{can we combine both of the theorems into one?}

\begin{theorem}[Exact lower-bound on support vector proliferation]\label{thm:asymptotic-lb}
% 	Consider training samples $\bX := [\bx_1 |  \dots | \bx_n]^T$, where each $\bx_i \sim \mathcal{N}(0, I_d)$ is independently drawn.
	Let $\bX$ and $y$ be a Gaussian isotropic sample.
	For all $\eps, \delta \in (0, 1)$, there exists a sufficiently large $n$ such that if $d = (2 - \eps) n \ln n$ \clayton{something stupid about rounding and floors}, then with probability $1 - \delta$, at least one training sample is not a support vector for the solution to the $\ell_2$ SVM problem.
\end{theorem}

\begin{theorem}[Exact upper-bound on support vector proliferation]\label{thm:asymptotic-up}
% 	Consider training samples $\bX := [\bx_1 |  \dots | \bx_n]^T$, where each $\bx_i \sim \mathcal{N}(0, I_d)$ is independently drawn.
    Let $\bX$ and $y$ be a Gaussian isotropic sample.
	For all $\eps, \delta \in (0, 1)$, there exists a sufficiently large $n$ such that if $d = (2 + \eps) n \ln n$, then with probability $1 - \delta$, every training sample is a support vector for the solution to the $\ell_2$ SVM problem.
\end{theorem}


We relegate both proofs to Appendix~\ref{app:asymp-proofs}.
The proof of Theorem~\ref{thm:asymptotic-up} mirrors that of Theorem~\ref{thm:anisotropic}, but deviates in the final step.
The Central Limit Theorem used in Lemma~\ref{lemma:e3} does not give sufficiently tight anti-concentration bounds on approximately-Gaussian random variables to ensure a constant threshold; instead, the proof of Theorem~\ref{thm:asymptotic-lb} takes advantage of the Gaussianity assumption to make use of known concentration properties about the maximum of independent Gaussians.
The proof of Theorem~\ref{thm:asymptotic-up} relies only on Gaussian concentration bounds.

==> asymptotic_proofs_old.tex <==
\section{Proofs for Section~\ref{sec:asymptotic}}\label{app:asymp-proofs}

\begin{proof}[Proof of Theorem~\ref{thm:asymptotic-lb}]
This proof is very similar to that of Theorem~\ref{thm:anisotropic}. 
Here, we let $m := \frac{n}{\log n} \leq \frac{n}{2}$.
Again, we break the argument down to three steps, which together prove the claim with Lemma~\ref{lemma:hmx-equivalence}:

\begin{enumerate}
    \item 
    By Lemma~\ref{lemma:e1} with $d_2 = d_{\infty} = d$ and $\delta := \frac{\delta}{3m}$, $\absl{y_i y_{\setminus i}^\T (\bK_{\setminus i}^{-1} - \frac{1}{d} I_{n-1}) \bX_{\setminus i} \bx_i } \leq \frac{\eps}{32}$ for all $i \in [m]$ with probability $1 - \frac{\delta}{3}$ as long as
    \[d = \Omega\paren{\frac{\sqrt{n d}}{\eps} + \frac{n}{\eps} \log \frac{1}{\delta}},\]
    which holds for sufficiently large $n$.

    \item By Lemma~\ref{lemma:e2}, $\frac{1}{d} y_i y_{[m] \setminus i}^\T \bX_{[m] \setminus i} \bx_i  \geq -\frac{\eps}{32}$ for all $i \in [m]$ holds with probability $1 - \frac{\delta}{3}$ as long as:
    \[d = d_{\infty} = \Omega(\frac{m}{\epsilon} \log \frac{m}{\delta})= \Omega(\frac{n}{\epsilon} \log \frac{1}{\delta})\]
    % \[n = \Omega\paren{\frac{\log{\frac{1}{\delta}}}{\epsilon^2}}.\]
    
    \item It remains to show that there exists some $i \in [m]$ such that $\frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i \geq 1 + \frac{\eps}{16}$ with probability $1- \frac{\delta}{3}$.
\end{enumerate}

The remainder of this proof shows why the third point holds. 

Observe that conditioned on $\bX_{\setminus [m]}$, $\frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i  \overset{\text{d}}{=} \sigma^{(m)} \mathbf{g}_{i}$ where $\sigma^{(m)} = \frac{1}{d} \norm[2]{y_{\setminus [m]}^\T \bX_{ \setminus [m]}}$ and $\mathbf{g}_{i}$ is a standard Gaussian.
We lower-bound the variance term with high probability. Expanding the term gives
\[\frac{1}{d^2} \norm[2]{y_{\setminus [m]}^\T \bX_{ \setminus [m]}}^2
= \frac{1}{d^2} y_{\setminus [m]}^\T \bK_{ \setminus [m]} y_{\setminus [m]}^\T
\geq \frac{n - m}{d^2} \mu_{\min}(\bK_{\setminus [m]}).\]
By Lemma~\ref{lemma:gram-evals}, $\mu_{\min}(\bK_{\setminus [m]}) \geq d(1 - c \sqrt{\fracl{(n-m)}{d}}) \geq d(1 - c \sqrt{\fracl{n}{2d}})$ with probability $1 - \frac{\delta}{6}$.
Thus, 
\[\sigma^{(m)} \geq \sqrt{\frac{(n-m)(1 - c \sqrt{\frac{n}{2d}})}{d}} \geq \sqrt{\frac{\paren{1 - \frac{1}{2\ln n}}\paren{1 -  \frac{c}{\sqrt{ \ln n}}}}{(2 - \eps) \ln n}}.\]
Similarly one can upper bound $\sigma^{(m)}$ using $\mu_{\max}(K_{\setminus [m]})$ and deduce that:
\[ \sigma^{(m)}\sqrt{2 \log(m)} \overset{\text{Pr.}}{\longrightarrow} \sqrt{\frac{2}{2-\epsilon}}
\]

Now since maximum is a 1-Lipschitz function of its input then for random variable $\bu = \max_{i \in [m]}{\frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i} \overset{\text{d}}{=} \sigma^{(m)} \max_{i \le m}{\mathbf{g}_{i}} $ we have:
\navid{This is not asymptotically sharp since it predicts constant variance for max of Gaussian, but it does the job, right?}
\[
\mathbf{P}[| \bu - \mathbf{E}[\bu \mid \bX_{\setminus [m]}] | \ge t \sigma^{(m)}  \mid  \bX_{\setminus [m]} ] \le 2 e^{\frac{-t^{2}}{2}} = \frac{\delta}{6}
\]
where $t = \sqrt{2 \log(\frac{12}{\delta})}$. Furthermore, it is a well known fact for Gaussian random variables:
\[
\lim_{m \to \infty} \frac{\mathbf{E}[\max_{i \le m}{\mathbf{g}_{i}}]}{\sqrt{2 \log(m)}} =
1
\Longrightarrow
\mathbf{E}[\bu \mid \bX_{\setminus [m]}] \overset{\text{Pr.}}{\longrightarrow} \sqrt{\frac{2}{2-\epsilon}}
\]
where the implication is based on Slutsky's Theorem. Moreover, since $t\sigma^{(m)} \overset{\text{Pr.}}{\longrightarrow} 0$ we can ensure the following event holds with probability $1-\frac{\delta}{6}$ for sufficiently large $n$:
\[
\mathbf{E}[\bu \mid \bX_{\setminus [m]}] \ge \sqrt{\frac{2}{2- \epsilon}} - \frac{\epsilon}{8} 
\ge 1 + \frac{\epsilon}{8}
\quad , \quad 
t \sigma^{(m)} \le \frac{\epsilon}{16}
\]
Combining all the above, by taking the $i \in [m]$ that realizes the maximum, then with probability at least $1 - \frac{\delta}{3}$: 
\[
    \frac{1}{d} y_i y_{\setminus [m]}^\T \bX_{ \setminus [m]} \bx_i = \bu
    \geq \mathbf{E}[\bu \mid \bX_{\setminus [m]}] - t\sigma^{(m)}
    \geq 1 + \frac{\epsilon}{16}\qedhere
\]
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:asymptotic-up}]
Our goal is to show that for all $i \in [n]$, $y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1}  \bX_{\setminus i} \bx_i  < 1$.
To do so, we show that with probability at most $1 - \frac{\delta}{n}$, $y_1 y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  \bX_{\setminus 1} \bx_1  < 1$; the claim follows from a union bound.
Conditioned on $\bX_{\setminus 1}$, the quantity is a Gaussian of mean 0 and variance $\norml[2]{y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  \bX_{\setminus 1}}^2 = y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  y_{\setminus 1} \leq (n-1) \mu_{\max}(\bK_{\setminus 1}^{-1})$. 
By Lemma~\ref{lemma:gram-evals}, $\mu_{\max}(\bK_{\setminus 1}^{-1}) \leq \frac{1}{d} \paren{1 + c \sqrt{\frac{n}{d}}}$ with probability $1 - \frac{\delta}{2n}$. 
Therefore, the variance is at most 
\[\frac{n}{d} \paren{1 + c \sqrt{\frac{n}{d}}} \leq \frac{1}{(2 + \eps) \ln n} \paren{1 + c \sqrt{\frac{1}{\ln n}}}.\]
We can then upper-bound the probability that the term is no more than 1, conditioned on this variance bound for sufficiently large $n$:
\begin{align*}
    \pr{y_1 y_{\setminus 1}^\T \bK_{\setminus 1}^{-1}  \bX_{\setminus 1} \bx_1  \geq 1}
    &\leq \exp\paren{-\frac{(2 + \eps) \ln n}{2\paren{1 + c \sqrt{\frac{1}{\ln n}}}}} = n^{-\paren{\frac{1 + \fracl{\eps}{2}}{1 + c \sqrt{\frac{1}{\ln n}}}}} \leq \frac{\delta}{2n}.\qedhere
\end{align*}
\end{proof}

==> junk.tex <==
\subsection{Junk Yard}
\navid{we should put more emphasis on this sentence I think} Note that we disregard the instances when the observed success rates are degenerate, that is there is ambiguity in defining Z-scores. We resolve this issue by restricting our attention to a narrower range of $n,d$. More precisely, we restrict $\tau \coloneqq \fracl{d}{\paren{2n\log n}}$ to be in the range [0.4,1.6] which will induce a negligible \navid{how should I argue here?} bias into our analysis. Unfortunately, this issue cannot be avoided by increasing the simulation size since actual probabilities of the desired events might be either exponentially small or exponentially close to one for some $n,d$ in our simulation range (see Theorem~\ref{thm:hmx-ub},\ref{thm:anisotropic}). 

As described in Section~\ref{sec:experiments} we attempt to show universality by computing Z-scores which assesses whether the underlying probability for which observed success rates are generated from are equal or not. More precisely, for distributions $\distr_{1}, \distr_{2}$ let us abbreviate $\hat{\mathbf{p}}_{1} = \hat{\mathbf{p}}(n,d; \distr_{1},M) ,\hat{\mathbf{p}}_{2} = \hat{\mathbf{p}}(n,d; \distr_{2},M)$ to be the observed success rates.
Therefore we can compute Z-scores between distributions using the following formula:
\[ 
\bZ (n,d; M,\distr) = \frac{\hat{\mathbf{p}}_{2} - \hat{\mathbf{p}}_{1}}{ \sqrt{ \frac{\paren{\hat{\mathbf{p}}_{2} + \hat{\mathbf{p}}_{1}} \paren{2 - \paren{\hat{\mathbf{p}}_{2} + \hat{\mathbf{p}}_{1}} } }{8 M} } }.
\]
In our analysis we fix $\distr_{1}$ to be the Gaussian ensemble. Under the null hypothesis of indifference between distributions for each $n,d$ one expects Z-scores to follow a standard normal distribution for large values of $M$. However, It might be naive to expect such hypothesis to hold true since phenomena at hand is an asymptotic statement and decaying deviations from the asymptotic behaviour should be expected non-asymptotically. Therefore, inspired by \cite{donoho2009observed} we instead form the following null-hypothesis and provide evidence for its significance. \navid{not sure whether we should say we don't reject this hypothesis or we show it's significance.}

\textbf{Universality Hypothesis:} For each $n,d$, Z-scores (defined above) follows a $\mathcal{N}\paren{\mu\paren{n, d; \distr},1}$ distribution where the mean decays to zero as $n, d$ grows large.

\begin{figure}[h]
    \begin{minipage}{\textwidth}
        \begin{minipage}{0.48\linewidth}
                \centering
                \includegraphics[width=\textwidth]{unnamed-chunk-10-1.pdf}
        \end{minipage}
        \hfill
        \begin{minipage}{0.48\linewidth}
                \centering
                \includegraphics[width=\textwidth]{unnamed-chunk-10-2.pdf}
        \end{minipage}
        \label{table:Z-scores}
        \caption{Comparing bulk distribution of Z-scores for suite of non-Gaussian distributions with Gaussian Ensemble. Note that white region corresponds to $\tau \notin [0.6,1.4]$ were Z-scores are ill-defined. \navid{Last sentence feel a bit ambiguous.}
        \clayton{These plots should be bigger. Maybe each needs their own figure?
        I'm also not very sure what the desired take-away here should be.}
        }
    \end{minipage}
\end{figure}

==> notes.tex <==
\todo{
\section*{Todo/things to resolve:}
\begin{itemize}
    \item For all-zero vectors, $\vec{0}, \mathbf{0}, 0$? \clayton{vote for $\vec{0}$}
    \item Standardize matrix row notation. ($\bA_{i,:}, \bA_{\cdot, j},$ etc.) \clayton{$\bA_i$ is the $i$th row, $\bA_{\cdot, j}$ is the $j$th column}
    % \item Standardize how we do citations: e.g. is it okay for say something like ``\cite{bhx20} proves \dots''? Also, if we do so, should we treat ``\cite{bhx}'' as singular or plural?
    \item What should we do about labels $y$ that depend on $\bX$? We could add a theorem for the case where $y$ corresponds to a true linear separator, but that might add unnecessary complexity 
    \clayton{mention briefly in intro}
    \item Numbered equations vs named equations? \clayton{New rule: important things that are referred to in different sections are named; less important equations are named}
    \item When referring to an equation, should we say ``Equation~\eqref{eq:3},'' ``equation~\eqref{eq:3},'' or ``\eqref{eq:3}?''
    \item When we prove things in the appendix, should we repeat the theorem there? \clayton{Hold off for now}
    \item Unify what we're calling samples (isotropic gaussian vs gaussian ensemble) \clayton{Sample = $(\bX, y)$, ensemble = $\bA$}
    \item Standardize $\ell_p$ SVMs and $\ell_q$ SVMs
    \item Be more consistent about $\bA$ and $\bX$. \clayton{Keep $\bA$ and $\bX$ separate, but take transpose of $\bA$ so that both $n \times d$.}
    \item Standardize $\R_+^d$, $\R_{\geq 0}^d$, $\text{int}(\R_+^d)$. \clayton{1 and 3, define int in intro}
    \item When do we use present vs past tense for discussing papers?
    \item $\log$ vs $\ln$ consistency \clayton{$\log$ everywhere, mention in notation that it's natural log}
\end{itemize}

}

==> prelim_old.tex <==
\section{Preliminaries}\label{sec:prelim}

\subsection{Notation}
For $\lambda\in \R_{+}^d$, define $d_2 := \fracl{\norml[1]{\lambda}^2}{\norml[2]{\lambda}^2}$ and $d_{\infty} := \fracl{\norml[1]{\lambda}}{\norml[\infty]{\lambda}}$, and note that $d \geq d_2 \geq d_{\infty}$.
$d_2$ and $d_{\infty}$ can differ substantially from one another:
If $\lambda = (1,\sqrt{d}, \dots, \sqrt{d})$, then $d_2 = \Theta(d)$ and $d_{\infty} = \Theta(\sqrt{d})$.

\todo{Notation for $\bX_{\setminus i}, \bX_{[m]}, \bx_{[m] \setminus i}, \bX_{\setminus [m]}$, etc}

Let $\mu_{\max}(A)$ and $\mu_{\min}(A)$ represent the largest and smallest eigenvalues of matrix $A$ respectively.

Let $[n] := \set{1, \dots,  n}$.

\subsection{Learning model}
\clayton{some of this will surely be moved to the introduction}

We consider the hard-margin support vector machine (SVM) optimization problem and ask under what conditions one may expect all the slackness conditions to be satisfied. 
We consider training samples $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \flip$ in a high-dimensional regime where $d \gg n$ and let $\bX := [\bx_1 | \dots | \bx_n]^\T \in \R^{n \times d}$ to represent the inputs collected into a matrix \todo{there's a name for this...} and $\bK = \bX \bX^\T \in \R^{n \times n}$ be the corresponding Gram matrix.
In full generality, the separating hyperplane corresponding to the $\ell_p$-norm SVM problem for some $p \geq 1$ is the solution to the following optimization problem:
\begin{equation}
    \tag{SVM Primal}
    \label{eq:svm-primal-lp}
    \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i \innerprod{w}{\bx_i} \geq 1, \ \forall i \in [n].
\end{equation}

It is worth mentioning that we are not concerned with feasibility issues since $w$ resides in a high dimensional world \navid{Somewhere probably we should mention about Cover's result}. Moreover, we call a training sample $(\bx_i, y_i)$ to be a \emph{support vector} if it lies exactly on the margin defined by separator $w$, or equivalently if $y_i \innerprod{w}{\bx_i} = 1$.
\todo{say something about alternate representation of $w$ as linear combination of support vectors}
We study the phenomenon of \emph{support vector proliferation}, which occurs when $(\bx_i, y_i)$ is a support vector for all $i \in [n]$.
This can be equivalently understood at the event that the solution to the \eqref{eq:svm-primal-lp} coincides exactly with that of
\begin{equation}
    \tag{Interpolation Primal}
    \label{eq:svm-restricted-primal-lp}
    \min_{w \in \R^d} \norm[p]{w} \quad \text{such that} \quad y_i \innerprod{w}{\bx_i} = 1, \ \forall i \in [n].
\end{equation}

% \begin{center}
% \begin{minipage}{0.25\textwidth}
%     \begin{align*}
%     \min & \quad \|w\|_{p} \\
%     \text{s.t.} & \quad Y_{i} \langle w , X_{i} \rangle \ge 1 
%     \end{align*}
% \end{minipage}
% $\overset{?}{=}$
% \begin{minipage}{0.25\textwidth}
%     \begin{align*}
%     \min & \quad \|w\|_{p} \\
%     \text{s.t.} & \quad Y_{i} \langle w , X_{i} \rangle = 1 
%     \end{align*}
% \end{minipage}
% \end{center}

Moreover, we can translate this relation in the dual space by adding Lagrange multipliers $\alpha \in \mathbb{R}^{n}$, and obtain the dual of \eqref{eq:svm-restricted-primal-lp}:
\[
\max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} + \min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \innerprod{ w}{ \sum_{i=1}^{n}{\alpha_{i}y_{i}\bx_{i} }}}.
\]
Now using Holder's inequality if we take $q$ to be the dual of $p$ (i.e. $\frac{1}{p} + \frac{1}{q} = 1$) then $\langle w, u \rangle \le \|w\|_{p} \|u\|_{q}$ where equality holds when $|u_{i}|^{q} = |w_{i}|^{p}$ thus we have:

\[\min_{w \in \mathbb{R}^{d}}{  \|w\|_{p} - \langle w, u \rangle} = 
\begin{cases}
0 & \|u\|_{q} \le 1 \\
-\infty & \text{otherwise.}\\
\end{cases}
\]
Let us further denote $\bA \in \mathbb{R}^{d \times n}$ where the $i$'th column is $y_{i}\bx_{i}$ then we conclude that the dual of optimization \eqref{eq:svm-primal-lp} is:
\begin{equation}
    \tag{Interpolation Dual}
    \label{eq:svm-restricted-dual-lp}
    \max_{\alpha \in \mathbb{R}^{n}} \sum_{i=1}^{n}{\alpha_{i}} \quad
    \text{such that}  \quad \|\bA\alpha \|_{q} \le 1 .
\end{equation}

Similarly one can find the dual of \eqref{eq:svm-primal-lp} to be analogous to \eqref{eq:svm-restricted-dual-lp} where the difference is excess restriction on $\alpha$ having non-negative coordinates, i.e. $\alpha \in \mathbb{R}_{+}^{n}$. To reiterate, we are interested in the event that this excessive constraints are in a sense redundant. In other words, support vector proliferation occurs if and only if $\alpha^{*}_i > 0$ for all $i \in [n]$ where $\alpha^{*}$ is an optimal solution for \eqref{eq:svm-restricted-dual-lp} problem \todo{ref to appropriate lemma here}.  It is fairly straightforward to see that optimal solutions of \eqref{eq:svm-restricted-dual-lp} are equivalent to the following problem:

\begin{equation}
    \label{eq:projection-lq}
    \min_{\alpha \in \mathbb{R}^{n} \setminus \{\mathbf{0}\}}{ \norm[q]{\bA \frac{\alpha}{\sum_{i=1}^{n}{\alpha_{i}}}} }
\end{equation}
\daniel{do you need to require $\sum \alpha_i \neq 0$?}

This formulation is intuitive at the very least for the $\ell_{2}$-case since it demonstrates a well known fact that separating hyperplane is obtained as  a linear combination of inputs. In order to provide a geometric interpretation of \eqref{eq:projection-lq} let us denote $T, T^{+}$ to respectively be the hyperplane passing through and convex hulls of columns of $A$. We may then interpret the optimization problem above as a projection of the origin onto the set $T = \{\sum_{i=1}^{n}{a_{i}A_{i}} : \sum_{i=1}^{n}{a_{i}} = 1\} \subset \mathbb{R}^{d}$ using $\ell_{q}$-norm. 

\textbf{Main Question:} Now that we have all the prerequisites we may form our main question in two alternative point of views roughly as the following:
\begin{itemize}
    \item Under which settings of input samples the optimal solution to \eqref{eq:svm-restricted-dual-lp} lies within the interior of $\mathbb{R}_{+}^{d}$?
    
    \item under which setting of input samples the projection of the origin onto $T$ denoted by $\Pi_{T}(0)$ lies inside $T^{+}$?
\end{itemize}
 


This dual framework gives an alternative geometric structure to consider for this problem, which is explored in detail for the $\ell_1$ case in Section~\ref{sec:l1}. Essentially, we use the fact that $\ell_{1}$-case boils down to an LP problem where the corner points of the constraint set determines the behaviour of our optimization problem.



%\begin{equation}
%    \label{eq:svm-dual-l1}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad -\vec{1} \leq \bA\alpha \leq \vec{1} .
%\end{equation}
%
%\begin{equation}
%    \label{eq:svm-dual-l2}
%    \max_{\alpha \in \mathbb{R}_{+}^{n}}  \sum_{i=1}^{n}{\alpha_{i}} %\quad
%    \text{such that}  \quad 1 \leq \alpha^\T \diag(y) \bK \diag(y) %\alpha \leq 1.
%\end{equation}


\subsection{Data model}
We use the same data model of \cite{hmx20}, where every labeled sample $(\bx_i, y_i)$ has $\bx_i$ drawn from an anisotropic subgaussian distribution with independent components and arbitrary fixed labels $y_i$.
\todo{Say something about why linear separability won't be a problem for us}

\begin{definition}
    For some $\lambda\in \R_{\geq 0}^d$, let a \emph{$\lambda$-anisotropic sample} be $(\bx_1, y_1), \dots, (\bx_n, y_n) \in \R^d \times \flip$ drawn as follows.
    Let $\bX := [\bx_1 |  \dots | \bx_n]^\T = \bZ \  \diag(\lambda)^{1/2} \in \R^{n \times d}$, where each $\bz_i$ has independent subgaussian components  with $\EEl{\bz_{i,j}} = 0$ and $\EEl{\bz_{i,j}^2} = 1$.
	Additionally, assume that $\bz_{i,j}$ is subgaussian for all $i \in [n], j \in [d]$.
	Let $y = (y_1, \dots, y_n)$ be arbitrary labels that do not depend on $\bX$.
\end{definition}

We also consider a simpler data model of isotropic Gaussian samples, which allows us to more tightly characterize the support vector proliferation threshold in Theorem~\ref{thm:asymptotic-lb} and \ref{thm:asymptotic-up}.

\begin{definition}
    A \emph{Gaussian isotropic sample} consists of independent $(\bx_1, y_1), \dots, (\bx_n, y_n) \sim \mathcal{N}(0, I_d)$ drawn as follows, which can be collected as $\bX := [\bx_1 |  \dots | \bx_n]^\T \in \R^{n \times d}$.
    Let $y = (y_1, \dots, y_n)$ be arbitrary labels that do not depend on $\bX$.
\end{definition}

\todo{Say something about random labels:

- we don't need to worry about linear separability for arbitrary labels because of Cover result

- we can also handle labels that depend on a ground truth linear classifier. banish this to the appendix or explain why it's easy? 
}

\subsection{Previous results}

We build on the upper- and lower-bounds presented in \cite{hmx20} for the support vector proliferation threshold. 
We give versions of their results that are directly comparable to our results in Sections~\ref{sec:nonasymp} and \ref{sec:asymptotic}.
\clayton{Is it okay that we rephrase them to have them in terms of $\delta$?}

\begin{theorem}[\cite{hmx20} Theorem~1: Upper-bound on SV proliferation threshold for anisotropic subgaussian]\label{thm:hmx-ub}
    Consider a $\lambda$-anisotropic sample $\bX$ and $y$ and some $\delta > 0$.
    If $d_{\infty} = \Omega(n \log (n) \log (\frac{1}{\delta}))$, then with every sample is a support vector for the $\ell_2$ SVM problem with probability $1 - \delta$.
\end{theorem}

\begin{theorem}[\cite{hmx20} Theorem~3: Lower-bound on SV proliferation threshold for isotropic Gaussian]\label{thm:hmx-lb}
    Consider an isotropic Gaussian sample $\bX$ and $y$. 
    If $d = O(n)$, then with constant probability, there exists some sample that is not a supprt vector for the $\ell_2$ SVM problem. 
\end{theorem}

The authors of \cite{hmx20} note the logarithmic separation between Theorems~\ref{thm:hmx-ub} and \ref{thm:hmx-lb} and the limited data model used in Theorem~\ref{thm:hmx-lb}, and pose an improvement to their lower-bound as an open problem.
We solve this problem for the $\ell_2$ case here by broadening Theorem~\ref{thm:hmx-lb} to handle $\lambda$-anisotropic samples and by eliminating the logarithmic separation in Theorem~\ref{thm:anisotropic}.
In addition, we show that the threshold can be precisely captured up to constant factor as $n$ and $d$ trend towards $\infty$ in the isotropic Gaussian setting in Theorems~\ref{thm:asymptotic-lb} and \ref{thm:asymptotic-up}.


We make extensive use of the deterministic equivalence given in \cite{hmx20}.
\begin{lemma}\label{lemma:hmx-equivalence}
    For samples $(\bx_1, y_1), \dots, (\bx_n, y_n)\in \R^d \times \flip$ such that $\bK$ and $\bK_{\setminus i} := \bX_{\setminus i} \bX_{\setminus i}^\T$ are non-singular for all $i \in [n]$, every training sample is a support vector for the solution to the $\ell_2$ SVM if and only if $y_i y_{\setminus i}^\T \bK_{\setminus i}^{-1} \bX_{\setminus i} \bx_i < 1$ for all $i \in [n]$.
\end{lemma}
We also offer an alternate proof the lemma in the appendix. \todo{do this and give geometric interpretation of lemma}
